Search for charged Higgs bosons in the $H^{\pm} \rightarrow tb$ decay channel in $pp$ collisions at $\sqrt{s} = 8$ TeV using the ATLAS detector

Charged Higgs bosons heavier than the top quark and decaying via $H^{\pm} \rightarrow tb$ are searched for in proton--proton collisions measured with the ATLAS experiment at $\sqrt{s}=8$ TeV corresponding to an integrated luminosity of 20.3 fb$^{-1}$. The production of a charged Higgs boson in association with a top quark, $gb \rightarrow tH^{\pm}$, is explored in the mass range 200 to 600 GeV using multi-jet final states with one electron or muon. In order to separate the signal from the Standard Model background, analysis techniques combining several kinematic variables are employed. An excess of events above the background-only hypothesis is observed across a wide mass range, amounting to up to 2.4 standard deviations. Upper limits are set on the $gb\rightarrow tH^{\pm}$ production cross section times the branching fraction $\mathrm{BR}(H^{\pm} \rightarrow tb)$. Additionally, the complementary $s$-channel production, $qq' \rightarrow H^{\pm}$, is investigated through a reinterpretation of $W' \rightarrow tb$ searches in ATLAS. Final states with one electron or muon are relevant for $H^{\pm}$ masses from 0.4 to 2.0 TeV, whereas the all-hadronic final state covers the range 1.5 to 3.0 TeV. In these search channels, no significant excesses from the predictions of the Standard Model are observed, and upper limits are placed on the $qq' \rightarrow H^{\pm}$ production cross section times the branching fraction BR$(H^{\pm} \rightarrow tb)$.

==> atlas_authlist.tex <==
% ATLAS Collaboration author list
% Data extracted on 27-Oct-2015 for paper reference HIGG-2013-28
%\documentclass[11pt]{article}
%\usepackage{a4wide}\begin{document}
\begin{flushleft}
{\Large The ATLAS Collaboration}

\bigskip

G.~Aad$^\textrm{\scriptsize 85}$,
B.~Abbott$^\textrm{\scriptsize 113}$,
J.~Abdallah$^\textrm{\scriptsize 151}$,
O.~Abdinov$^\textrm{\scriptsize 11}$,
R.~Aben$^\textrm{\scriptsize 107}$,
M.~Abolins$^\textrm{\scriptsize 90}$,
O.S.~AbouZeid$^\textrm{\scriptsize 158}$,
H.~Abramowicz$^\textrm{\scriptsize 153}$,
H.~Abreu$^\textrm{\scriptsize 152}$,
R.~Abreu$^\textrm{\scriptsize 116}$,
Y.~Abulaiti$^\textrm{\scriptsize 146a,146b}$,
B.S.~Acharya$^\textrm{\scriptsize 164a,164b}$$^{,a}$,
L.~Adamczyk$^\textrm{\scriptsize 38a}$,
D.L.~Adams$^\textrm{\scriptsize 25}$,
J.~Adelman$^\textrm{\scriptsize 108}$,
S.~Adomeit$^\textrm{\scriptsize 100}$,
T.~Adye$^\textrm{\scriptsize 131}$,
A.A.~Affolder$^\textrm{\scriptsize 74}$,
T.~Agatonovic-Jovin$^\textrm{\scriptsize 13}$,
J.~Agricola$^\textrm{\scriptsize 54}$,
J.A.~Aguilar-Saavedra$^\textrm{\scriptsize 126a,126f}$,
S.P.~Ahlen$^\textrm{\scriptsize 22}$,
F.~Ahmadov$^\textrm{\scriptsize 65}$$^{,b}$,
G.~Aielli$^\textrm{\scriptsize 133a,133b}$,
H.~Akerstedt$^\textrm{\scriptsize 146a,146b}$,
T.P.A.~{\AA}kesson$^\textrm{\scriptsize 81}$,
A.V.~Akimov$^\textrm{\scriptsize 96}$,
G.L.~Alberghi$^\textrm{\scriptsize 20a,20b}$,
J.~Albert$^\textrm{\scriptsize 169}$,
S.~Albrand$^\textrm{\scriptsize 55}$,
M.J.~Alconada~Verzini$^\textrm{\scriptsize 71}$,
M.~Aleksa$^\textrm{\scriptsize 30}$,
I.N.~Aleksandrov$^\textrm{\scriptsize 65}$,
C.~Alexa$^\textrm{\scriptsize 26b}$,
G.~Alexander$^\textrm{\scriptsize 153}$,
T.~Alexopoulos$^\textrm{\scriptsize 10}$,
M.~Alhroob$^\textrm{\scriptsize 113}$,
G.~Alimonti$^\textrm{\scriptsize 91a}$,
L.~Alio$^\textrm{\scriptsize 85}$,
J.~Alison$^\textrm{\scriptsize 31}$,
S.P.~Alkire$^\textrm{\scriptsize 35}$,
B.M.M.~Allbrooke$^\textrm{\scriptsize 149}$,
P.P.~Allport$^\textrm{\scriptsize 18}$,
A.~Aloisio$^\textrm{\scriptsize 104a,104b}$,
A.~Alonso$^\textrm{\scriptsize 36}$,
F.~Alonso$^\textrm{\scriptsize 71}$,
C.~Alpigiani$^\textrm{\scriptsize 138}$,
B.~Alvarez~Gonzalez$^\textrm{\scriptsize 30}$,
D.~\'{A}lvarez~Piqueras$^\textrm{\scriptsize 167}$,
M.G.~Alviggi$^\textrm{\scriptsize 104a,104b}$,
B.T.~Amadio$^\textrm{\scriptsize 15}$,
K.~Amako$^\textrm{\scriptsize 66}$,
Y.~Amaral~Coutinho$^\textrm{\scriptsize 24a}$,
C.~Amelung$^\textrm{\scriptsize 23}$,
D.~Amidei$^\textrm{\scriptsize 89}$,
S.P.~Amor~Dos~Santos$^\textrm{\scriptsize 126a,126c}$,
A.~Amorim$^\textrm{\scriptsize 126a,126b}$,
S.~Amoroso$^\textrm{\scriptsize 48}$,
N.~Amram$^\textrm{\scriptsize 153}$,
G.~Amundsen$^\textrm{\scriptsize 23}$,
C.~Anastopoulos$^\textrm{\scriptsize 139}$,
L.S.~Ancu$^\textrm{\scriptsize 49}$,
N.~Andari$^\textrm{\scriptsize 108}$,
T.~Andeen$^\textrm{\scriptsize 31}$,
C.F.~Anders$^\textrm{\scriptsize 58b}$,
G.~Anders$^\textrm{\scriptsize 30}$,
J.K.~Anders$^\textrm{\scriptsize 74}$,
K.J.~Anderson$^\textrm{\scriptsize 31}$,
A.~Andreazza$^\textrm{\scriptsize 91a,91b}$,
V.~Andrei$^\textrm{\scriptsize 58a}$,
S.~Angelidakis$^\textrm{\scriptsize 9}$,
I.~Angelozzi$^\textrm{\scriptsize 107}$,
P.~Anger$^\textrm{\scriptsize 44}$,
A.~Angerami$^\textrm{\scriptsize 35}$,
F.~Anghinolfi$^\textrm{\scriptsize 30}$,
A.V.~Anisenkov$^\textrm{\scriptsize 109}$$^{,c}$,
N.~Anjos$^\textrm{\scriptsize 12}$,
A.~Annovi$^\textrm{\scriptsize 124a,124b}$,
M.~Antonelli$^\textrm{\scriptsize 47}$,
A.~Antonov$^\textrm{\scriptsize 98}$,
J.~Antos$^\textrm{\scriptsize 144b}$,
F.~Anulli$^\textrm{\scriptsize 132a}$,
M.~Aoki$^\textrm{\scriptsize 66}$,
L.~Aperio~Bella$^\textrm{\scriptsize 18}$,
G.~Arabidze$^\textrm{\scriptsize 90}$,
Y.~Arai$^\textrm{\scriptsize 66}$,
J.P.~Araque$^\textrm{\scriptsize 126a}$,
A.T.H.~Arce$^\textrm{\scriptsize 45}$,
F.A.~Arduh$^\textrm{\scriptsize 71}$,
J-F.~Arguin$^\textrm{\scriptsize 95}$,
S.~Argyropoulos$^\textrm{\scriptsize 63}$,
M.~Arik$^\textrm{\scriptsize 19a}$,
A.J.~Armbruster$^\textrm{\scriptsize 30}$,
O.~Arnaez$^\textrm{\scriptsize 30}$,
H.~Arnold$^\textrm{\scriptsize 48}$,
M.~Arratia$^\textrm{\scriptsize 28}$,
O.~Arslan$^\textrm{\scriptsize 21}$,
A.~Artamonov$^\textrm{\scriptsize 97}$,
G.~Artoni$^\textrm{\scriptsize 120}$,
S.~Artz$^\textrm{\scriptsize 83}$,
S.~Asai$^\textrm{\scriptsize 155}$,
N.~Asbah$^\textrm{\scriptsize 42}$,
A.~Ashkenazi$^\textrm{\scriptsize 153}$,
B.~{\AA}sman$^\textrm{\scriptsize 146a,146b}$,
L.~Asquith$^\textrm{\scriptsize 149}$,
K.~Assamagan$^\textrm{\scriptsize 25}$,
R.~Astalos$^\textrm{\scriptsize 144a}$,
M.~Atkinson$^\textrm{\scriptsize 165}$,
N.B.~Atlay$^\textrm{\scriptsize 141}$,
K.~Augsten$^\textrm{\scriptsize 128}$,
M.~Aurousseau$^\textrm{\scriptsize 145b}$,
G.~Avolio$^\textrm{\scriptsize 30}$,
B.~Axen$^\textrm{\scriptsize 15}$,
M.K.~Ayoub$^\textrm{\scriptsize 117}$,
G.~Azuelos$^\textrm{\scriptsize 95}$$^{,d}$,
M.A.~Baak$^\textrm{\scriptsize 30}$,
A.E.~Baas$^\textrm{\scriptsize 58a}$,
M.J.~Baca$^\textrm{\scriptsize 18}$,
H.~Bachacou$^\textrm{\scriptsize 136}$,
K.~Bachas$^\textrm{\scriptsize 154}$,
M.~Backes$^\textrm{\scriptsize 30}$,
M.~Backhaus$^\textrm{\scriptsize 30}$,
P.~Bagiacchi$^\textrm{\scriptsize 132a,132b}$,
P.~Bagnaia$^\textrm{\scriptsize 132a,132b}$,
Y.~Bai$^\textrm{\scriptsize 33a}$,
J.T.~Baines$^\textrm{\scriptsize 131}$,
O.K.~Baker$^\textrm{\scriptsize 176}$,
E.M.~Baldin$^\textrm{\scriptsize 109}$$^{,c}$,
P.~Balek$^\textrm{\scriptsize 129}$,
T.~Balestri$^\textrm{\scriptsize 148}$,
F.~Balli$^\textrm{\scriptsize 84}$,
W.K.~Balunas$^\textrm{\scriptsize 122}$,
E.~Banas$^\textrm{\scriptsize 39}$,
Sw.~Banerjee$^\textrm{\scriptsize 173}$$^{,e}$,
A.A.E.~Bannoura$^\textrm{\scriptsize 175}$,
L.~Barak$^\textrm{\scriptsize 30}$,
E.L.~Barberio$^\textrm{\scriptsize 88}$,
D.~Barberis$^\textrm{\scriptsize 50a,50b}$,
M.~Barbero$^\textrm{\scriptsize 85}$,
T.~Barillari$^\textrm{\scriptsize 101}$,
M.~Barisonzi$^\textrm{\scriptsize 164a,164b}$,
T.~Barklow$^\textrm{\scriptsize 143}$,
N.~Barlow$^\textrm{\scriptsize 28}$,
S.L.~Barnes$^\textrm{\scriptsize 84}$,
B.M.~Barnett$^\textrm{\scriptsize 131}$,
R.M.~Barnett$^\textrm{\scriptsize 15}$,
Z.~Barnovska$^\textrm{\scriptsize 5}$,
A.~Baroncelli$^\textrm{\scriptsize 134a}$,
G.~Barone$^\textrm{\scriptsize 23}$,
A.J.~Barr$^\textrm{\scriptsize 120}$,
F.~Barreiro$^\textrm{\scriptsize 82}$,
J.~Barreiro~Guimar\~{a}es~da~Costa$^\textrm{\scriptsize 33a}$,
R.~Bartoldus$^\textrm{\scriptsize 143}$,
A.E.~Barton$^\textrm{\scriptsize 72}$,
P.~Bartos$^\textrm{\scriptsize 144a}$,
A.~Basalaev$^\textrm{\scriptsize 123}$,
A.~Bassalat$^\textrm{\scriptsize 117}$,
A.~Basye$^\textrm{\scriptsize 165}$,
R.L.~Bates$^\textrm{\scriptsize 53}$,
S.J.~Batista$^\textrm{\scriptsize 158}$,
J.R.~Batley$^\textrm{\scriptsize 28}$,
M.~Battaglia$^\textrm{\scriptsize 137}$,
M.~Bauce$^\textrm{\scriptsize 132a,132b}$,
F.~Bauer$^\textrm{\scriptsize 136}$,
H.S.~Bawa$^\textrm{\scriptsize 143}$$^{,f}$,
J.B.~Beacham$^\textrm{\scriptsize 111}$,
M.D.~Beattie$^\textrm{\scriptsize 72}$,
T.~Beau$^\textrm{\scriptsize 80}$,
P.H.~Beauchemin$^\textrm{\scriptsize 161}$,
R.~Beccherle$^\textrm{\scriptsize 124a,124b}$,
P.~Bechtle$^\textrm{\scriptsize 21}$,
H.P.~Beck$^\textrm{\scriptsize 17}$$^{,g}$,
K.~Becker$^\textrm{\scriptsize 120}$,
M.~Becker$^\textrm{\scriptsize 83}$,
M.~Beckingham$^\textrm{\scriptsize 170}$,
C.~Becot$^\textrm{\scriptsize 117}$,
A.J.~Beddall$^\textrm{\scriptsize 19b}$,
A.~Beddall$^\textrm{\scriptsize 19b}$,
V.A.~Bednyakov$^\textrm{\scriptsize 65}$,
C.P.~Bee$^\textrm{\scriptsize 148}$,
L.J.~Beemster$^\textrm{\scriptsize 107}$,
T.A.~Beermann$^\textrm{\scriptsize 30}$,
M.~Begel$^\textrm{\scriptsize 25}$,
J.K.~Behr$^\textrm{\scriptsize 120}$,
C.~Belanger-Champagne$^\textrm{\scriptsize 87}$,
W.H.~Bell$^\textrm{\scriptsize 49}$,
G.~Bella$^\textrm{\scriptsize 153}$,
L.~Bellagamba$^\textrm{\scriptsize 20a}$,
A.~Bellerive$^\textrm{\scriptsize 29}$,
M.~Bellomo$^\textrm{\scriptsize 86}$,
K.~Belotskiy$^\textrm{\scriptsize 98}$,
O.~Beltramello$^\textrm{\scriptsize 30}$,
O.~Benary$^\textrm{\scriptsize 153}$,
D.~Benchekroun$^\textrm{\scriptsize 135a}$,
M.~Bender$^\textrm{\scriptsize 100}$,
K.~Bendtz$^\textrm{\scriptsize 146a,146b}$,
N.~Benekos$^\textrm{\scriptsize 10}$,
Y.~Benhammou$^\textrm{\scriptsize 153}$,
E.~Benhar~Noccioli$^\textrm{\scriptsize 176}$,
J.A.~Benitez~Garcia$^\textrm{\scriptsize 159b}$,
D.P.~Benjamin$^\textrm{\scriptsize 45}$,
J.R.~Bensinger$^\textrm{\scriptsize 23}$,
S.~Bentvelsen$^\textrm{\scriptsize 107}$,
L.~Beresford$^\textrm{\scriptsize 120}$,
M.~Beretta$^\textrm{\scriptsize 47}$,
D.~Berge$^\textrm{\scriptsize 107}$,
E.~Bergeaas~Kuutmann$^\textrm{\scriptsize 166}$,
N.~Berger$^\textrm{\scriptsize 5}$,
F.~Berghaus$^\textrm{\scriptsize 169}$,
J.~Beringer$^\textrm{\scriptsize 15}$,
C.~Bernard$^\textrm{\scriptsize 22}$,
N.R.~Bernard$^\textrm{\scriptsize 86}$,
C.~Bernius$^\textrm{\scriptsize 110}$,
F.U.~Bernlochner$^\textrm{\scriptsize 21}$,
T.~Berry$^\textrm{\scriptsize 77}$,
P.~Berta$^\textrm{\scriptsize 129}$,
C.~Bertella$^\textrm{\scriptsize 83}$,
G.~Bertoli$^\textrm{\scriptsize 146a,146b}$,
F.~Bertolucci$^\textrm{\scriptsize 124a,124b}$,
C.~Bertsche$^\textrm{\scriptsize 113}$,
D.~Bertsche$^\textrm{\scriptsize 113}$,
G.J.~Besjes$^\textrm{\scriptsize 36}$,
O.~Bessidskaia~Bylund$^\textrm{\scriptsize 146a,146b}$,
M.~Bessner$^\textrm{\scriptsize 42}$,
N.~Besson$^\textrm{\scriptsize 136}$,
C.~Betancourt$^\textrm{\scriptsize 48}$,
S.~Bethke$^\textrm{\scriptsize 101}$,
A.J.~Bevan$^\textrm{\scriptsize 76}$,
W.~Bhimji$^\textrm{\scriptsize 15}$,
R.M.~Bianchi$^\textrm{\scriptsize 125}$,
L.~Bianchini$^\textrm{\scriptsize 23}$,
M.~Bianco$^\textrm{\scriptsize 30}$,
O.~Biebel$^\textrm{\scriptsize 100}$,
D.~Biedermann$^\textrm{\scriptsize 16}$,
N.V.~Biesuz$^\textrm{\scriptsize 124a,124b}$,
M.~Biglietti$^\textrm{\scriptsize 134a}$,
J.~Bilbao~De~Mendizabal$^\textrm{\scriptsize 49}$,
H.~Bilokon$^\textrm{\scriptsize 47}$,
M.~Bindi$^\textrm{\scriptsize 54}$,
S.~Binet$^\textrm{\scriptsize 117}$,
A.~Bingul$^\textrm{\scriptsize 19b}$,
C.~Bini$^\textrm{\scriptsize 132a,132b}$,
S.~Biondi$^\textrm{\scriptsize 20a,20b}$,
D.M.~Bjergaard$^\textrm{\scriptsize 45}$,
C.W.~Black$^\textrm{\scriptsize 150}$,
J.E.~Black$^\textrm{\scriptsize 143}$,
K.M.~Black$^\textrm{\scriptsize 22}$,
D.~Blackburn$^\textrm{\scriptsize 138}$,
R.E.~Blair$^\textrm{\scriptsize 6}$,
J.-B.~Blanchard$^\textrm{\scriptsize 136}$,
J.E.~Blanco$^\textrm{\scriptsize 77}$,
T.~Blazek$^\textrm{\scriptsize 144a}$,
I.~Bloch$^\textrm{\scriptsize 42}$,
C.~Blocker$^\textrm{\scriptsize 23}$,
W.~Blum$^\textrm{\scriptsize 83}$$^{,*}$,
U.~Blumenschein$^\textrm{\scriptsize 54}$,
S.~Blunier$^\textrm{\scriptsize 32a}$,
G.J.~Bobbink$^\textrm{\scriptsize 107}$,
V.S.~Bobrovnikov$^\textrm{\scriptsize 109}$$^{,c}$,
S.S.~Bocchetta$^\textrm{\scriptsize 81}$,
A.~Bocci$^\textrm{\scriptsize 45}$,
C.~Bock$^\textrm{\scriptsize 100}$,
M.~Boehler$^\textrm{\scriptsize 48}$,
J.A.~Bogaerts$^\textrm{\scriptsize 30}$,
D.~Bogavac$^\textrm{\scriptsize 13}$,
A.G.~Bogdanchikov$^\textrm{\scriptsize 109}$,
C.~Bohm$^\textrm{\scriptsize 146a}$,
V.~Boisvert$^\textrm{\scriptsize 77}$,
T.~Bold$^\textrm{\scriptsize 38a}$,
V.~Boldea$^\textrm{\scriptsize 26b}$,
A.S.~Boldyrev$^\textrm{\scriptsize 99}$,
M.~Bomben$^\textrm{\scriptsize 80}$,
M.~Bona$^\textrm{\scriptsize 76}$,
M.~Boonekamp$^\textrm{\scriptsize 136}$,
A.~Borisov$^\textrm{\scriptsize 130}$,
G.~Borissov$^\textrm{\scriptsize 72}$,
S.~Borroni$^\textrm{\scriptsize 42}$,
J.~Bortfeldt$^\textrm{\scriptsize 100}$,
V.~Bortolotto$^\textrm{\scriptsize 60a,60b,60c}$,
K.~Bos$^\textrm{\scriptsize 107}$,
D.~Boscherini$^\textrm{\scriptsize 20a}$,
M.~Bosman$^\textrm{\scriptsize 12}$,
J.~Boudreau$^\textrm{\scriptsize 125}$,
J.~Bouffard$^\textrm{\scriptsize 2}$,
E.V.~Bouhova-Thacker$^\textrm{\scriptsize 72}$,
D.~Boumediene$^\textrm{\scriptsize 34}$,
C.~Bourdarios$^\textrm{\scriptsize 117}$,
N.~Bousson$^\textrm{\scriptsize 114}$,
S.K.~Boutle$^\textrm{\scriptsize 53}$,
A.~Boveia$^\textrm{\scriptsize 30}$,
J.~Boyd$^\textrm{\scriptsize 30}$,
I.R.~Boyko$^\textrm{\scriptsize 65}$,
J.~Bracinik$^\textrm{\scriptsize 18}$,
A.~Brandt$^\textrm{\scriptsize 8}$,
G.~Brandt$^\textrm{\scriptsize 54}$,
O.~Brandt$^\textrm{\scriptsize 58a}$,
U.~Bratzler$^\textrm{\scriptsize 156}$,
B.~Brau$^\textrm{\scriptsize 86}$,
J.E.~Brau$^\textrm{\scriptsize 116}$,
H.M.~Braun$^\textrm{\scriptsize 175}$$^{,*}$,
W.D.~Breaden~Madden$^\textrm{\scriptsize 53}$,
K.~Brendlinger$^\textrm{\scriptsize 122}$,
A.J.~Brennan$^\textrm{\scriptsize 88}$,
L.~Brenner$^\textrm{\scriptsize 107}$,
R.~Brenner$^\textrm{\scriptsize 166}$,
S.~Bressler$^\textrm{\scriptsize 172}$,
T.M.~Bristow$^\textrm{\scriptsize 46}$,
D.~Britton$^\textrm{\scriptsize 53}$,
D.~Britzger$^\textrm{\scriptsize 42}$,
F.M.~Brochu$^\textrm{\scriptsize 28}$,
I.~Brock$^\textrm{\scriptsize 21}$,
R.~Brock$^\textrm{\scriptsize 90}$,
G.~Brooijmans$^\textrm{\scriptsize 35}$,
T.~Brooks$^\textrm{\scriptsize 77}$,
W.K.~Brooks$^\textrm{\scriptsize 32b}$,
J.~Brosamer$^\textrm{\scriptsize 15}$,
E.~Brost$^\textrm{\scriptsize 116}$,
P.A.~Bruckman~de~Renstrom$^\textrm{\scriptsize 39}$,
D.~Bruncko$^\textrm{\scriptsize 144b}$,
R.~Bruneliere$^\textrm{\scriptsize 48}$,
A.~Bruni$^\textrm{\scriptsize 20a}$,
G.~Bruni$^\textrm{\scriptsize 20a}$,
M.~Bruschi$^\textrm{\scriptsize 20a}$,
N.~Bruscino$^\textrm{\scriptsize 21}$,
L.~Bryngemark$^\textrm{\scriptsize 81}$,
T.~Buanes$^\textrm{\scriptsize 14}$,
Q.~Buat$^\textrm{\scriptsize 142}$,
P.~Buchholz$^\textrm{\scriptsize 141}$,
A.G.~Buckley$^\textrm{\scriptsize 53}$,
I.A.~Budagov$^\textrm{\scriptsize 65}$,
F.~Buehrer$^\textrm{\scriptsize 48}$,
L.~Bugge$^\textrm{\scriptsize 119}$,
M.K.~Bugge$^\textrm{\scriptsize 119}$,
O.~Bulekov$^\textrm{\scriptsize 98}$,
D.~Bullock$^\textrm{\scriptsize 8}$,
H.~Burckhart$^\textrm{\scriptsize 30}$,
S.~Burdin$^\textrm{\scriptsize 74}$,
C.D.~Burgard$^\textrm{\scriptsize 48}$,
B.~Burghgrave$^\textrm{\scriptsize 108}$,
S.~Burke$^\textrm{\scriptsize 131}$,
I.~Burmeister$^\textrm{\scriptsize 43}$,
E.~Busato$^\textrm{\scriptsize 34}$,
D.~B\"uscher$^\textrm{\scriptsize 48}$,
V.~B\"uscher$^\textrm{\scriptsize 83}$,
P.~Bussey$^\textrm{\scriptsize 53}$,
J.M.~Butler$^\textrm{\scriptsize 22}$,
A.I.~Butt$^\textrm{\scriptsize 3}$,
C.M.~Buttar$^\textrm{\scriptsize 53}$,
J.M.~Butterworth$^\textrm{\scriptsize 78}$,
P.~Butti$^\textrm{\scriptsize 107}$,
W.~Buttinger$^\textrm{\scriptsize 25}$,
A.~Buzatu$^\textrm{\scriptsize 53}$,
A.R.~Buzykaev$^\textrm{\scriptsize 109}$$^{,c}$,
S.~Cabrera~Urb\'an$^\textrm{\scriptsize 167}$,
D.~Caforio$^\textrm{\scriptsize 128}$,
V.M.~Cairo$^\textrm{\scriptsize 37a,37b}$,
O.~Cakir$^\textrm{\scriptsize 4a}$,
N.~Calace$^\textrm{\scriptsize 49}$,
P.~Calafiura$^\textrm{\scriptsize 15}$,
A.~Calandri$^\textrm{\scriptsize 136}$,
G.~Calderini$^\textrm{\scriptsize 80}$,
P.~Calfayan$^\textrm{\scriptsize 100}$,
L.P.~Caloba$^\textrm{\scriptsize 24a}$,
D.~Calvet$^\textrm{\scriptsize 34}$,
S.~Calvet$^\textrm{\scriptsize 34}$,
R.~Camacho~Toro$^\textrm{\scriptsize 31}$,
S.~Camarda$^\textrm{\scriptsize 42}$,
P.~Camarri$^\textrm{\scriptsize 133a,133b}$,
D.~Cameron$^\textrm{\scriptsize 119}$,
R.~Caminal~Armadans$^\textrm{\scriptsize 165}$,
S.~Campana$^\textrm{\scriptsize 30}$,
M.~Campanelli$^\textrm{\scriptsize 78}$,
A.~Campoverde$^\textrm{\scriptsize 148}$,
V.~Canale$^\textrm{\scriptsize 104a,104b}$,
A.~Canepa$^\textrm{\scriptsize 159a}$,
M.~Cano~Bret$^\textrm{\scriptsize 33e}$,
J.~Cantero$^\textrm{\scriptsize 82}$,
R.~Cantrill$^\textrm{\scriptsize 126a}$,
T.~Cao$^\textrm{\scriptsize 40}$,
M.D.M.~Capeans~Garrido$^\textrm{\scriptsize 30}$,
I.~Caprini$^\textrm{\scriptsize 26b}$,
M.~Caprini$^\textrm{\scriptsize 26b}$,
M.~Capua$^\textrm{\scriptsize 37a,37b}$,
R.~Caputo$^\textrm{\scriptsize 83}$,
R.M.~Carbone$^\textrm{\scriptsize 35}$,
R.~Cardarelli$^\textrm{\scriptsize 133a}$,
F.~Cardillo$^\textrm{\scriptsize 48}$,
T.~Carli$^\textrm{\scriptsize 30}$,
G.~Carlino$^\textrm{\scriptsize 104a}$,
L.~Carminati$^\textrm{\scriptsize 91a,91b}$,
S.~Caron$^\textrm{\scriptsize 106}$,
E.~Carquin$^\textrm{\scriptsize 32a}$,
G.D.~Carrillo-Montoya$^\textrm{\scriptsize 30}$,
J.R.~Carter$^\textrm{\scriptsize 28}$,
J.~Carvalho$^\textrm{\scriptsize 126a,126c}$,
D.~Casadei$^\textrm{\scriptsize 78}$,
M.P.~Casado$^\textrm{\scriptsize 12}$,
M.~Casolino$^\textrm{\scriptsize 12}$,
D.W.~Casper$^\textrm{\scriptsize 163}$,
E.~Castaneda-Miranda$^\textrm{\scriptsize 145a}$,
A.~Castelli$^\textrm{\scriptsize 107}$,
V.~Castillo~Gimenez$^\textrm{\scriptsize 167}$,
N.F.~Castro$^\textrm{\scriptsize 126a}$$^{,h}$,
P.~Catastini$^\textrm{\scriptsize 57}$,
A.~Catinaccio$^\textrm{\scriptsize 30}$,
J.R.~Catmore$^\textrm{\scriptsize 119}$,
A.~Cattai$^\textrm{\scriptsize 30}$,
J.~Caudron$^\textrm{\scriptsize 83}$,
V.~Cavaliere$^\textrm{\scriptsize 165}$,
D.~Cavalli$^\textrm{\scriptsize 91a}$,
M.~Cavalli-Sforza$^\textrm{\scriptsize 12}$,
V.~Cavasinni$^\textrm{\scriptsize 124a,124b}$,
F.~Ceradini$^\textrm{\scriptsize 134a,134b}$,
L.~Cerda~Alberich$^\textrm{\scriptsize 167}$,
B.C.~Cerio$^\textrm{\scriptsize 45}$,
A.S.~Cerqueira$^\textrm{\scriptsize 24b}$,
A.~Cerri$^\textrm{\scriptsize 149}$,
L.~Cerrito$^\textrm{\scriptsize 76}$,
F.~Cerutti$^\textrm{\scriptsize 15}$,
M.~Cerv$^\textrm{\scriptsize 30}$,
A.~Cervelli$^\textrm{\scriptsize 17}$,
S.A.~Cetin$^\textrm{\scriptsize 19c}$,
A.~Chafaq$^\textrm{\scriptsize 135a}$,
D.~Chakraborty$^\textrm{\scriptsize 108}$,
I.~Chalupkova$^\textrm{\scriptsize 129}$,
Y.L.~Chan$^\textrm{\scriptsize 60a}$,
P.~Chang$^\textrm{\scriptsize 165}$,
J.D.~Chapman$^\textrm{\scriptsize 28}$,
D.G.~Charlton$^\textrm{\scriptsize 18}$,
C.C.~Chau$^\textrm{\scriptsize 158}$,
C.A.~Chavez~Barajas$^\textrm{\scriptsize 149}$,
S.~Che$^\textrm{\scriptsize 111}$,
S.~Cheatham$^\textrm{\scriptsize 152}$,
A.~Chegwidden$^\textrm{\scriptsize 90}$,
S.~Chekanov$^\textrm{\scriptsize 6}$,
S.V.~Chekulaev$^\textrm{\scriptsize 159a}$,
G.A.~Chelkov$^\textrm{\scriptsize 65}$$^{,i}$,
M.A.~Chelstowska$^\textrm{\scriptsize 89}$,
C.~Chen$^\textrm{\scriptsize 64}$,
H.~Chen$^\textrm{\scriptsize 25}$,
K.~Chen$^\textrm{\scriptsize 148}$,
L.~Chen$^\textrm{\scriptsize 33d}$$^{,j}$,
S.~Chen$^\textrm{\scriptsize 33c}$,
S.~Chen$^\textrm{\scriptsize 155}$,
X.~Chen$^\textrm{\scriptsize 33f}$,
Y.~Chen$^\textrm{\scriptsize 67}$,
H.C.~Cheng$^\textrm{\scriptsize 89}$,
Y.~Cheng$^\textrm{\scriptsize 31}$,
A.~Cheplakov$^\textrm{\scriptsize 65}$,
E.~Cheremushkina$^\textrm{\scriptsize 130}$,
R.~Cherkaoui~El~Moursli$^\textrm{\scriptsize 135e}$,
V.~Chernyatin$^\textrm{\scriptsize 25}$$^{,*}$,
E.~Cheu$^\textrm{\scriptsize 7}$,
L.~Chevalier$^\textrm{\scriptsize 136}$,
V.~Chiarella$^\textrm{\scriptsize 47}$,
G.~Chiarelli$^\textrm{\scriptsize 124a,124b}$,
G.~Chiodini$^\textrm{\scriptsize 73a}$,
A.S.~Chisholm$^\textrm{\scriptsize 18}$,
R.T.~Chislett$^\textrm{\scriptsize 78}$,
A.~Chitan$^\textrm{\scriptsize 26b}$,
M.V.~Chizhov$^\textrm{\scriptsize 65}$,
K.~Choi$^\textrm{\scriptsize 61}$,
S.~Chouridou$^\textrm{\scriptsize 9}$,
B.K.B.~Chow$^\textrm{\scriptsize 100}$,
V.~Christodoulou$^\textrm{\scriptsize 78}$,
D.~Chromek-Burckhart$^\textrm{\scriptsize 30}$,
J.~Chudoba$^\textrm{\scriptsize 127}$,
A.J.~Chuinard$^\textrm{\scriptsize 87}$,
J.J.~Chwastowski$^\textrm{\scriptsize 39}$,
L.~Chytka$^\textrm{\scriptsize 115}$,
G.~Ciapetti$^\textrm{\scriptsize 132a,132b}$,
A.K.~Ciftci$^\textrm{\scriptsize 4a}$,
D.~Cinca$^\textrm{\scriptsize 53}$,
V.~Cindro$^\textrm{\scriptsize 75}$,
I.A.~Cioara$^\textrm{\scriptsize 21}$,
A.~Ciocio$^\textrm{\scriptsize 15}$,
F.~Cirotto$^\textrm{\scriptsize 104a,104b}$,
Z.H.~Citron$^\textrm{\scriptsize 172}$,
M.~Ciubancan$^\textrm{\scriptsize 26b}$,
A.~Clark$^\textrm{\scriptsize 49}$,
B.L.~Clark$^\textrm{\scriptsize 57}$,
P.J.~Clark$^\textrm{\scriptsize 46}$,
R.N.~Clarke$^\textrm{\scriptsize 15}$,
C.~Clement$^\textrm{\scriptsize 146a,146b}$,
Y.~Coadou$^\textrm{\scriptsize 85}$,
M.~Cobal$^\textrm{\scriptsize 164a,164c}$,
A.~Coccaro$^\textrm{\scriptsize 49}$,
J.~Cochran$^\textrm{\scriptsize 64}$,
L.~Coffey$^\textrm{\scriptsize 23}$,
H.~Cohen$^\textrm{\scriptsize 153}$,
L.~Colasurdo$^\textrm{\scriptsize 106}$,
B.~Cole$^\textrm{\scriptsize 35}$,
S.~Cole$^\textrm{\scriptsize 108}$,
A.P.~Colijn$^\textrm{\scriptsize 107}$,
J.~Collot$^\textrm{\scriptsize 55}$,
T.~Colombo$^\textrm{\scriptsize 58c}$,
G.~Compostella$^\textrm{\scriptsize 101}$,
P.~Conde~Mui\~no$^\textrm{\scriptsize 126a,126b}$,
E.~Coniavitis$^\textrm{\scriptsize 48}$,
S.H.~Connell$^\textrm{\scriptsize 145b}$,
I.A.~Connelly$^\textrm{\scriptsize 77}$,
V.~Consorti$^\textrm{\scriptsize 48}$,
S.~Constantinescu$^\textrm{\scriptsize 26b}$,
C.~Conta$^\textrm{\scriptsize 121a,121b}$,
G.~Conti$^\textrm{\scriptsize 30}$,
F.~Conventi$^\textrm{\scriptsize 104a}$$^{,k}$,
M.~Cooke$^\textrm{\scriptsize 15}$,
B.D.~Cooper$^\textrm{\scriptsize 78}$,
A.M.~Cooper-Sarkar$^\textrm{\scriptsize 120}$,
T.~Cornelissen$^\textrm{\scriptsize 175}$,
M.~Corradi$^\textrm{\scriptsize 132a,132b}$,
F.~Corriveau$^\textrm{\scriptsize 87}$$^{,l}$,
A.~Corso-Radu$^\textrm{\scriptsize 163}$,
A.~Cortes-Gonzalez$^\textrm{\scriptsize 12}$,
G.~Cortiana$^\textrm{\scriptsize 101}$,
G.~Costa$^\textrm{\scriptsize 91a}$,
M.J.~Costa$^\textrm{\scriptsize 167}$,
D.~Costanzo$^\textrm{\scriptsize 139}$,
D.~C\^ot\'e$^\textrm{\scriptsize 8}$,
G.~Cottin$^\textrm{\scriptsize 28}$,
G.~Cowan$^\textrm{\scriptsize 77}$,
B.E.~Cox$^\textrm{\scriptsize 84}$,
K.~Cranmer$^\textrm{\scriptsize 110}$,
S.J.~Crawley$^\textrm{\scriptsize 53}$,
G.~Cree$^\textrm{\scriptsize 29}$,
S.~Cr\'ep\'e-Renaudin$^\textrm{\scriptsize 55}$,
F.~Crescioli$^\textrm{\scriptsize 80}$,
W.A.~Cribbs$^\textrm{\scriptsize 146a,146b}$,
M.~Crispin~Ortuzar$^\textrm{\scriptsize 120}$,
M.~Cristinziani$^\textrm{\scriptsize 21}$,
V.~Croft$^\textrm{\scriptsize 106}$,
G.~Crosetti$^\textrm{\scriptsize 37a,37b}$,
T.~Cuhadar~Donszelmann$^\textrm{\scriptsize 139}$,
J.~Cummings$^\textrm{\scriptsize 176}$,
M.~Curatolo$^\textrm{\scriptsize 47}$,
J.~C\'uth$^\textrm{\scriptsize 83}$,
C.~Cuthbert$^\textrm{\scriptsize 150}$,
H.~Czirr$^\textrm{\scriptsize 141}$,
P.~Czodrowski$^\textrm{\scriptsize 3}$,
S.~D'Auria$^\textrm{\scriptsize 53}$,
M.~D'Onofrio$^\textrm{\scriptsize 74}$,
M.J.~Da~Cunha~Sargedas~De~Sousa$^\textrm{\scriptsize 126a,126b}$,
C.~Da~Via$^\textrm{\scriptsize 84}$,
W.~Dabrowski$^\textrm{\scriptsize 38a}$,
A.~Dafinca$^\textrm{\scriptsize 120}$,
T.~Dai$^\textrm{\scriptsize 89}$,
O.~Dale$^\textrm{\scriptsize 14}$,
F.~Dallaire$^\textrm{\scriptsize 95}$,
C.~Dallapiccola$^\textrm{\scriptsize 86}$,
M.~Dam$^\textrm{\scriptsize 36}$,
J.R.~Dandoy$^\textrm{\scriptsize 31}$,
N.P.~Dang$^\textrm{\scriptsize 48}$,
A.C.~Daniells$^\textrm{\scriptsize 18}$,
M.~Danninger$^\textrm{\scriptsize 168}$,
M.~Dano~Hoffmann$^\textrm{\scriptsize 136}$,
V.~Dao$^\textrm{\scriptsize 48}$,
G.~Darbo$^\textrm{\scriptsize 50a}$,
S.~Darmora$^\textrm{\scriptsize 8}$,
J.~Dassoulas$^\textrm{\scriptsize 3}$,
A.~Dattagupta$^\textrm{\scriptsize 61}$,
W.~Davey$^\textrm{\scriptsize 21}$,
C.~David$^\textrm{\scriptsize 169}$,
T.~Davidek$^\textrm{\scriptsize 129}$,
E.~Davies$^\textrm{\scriptsize 120}$$^{,m}$,
M.~Davies$^\textrm{\scriptsize 153}$,
P.~Davison$^\textrm{\scriptsize 78}$,
Y.~Davygora$^\textrm{\scriptsize 58a}$,
E.~Dawe$^\textrm{\scriptsize 88}$,
I.~Dawson$^\textrm{\scriptsize 139}$,
R.K.~Daya-Ishmukhametova$^\textrm{\scriptsize 86}$,
K.~De$^\textrm{\scriptsize 8}$,
R.~de~Asmundis$^\textrm{\scriptsize 104a}$,
A.~De~Benedetti$^\textrm{\scriptsize 113}$,
S.~De~Castro$^\textrm{\scriptsize 20a,20b}$,
S.~De~Cecco$^\textrm{\scriptsize 80}$,
N.~De~Groot$^\textrm{\scriptsize 106}$,
P.~de~Jong$^\textrm{\scriptsize 107}$,
H.~De~la~Torre$^\textrm{\scriptsize 82}$,
F.~De~Lorenzi$^\textrm{\scriptsize 64}$,
D.~De~Pedis$^\textrm{\scriptsize 132a}$,
A.~De~Salvo$^\textrm{\scriptsize 132a}$,
U.~De~Sanctis$^\textrm{\scriptsize 149}$,
A.~De~Santo$^\textrm{\scriptsize 149}$,
J.B.~De~Vivie~De~Regie$^\textrm{\scriptsize 117}$,
W.J.~Dearnaley$^\textrm{\scriptsize 72}$,
R.~Debbe$^\textrm{\scriptsize 25}$,
C.~Debenedetti$^\textrm{\scriptsize 137}$,
D.V.~Dedovich$^\textrm{\scriptsize 65}$,
I.~Deigaard$^\textrm{\scriptsize 107}$,
J.~Del~Peso$^\textrm{\scriptsize 82}$,
T.~Del~Prete$^\textrm{\scriptsize 124a,124b}$,
D.~Delgove$^\textrm{\scriptsize 117}$,
F.~Deliot$^\textrm{\scriptsize 136}$,
C.M.~Delitzsch$^\textrm{\scriptsize 49}$,
M.~Deliyergiyev$^\textrm{\scriptsize 75}$,
A.~Dell'Acqua$^\textrm{\scriptsize 30}$,
L.~Dell'Asta$^\textrm{\scriptsize 22}$,
M.~Dell'Orso$^\textrm{\scriptsize 124a,124b}$,
M.~Della~Pietra$^\textrm{\scriptsize 104a}$$^{,k}$,
D.~della~Volpe$^\textrm{\scriptsize 49}$,
M.~Delmastro$^\textrm{\scriptsize 5}$,
P.A.~Delsart$^\textrm{\scriptsize 55}$,
C.~Deluca$^\textrm{\scriptsize 107}$,
D.A.~DeMarco$^\textrm{\scriptsize 158}$,
S.~Demers$^\textrm{\scriptsize 176}$,
M.~Demichev$^\textrm{\scriptsize 65}$,
A.~Demilly$^\textrm{\scriptsize 80}$,
S.P.~Denisov$^\textrm{\scriptsize 130}$,
D.~Denysiuk$^\textrm{\scriptsize 136}$,
D.~Derendarz$^\textrm{\scriptsize 39}$,
J.E.~Derkaoui$^\textrm{\scriptsize 135d}$,
F.~Derue$^\textrm{\scriptsize 80}$,
P.~Dervan$^\textrm{\scriptsize 74}$,
K.~Desch$^\textrm{\scriptsize 21}$,
C.~Deterre$^\textrm{\scriptsize 42}$,
K.~Dette$^\textrm{\scriptsize 43}$,
P.O.~Deviveiros$^\textrm{\scriptsize 30}$,
A.~Dewhurst$^\textrm{\scriptsize 131}$,
S.~Dhaliwal$^\textrm{\scriptsize 23}$,
A.~Di~Ciaccio$^\textrm{\scriptsize 133a,133b}$,
L.~Di~Ciaccio$^\textrm{\scriptsize 5}$,
A.~Di~Domenico$^\textrm{\scriptsize 132a,132b}$,
C.~Di~Donato$^\textrm{\scriptsize 132a,132b}$,
A.~Di~Girolamo$^\textrm{\scriptsize 30}$,
B.~Di~Girolamo$^\textrm{\scriptsize 30}$,
A.~Di~Mattia$^\textrm{\scriptsize 152}$,
B.~Di~Micco$^\textrm{\scriptsize 134a,134b}$,
R.~Di~Nardo$^\textrm{\scriptsize 47}$,
A.~Di~Simone$^\textrm{\scriptsize 48}$,
R.~Di~Sipio$^\textrm{\scriptsize 158}$,
D.~Di~Valentino$^\textrm{\scriptsize 29}$,
C.~Diaconu$^\textrm{\scriptsize 85}$,
M.~Diamond$^\textrm{\scriptsize 158}$,
F.A.~Dias$^\textrm{\scriptsize 46}$,
M.A.~Diaz$^\textrm{\scriptsize 32a}$,
E.B.~Diehl$^\textrm{\scriptsize 89}$,
J.~Dietrich$^\textrm{\scriptsize 16}$,
S.~Diglio$^\textrm{\scriptsize 85}$,
A.~Dimitrievska$^\textrm{\scriptsize 13}$,
J.~Dingfelder$^\textrm{\scriptsize 21}$,
P.~Dita$^\textrm{\scriptsize 26b}$,
S.~Dita$^\textrm{\scriptsize 26b}$,
F.~Dittus$^\textrm{\scriptsize 30}$,
F.~Djama$^\textrm{\scriptsize 85}$,
T.~Djobava$^\textrm{\scriptsize 51b}$,
J.I.~Djuvsland$^\textrm{\scriptsize 58a}$,
M.A.B.~do~Vale$^\textrm{\scriptsize 24c}$,
D.~Dobos$^\textrm{\scriptsize 30}$,
M.~Dobre$^\textrm{\scriptsize 26b}$,
C.~Doglioni$^\textrm{\scriptsize 81}$,
T.~Dohmae$^\textrm{\scriptsize 155}$,
J.~Dolejsi$^\textrm{\scriptsize 129}$,
Z.~Dolezal$^\textrm{\scriptsize 129}$,
B.A.~Dolgoshein$^\textrm{\scriptsize 98}$$^{,*}$,
M.~Donadelli$^\textrm{\scriptsize 24d}$,
S.~Donati$^\textrm{\scriptsize 124a,124b}$,
P.~Dondero$^\textrm{\scriptsize 121a,121b}$,
J.~Donini$^\textrm{\scriptsize 34}$,
J.~Dopke$^\textrm{\scriptsize 131}$,
A.~Doria$^\textrm{\scriptsize 104a}$,
M.T.~Dova$^\textrm{\scriptsize 71}$,
A.T.~Doyle$^\textrm{\scriptsize 53}$,
E.~Drechsler$^\textrm{\scriptsize 54}$,
M.~Dris$^\textrm{\scriptsize 10}$,
Y.~Du$^\textrm{\scriptsize 33d}$,
J.~Duarte-Campderros$^\textrm{\scriptsize 153}$,
E.~Dubreuil$^\textrm{\scriptsize 34}$,
E.~Duchovni$^\textrm{\scriptsize 172}$,
G.~Duckeck$^\textrm{\scriptsize 100}$,
O.A.~Ducu$^\textrm{\scriptsize 26b,85}$,
D.~Duda$^\textrm{\scriptsize 107}$,
A.~Dudarev$^\textrm{\scriptsize 30}$,
L.~Duflot$^\textrm{\scriptsize 117}$,
L.~Duguid$^\textrm{\scriptsize 77}$,
M.~D\"uhrssen$^\textrm{\scriptsize 30}$,
M.~Dunford$^\textrm{\scriptsize 58a}$,
H.~Duran~Yildiz$^\textrm{\scriptsize 4a}$,
M.~D\"uren$^\textrm{\scriptsize 52}$,
A.~Durglishvili$^\textrm{\scriptsize 51b}$,
D.~Duschinger$^\textrm{\scriptsize 44}$,
B.~Dutta$^\textrm{\scriptsize 42}$,
M.~Dyndal$^\textrm{\scriptsize 38a}$,
C.~Eckardt$^\textrm{\scriptsize 42}$,
K.M.~Ecker$^\textrm{\scriptsize 101}$,
R.C.~Edgar$^\textrm{\scriptsize 89}$,
W.~Edson$^\textrm{\scriptsize 2}$,
N.C.~Edwards$^\textrm{\scriptsize 46}$,
W.~Ehrenfeld$^\textrm{\scriptsize 21}$,
T.~Eifert$^\textrm{\scriptsize 30}$,
G.~Eigen$^\textrm{\scriptsize 14}$,
K.~Einsweiler$^\textrm{\scriptsize 15}$,
T.~Ekelof$^\textrm{\scriptsize 166}$,
M.~El~Kacimi$^\textrm{\scriptsize 135c}$,
M.~Ellert$^\textrm{\scriptsize 166}$,
S.~Elles$^\textrm{\scriptsize 5}$,
F.~Ellinghaus$^\textrm{\scriptsize 175}$,
A.A.~Elliot$^\textrm{\scriptsize 169}$,
N.~Ellis$^\textrm{\scriptsize 30}$,
J.~Elmsheuser$^\textrm{\scriptsize 100}$,
M.~Elsing$^\textrm{\scriptsize 30}$,
D.~Emeliyanov$^\textrm{\scriptsize 131}$,
Y.~Enari$^\textrm{\scriptsize 155}$,
O.C.~Endner$^\textrm{\scriptsize 83}$,
M.~Endo$^\textrm{\scriptsize 118}$,
J.~Erdmann$^\textrm{\scriptsize 43}$,
A.~Ereditato$^\textrm{\scriptsize 17}$,
G.~Ernis$^\textrm{\scriptsize 175}$,
J.~Ernst$^\textrm{\scriptsize 2}$,
M.~Ernst$^\textrm{\scriptsize 25}$,
S.~Errede$^\textrm{\scriptsize 165}$,
E.~Ertel$^\textrm{\scriptsize 83}$,
M.~Escalier$^\textrm{\scriptsize 117}$,
H.~Esch$^\textrm{\scriptsize 43}$,
C.~Escobar$^\textrm{\scriptsize 125}$,
B.~Esposito$^\textrm{\scriptsize 47}$,
A.I.~Etienvre$^\textrm{\scriptsize 136}$,
E.~Etzion$^\textrm{\scriptsize 153}$,
H.~Evans$^\textrm{\scriptsize 61}$,
A.~Ezhilov$^\textrm{\scriptsize 123}$,
L.~Fabbri$^\textrm{\scriptsize 20a,20b}$,
G.~Facini$^\textrm{\scriptsize 31}$,
R.M.~Fakhrutdinov$^\textrm{\scriptsize 130}$,
S.~Falciano$^\textrm{\scriptsize 132a}$,
R.J.~Falla$^\textrm{\scriptsize 78}$,
J.~Faltova$^\textrm{\scriptsize 129}$,
Y.~Fang$^\textrm{\scriptsize 33a}$,
M.~Fanti$^\textrm{\scriptsize 91a,91b}$,
A.~Farbin$^\textrm{\scriptsize 8}$,
A.~Farilla$^\textrm{\scriptsize 134a}$,
T.~Farooque$^\textrm{\scriptsize 12}$,
S.~Farrell$^\textrm{\scriptsize 15}$,
S.M.~Farrington$^\textrm{\scriptsize 170}$,
P.~Farthouat$^\textrm{\scriptsize 30}$,
F.~Fassi$^\textrm{\scriptsize 135e}$,
P.~Fassnacht$^\textrm{\scriptsize 30}$,
D.~Fassouliotis$^\textrm{\scriptsize 9}$,
M.~Faucci~Giannelli$^\textrm{\scriptsize 77}$,
A.~Favareto$^\textrm{\scriptsize 50a,50b}$,
L.~Fayard$^\textrm{\scriptsize 117}$,
O.L.~Fedin$^\textrm{\scriptsize 123}$$^{,n}$,
W.~Fedorko$^\textrm{\scriptsize 168}$,
S.~Feigl$^\textrm{\scriptsize 119}$,
L.~Feligioni$^\textrm{\scriptsize 85}$,
C.~Feng$^\textrm{\scriptsize 33d}$,
E.J.~Feng$^\textrm{\scriptsize 30}$,
H.~Feng$^\textrm{\scriptsize 89}$,
A.B.~Fenyuk$^\textrm{\scriptsize 130}$,
L.~Feremenga$^\textrm{\scriptsize 8}$,
P.~Fernandez~Martinez$^\textrm{\scriptsize 167}$,
S.~Fernandez~Perez$^\textrm{\scriptsize 12}$,
J.~Ferrando$^\textrm{\scriptsize 53}$,
A.~Ferrari$^\textrm{\scriptsize 166}$,
P.~Ferrari$^\textrm{\scriptsize 107}$,
R.~Ferrari$^\textrm{\scriptsize 121a}$,
D.E.~Ferreira~de~Lima$^\textrm{\scriptsize 53}$,
A.~Ferrer$^\textrm{\scriptsize 167}$,
D.~Ferrere$^\textrm{\scriptsize 49}$,
C.~Ferretti$^\textrm{\scriptsize 89}$,
A.~Ferretto~Parodi$^\textrm{\scriptsize 50a,50b}$,
F.~Fiedler$^\textrm{\scriptsize 83}$,
A.~Filip\v{c}i\v{c}$^\textrm{\scriptsize 75}$,
M.~Filipuzzi$^\textrm{\scriptsize 42}$,
F.~Filthaut$^\textrm{\scriptsize 106}$,
M.~Fincke-Keeler$^\textrm{\scriptsize 169}$,
K.D.~Finelli$^\textrm{\scriptsize 150}$,
M.C.N.~Fiolhais$^\textrm{\scriptsize 126a,126c}$,
L.~Fiorini$^\textrm{\scriptsize 167}$,
A.~Firan$^\textrm{\scriptsize 40}$,
A.~Fischer$^\textrm{\scriptsize 2}$,
C.~Fischer$^\textrm{\scriptsize 12}$,
J.~Fischer$^\textrm{\scriptsize 175}$,
W.C.~Fisher$^\textrm{\scriptsize 90}$,
N.~Flaschel$^\textrm{\scriptsize 42}$,
I.~Fleck$^\textrm{\scriptsize 141}$,
P.~Fleischmann$^\textrm{\scriptsize 89}$,
G.T.~Fletcher$^\textrm{\scriptsize 139}$,
G.~Fletcher$^\textrm{\scriptsize 76}$,
R.R.M.~Fletcher$^\textrm{\scriptsize 122}$,
T.~Flick$^\textrm{\scriptsize 175}$,
A.~Floderus$^\textrm{\scriptsize 81}$,
L.R.~Flores~Castillo$^\textrm{\scriptsize 60a}$,
M.J.~Flowerdew$^\textrm{\scriptsize 101}$,
G.T.~Forcolin$^\textrm{\scriptsize 84}$,
A.~Formica$^\textrm{\scriptsize 136}$,
A.~Forti$^\textrm{\scriptsize 84}$,
D.~Fournier$^\textrm{\scriptsize 117}$,
H.~Fox$^\textrm{\scriptsize 72}$,
S.~Fracchia$^\textrm{\scriptsize 12}$,
P.~Francavilla$^\textrm{\scriptsize 80}$,
M.~Franchini$^\textrm{\scriptsize 20a,20b}$,
D.~Francis$^\textrm{\scriptsize 30}$,
L.~Franconi$^\textrm{\scriptsize 119}$,
M.~Franklin$^\textrm{\scriptsize 57}$,
M.~Frate$^\textrm{\scriptsize 163}$,
M.~Fraternali$^\textrm{\scriptsize 121a,121b}$,
D.~Freeborn$^\textrm{\scriptsize 78}$,
S.T.~French$^\textrm{\scriptsize 28}$,
S.M.~Fressard-Batraneanu$^\textrm{\scriptsize 30}$,
F.~Friedrich$^\textrm{\scriptsize 44}$,
D.~Froidevaux$^\textrm{\scriptsize 30}$,
J.A.~Frost$^\textrm{\scriptsize 120}$,
C.~Fukunaga$^\textrm{\scriptsize 156}$,
E.~Fullana~Torregrosa$^\textrm{\scriptsize 83}$,
T.~Fusayasu$^\textrm{\scriptsize 102}$,
J.~Fuster$^\textrm{\scriptsize 167}$,
C.~Gabaldon$^\textrm{\scriptsize 55}$,
O.~Gabizon$^\textrm{\scriptsize 175}$,
A.~Gabrielli$^\textrm{\scriptsize 20a,20b}$,
A.~Gabrielli$^\textrm{\scriptsize 15}$,
G.P.~Gach$^\textrm{\scriptsize 18}$,
S.~Gadatsch$^\textrm{\scriptsize 30}$,
S.~Gadomski$^\textrm{\scriptsize 49}$,
G.~Gagliardi$^\textrm{\scriptsize 50a,50b}$,
P.~Gagnon$^\textrm{\scriptsize 61}$,
C.~Galea$^\textrm{\scriptsize 106}$,
B.~Galhardo$^\textrm{\scriptsize 126a,126c}$,
E.J.~Gallas$^\textrm{\scriptsize 120}$,
B.J.~Gallop$^\textrm{\scriptsize 131}$,
P.~Gallus$^\textrm{\scriptsize 128}$,
G.~Galster$^\textrm{\scriptsize 36}$,
K.K.~Gan$^\textrm{\scriptsize 111}$,
J.~Gao$^\textrm{\scriptsize 33b,85}$,
Y.~Gao$^\textrm{\scriptsize 46}$,
Y.S.~Gao$^\textrm{\scriptsize 143}$$^{,f}$,
F.M.~Garay~Walls$^\textrm{\scriptsize 46}$,
C.~Garc\'ia$^\textrm{\scriptsize 167}$,
J.E.~Garc\'ia~Navarro$^\textrm{\scriptsize 167}$,
M.~Garcia-Sciveres$^\textrm{\scriptsize 15}$,
R.W.~Gardner$^\textrm{\scriptsize 31}$,
N.~Garelli$^\textrm{\scriptsize 143}$,
V.~Garonne$^\textrm{\scriptsize 119}$,
C.~Gatti$^\textrm{\scriptsize 47}$,
A.~Gaudiello$^\textrm{\scriptsize 50a,50b}$,
G.~Gaudio$^\textrm{\scriptsize 121a}$,
B.~Gaur$^\textrm{\scriptsize 141}$,
L.~Gauthier$^\textrm{\scriptsize 95}$,
I.L.~Gavrilenko$^\textrm{\scriptsize 96}$,
C.~Gay$^\textrm{\scriptsize 168}$,
G.~Gaycken$^\textrm{\scriptsize 21}$,
E.N.~Gazis$^\textrm{\scriptsize 10}$,
Z.~Gecse$^\textrm{\scriptsize 168}$,
C.N.P.~Gee$^\textrm{\scriptsize 131}$,
Ch.~Geich-Gimbel$^\textrm{\scriptsize 21}$,
M.P.~Geisler$^\textrm{\scriptsize 58a}$,
C.~Gemme$^\textrm{\scriptsize 50a}$,
M.H.~Genest$^\textrm{\scriptsize 55}$,
C.~Geng$^\textrm{\scriptsize 33b}$$^{,o}$,
S.~Gentile$^\textrm{\scriptsize 132a,132b}$,
S.~George$^\textrm{\scriptsize 77}$,
D.~Gerbaudo$^\textrm{\scriptsize 163}$,
A.~Gershon$^\textrm{\scriptsize 153}$,
S.~Ghasemi$^\textrm{\scriptsize 141}$,
H.~Ghazlane$^\textrm{\scriptsize 135b}$,
B.~Giacobbe$^\textrm{\scriptsize 20a}$,
S.~Giagu$^\textrm{\scriptsize 132a,132b}$,
P.~Giannetti$^\textrm{\scriptsize 124a,124b}$,
B.~Gibbard$^\textrm{\scriptsize 25}$,
S.M.~Gibson$^\textrm{\scriptsize 77}$,
M.~Gignac$^\textrm{\scriptsize 168}$,
M.~Gilchriese$^\textrm{\scriptsize 15}$,
T.P.S.~Gillam$^\textrm{\scriptsize 28}$,
D.~Gillberg$^\textrm{\scriptsize 30}$,
G.~Gilles$^\textrm{\scriptsize 34}$,
D.M.~Gingrich$^\textrm{\scriptsize 3}$$^{,d}$,
N.~Giokaris$^\textrm{\scriptsize 9}$,
M.P.~Giordani$^\textrm{\scriptsize 164a,164c}$,
F.M.~Giorgi$^\textrm{\scriptsize 20a}$,
F.M.~Giorgi$^\textrm{\scriptsize 16}$,
P.F.~Giraud$^\textrm{\scriptsize 136}$,
P.~Giromini$^\textrm{\scriptsize 57}$,
D.~Giugni$^\textrm{\scriptsize 91a}$,
C.~Giuliani$^\textrm{\scriptsize 101}$,
M.~Giulini$^\textrm{\scriptsize 58b}$,
B.K.~Gjelsten$^\textrm{\scriptsize 119}$,
S.~Gkaitatzis$^\textrm{\scriptsize 154}$,
I.~Gkialas$^\textrm{\scriptsize 154}$,
E.L.~Gkougkousis$^\textrm{\scriptsize 117}$,
L.K.~Gladilin$^\textrm{\scriptsize 99}$,
C.~Glasman$^\textrm{\scriptsize 82}$,
J.~Glatzer$^\textrm{\scriptsize 30}$,
P.C.F.~Glaysher$^\textrm{\scriptsize 46}$,
A.~Glazov$^\textrm{\scriptsize 42}$,
M.~Goblirsch-Kolb$^\textrm{\scriptsize 101}$,
J.R.~Goddard$^\textrm{\scriptsize 76}$,
J.~Godlewski$^\textrm{\scriptsize 39}$,
S.~Goldfarb$^\textrm{\scriptsize 89}$,
T.~Golling$^\textrm{\scriptsize 49}$,
D.~Golubkov$^\textrm{\scriptsize 130}$,
A.~Gomes$^\textrm{\scriptsize 126a,126b,126d}$,
R.~Gon\c{c}alo$^\textrm{\scriptsize 126a}$,
J.~Goncalves~Pinto~Firmino~Da~Costa$^\textrm{\scriptsize 136}$,
L.~Gonella$^\textrm{\scriptsize 21}$,
S.~Gonz\'alez~de~la~Hoz$^\textrm{\scriptsize 167}$,
G.~Gonzalez~Parra$^\textrm{\scriptsize 12}$,
S.~Gonzalez-Sevilla$^\textrm{\scriptsize 49}$,
L.~Goossens$^\textrm{\scriptsize 30}$,
P.A.~Gorbounov$^\textrm{\scriptsize 97}$,
H.A.~Gordon$^\textrm{\scriptsize 25}$,
I.~Gorelov$^\textrm{\scriptsize 105}$,
B.~Gorini$^\textrm{\scriptsize 30}$,
E.~Gorini$^\textrm{\scriptsize 73a,73b}$,
A.~Gori\v{s}ek$^\textrm{\scriptsize 75}$,
E.~Gornicki$^\textrm{\scriptsize 39}$,
A.T.~Goshaw$^\textrm{\scriptsize 45}$,
C.~G\"ossling$^\textrm{\scriptsize 43}$,
M.I.~Gostkin$^\textrm{\scriptsize 65}$,
D.~Goujdami$^\textrm{\scriptsize 135c}$,
A.G.~Goussiou$^\textrm{\scriptsize 138}$,
N.~Govender$^\textrm{\scriptsize 145b}$,
E.~Gozani$^\textrm{\scriptsize 152}$,
L.~Graber$^\textrm{\scriptsize 54}$,
I.~Grabowska-Bold$^\textrm{\scriptsize 38a}$,
P.O.J.~Gradin$^\textrm{\scriptsize 166}$,
P.~Grafstr\"om$^\textrm{\scriptsize 20a,20b}$,
J.~Gramling$^\textrm{\scriptsize 49}$,
E.~Gramstad$^\textrm{\scriptsize 119}$,
S.~Grancagnolo$^\textrm{\scriptsize 16}$,
V.~Gratchev$^\textrm{\scriptsize 123}$,
H.M.~Gray$^\textrm{\scriptsize 30}$,
E.~Graziani$^\textrm{\scriptsize 134a}$,
Z.D.~Greenwood$^\textrm{\scriptsize 79}$$^{,p}$,
C.~Grefe$^\textrm{\scriptsize 21}$,
K.~Gregersen$^\textrm{\scriptsize 78}$,
I.M.~Gregor$^\textrm{\scriptsize 42}$,
P.~Grenier$^\textrm{\scriptsize 143}$,
J.~Griffiths$^\textrm{\scriptsize 8}$,
A.A.~Grillo$^\textrm{\scriptsize 137}$,
K.~Grimm$^\textrm{\scriptsize 72}$,
S.~Grinstein$^\textrm{\scriptsize 12}$$^{,q}$,
Ph.~Gris$^\textrm{\scriptsize 34}$,
J.-F.~Grivaz$^\textrm{\scriptsize 117}$,
S.~Groh$^\textrm{\scriptsize 83}$,
J.P.~Grohs$^\textrm{\scriptsize 44}$,
A.~Grohsjean$^\textrm{\scriptsize 42}$,
E.~Gross$^\textrm{\scriptsize 172}$,
J.~Grosse-Knetter$^\textrm{\scriptsize 54}$,
G.C.~Grossi$^\textrm{\scriptsize 79}$,
Z.J.~Grout$^\textrm{\scriptsize 149}$,
L.~Guan$^\textrm{\scriptsize 89}$,
J.~Guenther$^\textrm{\scriptsize 128}$,
F.~Guescini$^\textrm{\scriptsize 49}$,
D.~Guest$^\textrm{\scriptsize 163}$,
O.~Gueta$^\textrm{\scriptsize 153}$,
E.~Guido$^\textrm{\scriptsize 50a,50b}$,
T.~Guillemin$^\textrm{\scriptsize 5}$,
S.~Guindon$^\textrm{\scriptsize 2}$,
U.~Gul$^\textrm{\scriptsize 53}$,
C.~Gumpert$^\textrm{\scriptsize 30}$,
J.~Guo$^\textrm{\scriptsize 33e}$,
Y.~Guo$^\textrm{\scriptsize 33b}$$^{,o}$,
S.~Gupta$^\textrm{\scriptsize 120}$,
G.~Gustavino$^\textrm{\scriptsize 132a,132b}$,
P.~Gutierrez$^\textrm{\scriptsize 113}$,
N.G.~Gutierrez~Ortiz$^\textrm{\scriptsize 78}$,
C.~Gutschow$^\textrm{\scriptsize 44}$,
C.~Guyot$^\textrm{\scriptsize 136}$,
C.~Gwenlan$^\textrm{\scriptsize 120}$,
C.B.~Gwilliam$^\textrm{\scriptsize 74}$,
A.~Haas$^\textrm{\scriptsize 110}$,
C.~Haber$^\textrm{\scriptsize 15}$,
H.K.~Hadavand$^\textrm{\scriptsize 8}$,
N.~Haddad$^\textrm{\scriptsize 135e}$,
P.~Haefner$^\textrm{\scriptsize 21}$,
S.~Hageb\"ock$^\textrm{\scriptsize 21}$,
Z.~Hajduk$^\textrm{\scriptsize 39}$,
H.~Hakobyan$^\textrm{\scriptsize 177}$,
M.~Haleem$^\textrm{\scriptsize 42}$,
J.~Haley$^\textrm{\scriptsize 114}$,
D.~Hall$^\textrm{\scriptsize 120}$,
G.~Halladjian$^\textrm{\scriptsize 90}$,
G.D.~Hallewell$^\textrm{\scriptsize 85}$,
K.~Hamacher$^\textrm{\scriptsize 175}$,
P.~Hamal$^\textrm{\scriptsize 115}$,
K.~Hamano$^\textrm{\scriptsize 169}$,
A.~Hamilton$^\textrm{\scriptsize 145a}$,
G.N.~Hamity$^\textrm{\scriptsize 139}$,
P.G.~Hamnett$^\textrm{\scriptsize 42}$,
L.~Han$^\textrm{\scriptsize 33b}$,
K.~Hanagaki$^\textrm{\scriptsize 66}$$^{,r}$,
K.~Hanawa$^\textrm{\scriptsize 155}$,
M.~Hance$^\textrm{\scriptsize 137}$,
B.~Haney$^\textrm{\scriptsize 122}$,
P.~Hanke$^\textrm{\scriptsize 58a}$,
R.~Hanna$^\textrm{\scriptsize 136}$,
J.B.~Hansen$^\textrm{\scriptsize 36}$,
J.D.~Hansen$^\textrm{\scriptsize 36}$,
M.C.~Hansen$^\textrm{\scriptsize 21}$,
P.H.~Hansen$^\textrm{\scriptsize 36}$,
K.~Hara$^\textrm{\scriptsize 160}$,
A.S.~Hard$^\textrm{\scriptsize 173}$,
T.~Harenberg$^\textrm{\scriptsize 175}$,
F.~Hariri$^\textrm{\scriptsize 117}$,
S.~Harkusha$^\textrm{\scriptsize 92}$,
R.D.~Harrington$^\textrm{\scriptsize 46}$,
P.F.~Harrison$^\textrm{\scriptsize 170}$,
F.~Hartjes$^\textrm{\scriptsize 107}$,
M.~Hasegawa$^\textrm{\scriptsize 67}$,
Y.~Hasegawa$^\textrm{\scriptsize 140}$,
A.~Hasib$^\textrm{\scriptsize 113}$,
S.~Hassani$^\textrm{\scriptsize 136}$,
S.~Haug$^\textrm{\scriptsize 17}$,
R.~Hauser$^\textrm{\scriptsize 90}$,
L.~Hauswald$^\textrm{\scriptsize 44}$,
M.~Havranek$^\textrm{\scriptsize 127}$,
C.M.~Hawkes$^\textrm{\scriptsize 18}$,
R.J.~Hawkings$^\textrm{\scriptsize 30}$,
A.D.~Hawkins$^\textrm{\scriptsize 81}$,
T.~Hayashi$^\textrm{\scriptsize 160}$,
D.~Hayden$^\textrm{\scriptsize 90}$,
C.P.~Hays$^\textrm{\scriptsize 120}$,
J.M.~Hays$^\textrm{\scriptsize 76}$,
H.S.~Hayward$^\textrm{\scriptsize 74}$,
S.J.~Haywood$^\textrm{\scriptsize 131}$,
S.J.~Head$^\textrm{\scriptsize 18}$,
T.~Heck$^\textrm{\scriptsize 83}$,
V.~Hedberg$^\textrm{\scriptsize 81}$,
L.~Heelan$^\textrm{\scriptsize 8}$,
S.~Heim$^\textrm{\scriptsize 122}$,
T.~Heim$^\textrm{\scriptsize 15}$,
B.~Heinemann$^\textrm{\scriptsize 15}$,
L.~Heinrich$^\textrm{\scriptsize 110}$,
J.~Hejbal$^\textrm{\scriptsize 127}$,
L.~Helary$^\textrm{\scriptsize 22}$,
S.~Hellman$^\textrm{\scriptsize 146a,146b}$,
C.~Helsens$^\textrm{\scriptsize 30}$,
J.~Henderson$^\textrm{\scriptsize 120}$,
R.C.W.~Henderson$^\textrm{\scriptsize 72}$,
Y.~Heng$^\textrm{\scriptsize 173}$,
S.~Henkelmann$^\textrm{\scriptsize 168}$,
A.M.~Henriques~Correia$^\textrm{\scriptsize 30}$,
S.~Henrot-Versille$^\textrm{\scriptsize 117}$,
G.H.~Herbert$^\textrm{\scriptsize 16}$,
Y.~Hern\'andez~Jim\'enez$^\textrm{\scriptsize 167}$,
G.~Herten$^\textrm{\scriptsize 48}$,
R.~Hertenberger$^\textrm{\scriptsize 100}$,
L.~Hervas$^\textrm{\scriptsize 30}$,
G.G.~Hesketh$^\textrm{\scriptsize 78}$,
N.P.~Hessey$^\textrm{\scriptsize 107}$,
J.W.~Hetherly$^\textrm{\scriptsize 40}$,
R.~Hickling$^\textrm{\scriptsize 76}$,
E.~Hig\'on-Rodriguez$^\textrm{\scriptsize 167}$,
E.~Hill$^\textrm{\scriptsize 169}$,
J.C.~Hill$^\textrm{\scriptsize 28}$,
K.H.~Hiller$^\textrm{\scriptsize 42}$,
S.J.~Hillier$^\textrm{\scriptsize 18}$,
I.~Hinchliffe$^\textrm{\scriptsize 15}$,
E.~Hines$^\textrm{\scriptsize 122}$,
R.R.~Hinman$^\textrm{\scriptsize 15}$,
M.~Hirose$^\textrm{\scriptsize 157}$,
D.~Hirschbuehl$^\textrm{\scriptsize 175}$,
J.~Hobbs$^\textrm{\scriptsize 148}$,
N.~Hod$^\textrm{\scriptsize 107}$,
M.C.~Hodgkinson$^\textrm{\scriptsize 139}$,
P.~Hodgson$^\textrm{\scriptsize 139}$,
A.~Hoecker$^\textrm{\scriptsize 30}$,
M.R.~Hoeferkamp$^\textrm{\scriptsize 105}$,
F.~Hoenig$^\textrm{\scriptsize 100}$,
M.~Hohlfeld$^\textrm{\scriptsize 83}$,
D.~Hohn$^\textrm{\scriptsize 21}$,
T.R.~Holmes$^\textrm{\scriptsize 15}$,
M.~Homann$^\textrm{\scriptsize 43}$,
T.M.~Hong$^\textrm{\scriptsize 125}$,
B.H.~Hooberman$^\textrm{\scriptsize 165}$,
W.H.~Hopkins$^\textrm{\scriptsize 116}$,
Y.~Horii$^\textrm{\scriptsize 103}$,
A.J.~Horton$^\textrm{\scriptsize 142}$,
J-Y.~Hostachy$^\textrm{\scriptsize 55}$,
S.~Hou$^\textrm{\scriptsize 151}$,
A.~Hoummada$^\textrm{\scriptsize 135a}$,
J.~Howard$^\textrm{\scriptsize 120}$,
J.~Howarth$^\textrm{\scriptsize 42}$,
M.~Hrabovsky$^\textrm{\scriptsize 115}$,
I.~Hristova$^\textrm{\scriptsize 16}$,
J.~Hrivnac$^\textrm{\scriptsize 117}$,
T.~Hryn'ova$^\textrm{\scriptsize 5}$,
A.~Hrynevich$^\textrm{\scriptsize 93}$,
C.~Hsu$^\textrm{\scriptsize 145c}$,
P.J.~Hsu$^\textrm{\scriptsize 151}$$^{,s}$,
S.-C.~Hsu$^\textrm{\scriptsize 138}$,
D.~Hu$^\textrm{\scriptsize 35}$,
Q.~Hu$^\textrm{\scriptsize 33b}$,
Y.~Huang$^\textrm{\scriptsize 42}$,
Z.~Hubacek$^\textrm{\scriptsize 128}$,
F.~Hubaut$^\textrm{\scriptsize 85}$,
F.~Huegging$^\textrm{\scriptsize 21}$,
T.B.~Huffman$^\textrm{\scriptsize 120}$,
E.W.~Hughes$^\textrm{\scriptsize 35}$,
G.~Hughes$^\textrm{\scriptsize 72}$,
M.~Huhtinen$^\textrm{\scriptsize 30}$,
T.A.~H\"ulsing$^\textrm{\scriptsize 83}$,
N.~Huseynov$^\textrm{\scriptsize 65}$$^{,b}$,
J.~Huston$^\textrm{\scriptsize 90}$,
J.~Huth$^\textrm{\scriptsize 57}$,
G.~Iacobucci$^\textrm{\scriptsize 49}$,
G.~Iakovidis$^\textrm{\scriptsize 25}$,
I.~Ibragimov$^\textrm{\scriptsize 141}$,
L.~Iconomidou-Fayard$^\textrm{\scriptsize 117}$,
E.~Ideal$^\textrm{\scriptsize 176}$,
Z.~Idrissi$^\textrm{\scriptsize 135e}$,
P.~Iengo$^\textrm{\scriptsize 30}$,
O.~Igonkina$^\textrm{\scriptsize 107}$,
T.~Iizawa$^\textrm{\scriptsize 171}$,
Y.~Ikegami$^\textrm{\scriptsize 66}$,
M.~Ikeno$^\textrm{\scriptsize 66}$,
Y.~Ilchenko$^\textrm{\scriptsize 31}$$^{,t}$,
D.~Iliadis$^\textrm{\scriptsize 154}$,
N.~Ilic$^\textrm{\scriptsize 143}$,
T.~Ince$^\textrm{\scriptsize 101}$,
G.~Introzzi$^\textrm{\scriptsize 121a,121b}$,
P.~Ioannou$^\textrm{\scriptsize 9}$,
M.~Iodice$^\textrm{\scriptsize 134a}$,
K.~Iordanidou$^\textrm{\scriptsize 35}$,
V.~Ippolito$^\textrm{\scriptsize 57}$,
A.~Irles~Quiles$^\textrm{\scriptsize 167}$,
C.~Isaksson$^\textrm{\scriptsize 166}$,
M.~Ishino$^\textrm{\scriptsize 68}$,
M.~Ishitsuka$^\textrm{\scriptsize 157}$,
R.~Ishmukhametov$^\textrm{\scriptsize 111}$,
C.~Issever$^\textrm{\scriptsize 120}$,
S.~Istin$^\textrm{\scriptsize 19a}$,
J.M.~Iturbe~Ponce$^\textrm{\scriptsize 84}$,
R.~Iuppa$^\textrm{\scriptsize 133a,133b}$,
J.~Ivarsson$^\textrm{\scriptsize 81}$,
W.~Iwanski$^\textrm{\scriptsize 39}$,
H.~Iwasaki$^\textrm{\scriptsize 66}$,
J.M.~Izen$^\textrm{\scriptsize 41}$,
V.~Izzo$^\textrm{\scriptsize 104a}$,
S.~Jabbar$^\textrm{\scriptsize 3}$,
B.~Jackson$^\textrm{\scriptsize 122}$,
M.~Jackson$^\textrm{\scriptsize 74}$,
P.~Jackson$^\textrm{\scriptsize 1}$,
M.R.~Jaekel$^\textrm{\scriptsize 30}$,
V.~Jain$^\textrm{\scriptsize 2}$,
K.B.~Jakobi$^\textrm{\scriptsize 83}$,
K.~Jakobs$^\textrm{\scriptsize 48}$,
S.~Jakobsen$^\textrm{\scriptsize 30}$,
T.~Jakoubek$^\textrm{\scriptsize 127}$,
J.~Jakubek$^\textrm{\scriptsize 128}$,
D.O.~Jamin$^\textrm{\scriptsize 114}$,
D.K.~Jana$^\textrm{\scriptsize 79}$,
E.~Jansen$^\textrm{\scriptsize 78}$,
R.~Jansky$^\textrm{\scriptsize 62}$,
J.~Janssen$^\textrm{\scriptsize 21}$,
M.~Janus$^\textrm{\scriptsize 54}$,
G.~Jarlskog$^\textrm{\scriptsize 81}$,
N.~Javadov$^\textrm{\scriptsize 65}$$^{,b}$,
T.~Jav\r{u}rek$^\textrm{\scriptsize 48}$,
F.~Jeanneau$^\textrm{\scriptsize 136}$,
L.~Jeanty$^\textrm{\scriptsize 15}$,
J.~Jejelava$^\textrm{\scriptsize 51a}$$^{,u}$,
G.-Y.~Jeng$^\textrm{\scriptsize 150}$,
D.~Jennens$^\textrm{\scriptsize 88}$,
P.~Jenni$^\textrm{\scriptsize 48}$$^{,v}$,
J.~Jentzsch$^\textrm{\scriptsize 43}$,
C.~Jeske$^\textrm{\scriptsize 170}$,
S.~J\'ez\'equel$^\textrm{\scriptsize 5}$,
H.~Ji$^\textrm{\scriptsize 173}$,
J.~Jia$^\textrm{\scriptsize 148}$,
H.~Jiang$^\textrm{\scriptsize 64}$,
Y.~Jiang$^\textrm{\scriptsize 33b}$,
S.~Jiggins$^\textrm{\scriptsize 78}$,
J.~Jimenez~Pena$^\textrm{\scriptsize 167}$,
S.~Jin$^\textrm{\scriptsize 33a}$,
A.~Jinaru$^\textrm{\scriptsize 26b}$,
O.~Jinnouchi$^\textrm{\scriptsize 157}$,
P.~Johansson$^\textrm{\scriptsize 139}$,
K.A.~Johns$^\textrm{\scriptsize 7}$,
W.J.~Johnson$^\textrm{\scriptsize 138}$,
K.~Jon-And$^\textrm{\scriptsize 146a,146b}$,
G.~Jones$^\textrm{\scriptsize 170}$,
R.W.L.~Jones$^\textrm{\scriptsize 72}$,
T.J.~Jones$^\textrm{\scriptsize 74}$,
J.~Jongmanns$^\textrm{\scriptsize 58a}$,
P.M.~Jorge$^\textrm{\scriptsize 126a,126b}$,
K.D.~Joshi$^\textrm{\scriptsize 84}$,
J.~Jovicevic$^\textrm{\scriptsize 159a}$,
X.~Ju$^\textrm{\scriptsize 173}$,
A.~Juste~Rozas$^\textrm{\scriptsize 12}$$^{,q}$,
M.K.~K\"{o}hler$^\textrm{\scriptsize 172}$,
M.~Kaci$^\textrm{\scriptsize 167}$,
A.~Kaczmarska$^\textrm{\scriptsize 39}$,
M.~Kado$^\textrm{\scriptsize 117}$,
H.~Kagan$^\textrm{\scriptsize 111}$,
M.~Kagan$^\textrm{\scriptsize 143}$,
S.J.~Kahn$^\textrm{\scriptsize 85}$,
E.~Kajomovitz$^\textrm{\scriptsize 45}$,
C.W.~Kalderon$^\textrm{\scriptsize 120}$,
A.~Kaluza$^\textrm{\scriptsize 83}$,
S.~Kama$^\textrm{\scriptsize 40}$,
A.~Kamenshchikov$^\textrm{\scriptsize 130}$,
N.~Kanaya$^\textrm{\scriptsize 155}$,
S.~Kaneti$^\textrm{\scriptsize 28}$,
V.A.~Kantserov$^\textrm{\scriptsize 98}$,
J.~Kanzaki$^\textrm{\scriptsize 66}$,
B.~Kaplan$^\textrm{\scriptsize 110}$,
L.S.~Kaplan$^\textrm{\scriptsize 173}$,
A.~Kapliy$^\textrm{\scriptsize 31}$,
D.~Kar$^\textrm{\scriptsize 145c}$,
K.~Karakostas$^\textrm{\scriptsize 10}$,
A.~Karamaoun$^\textrm{\scriptsize 3}$,
N.~Karastathis$^\textrm{\scriptsize 10,107}$,
M.J.~Kareem$^\textrm{\scriptsize 54}$,
E.~Karentzos$^\textrm{\scriptsize 10}$,
M.~Karnevskiy$^\textrm{\scriptsize 83}$,
S.N.~Karpov$^\textrm{\scriptsize 65}$,
Z.M.~Karpova$^\textrm{\scriptsize 65}$,
K.~Karthik$^\textrm{\scriptsize 110}$,
V.~Kartvelishvili$^\textrm{\scriptsize 72}$,
A.N.~Karyukhin$^\textrm{\scriptsize 130}$,
K.~Kasahara$^\textrm{\scriptsize 160}$,
L.~Kashif$^\textrm{\scriptsize 173}$,
R.D.~Kass$^\textrm{\scriptsize 111}$,
A.~Kastanas$^\textrm{\scriptsize 14}$,
Y.~Kataoka$^\textrm{\scriptsize 155}$,
C.~Kato$^\textrm{\scriptsize 155}$,
A.~Katre$^\textrm{\scriptsize 49}$,
J.~Katzy$^\textrm{\scriptsize 42}$,
K.~Kawade$^\textrm{\scriptsize 103}$,
K.~Kawagoe$^\textrm{\scriptsize 70}$,
T.~Kawamoto$^\textrm{\scriptsize 155}$,
G.~Kawamura$^\textrm{\scriptsize 54}$,
S.~Kazama$^\textrm{\scriptsize 155}$,
V.F.~Kazanin$^\textrm{\scriptsize 109}$$^{,c}$,
R.~Keeler$^\textrm{\scriptsize 169}$,
R.~Kehoe$^\textrm{\scriptsize 40}$,
J.S.~Keller$^\textrm{\scriptsize 42}$,
J.J.~Kempster$^\textrm{\scriptsize 77}$,
H.~Keoshkerian$^\textrm{\scriptsize 84}$,
O.~Kepka$^\textrm{\scriptsize 127}$,
B.P.~Ker\v{s}evan$^\textrm{\scriptsize 75}$,
S.~Kersten$^\textrm{\scriptsize 175}$,
R.A.~Keyes$^\textrm{\scriptsize 87}$,
F.~Khalil-zada$^\textrm{\scriptsize 11}$,
H.~Khandanyan$^\textrm{\scriptsize 146a,146b}$,
A.~Khanov$^\textrm{\scriptsize 114}$,
A.G.~Kharlamov$^\textrm{\scriptsize 109}$$^{,c}$,
T.J.~Khoo$^\textrm{\scriptsize 28}$,
V.~Khovanskiy$^\textrm{\scriptsize 97}$,
E.~Khramov$^\textrm{\scriptsize 65}$,
J.~Khubua$^\textrm{\scriptsize 51b}$$^{,w}$,
S.~Kido$^\textrm{\scriptsize 67}$,
H.Y.~Kim$^\textrm{\scriptsize 8}$,
S.H.~Kim$^\textrm{\scriptsize 160}$,
Y.K.~Kim$^\textrm{\scriptsize 31}$,
N.~Kimura$^\textrm{\scriptsize 154}$,
O.M.~Kind$^\textrm{\scriptsize 16}$,
B.T.~King$^\textrm{\scriptsize 74}$,
M.~King$^\textrm{\scriptsize 167}$,
S.B.~King$^\textrm{\scriptsize 168}$,
J.~Kirk$^\textrm{\scriptsize 131}$,
A.E.~Kiryunin$^\textrm{\scriptsize 101}$,
T.~Kishimoto$^\textrm{\scriptsize 67}$,
D.~Kisielewska$^\textrm{\scriptsize 38a}$,
F.~Kiss$^\textrm{\scriptsize 48}$,
K.~Kiuchi$^\textrm{\scriptsize 160}$,
O.~Kivernyk$^\textrm{\scriptsize 136}$,
E.~Kladiva$^\textrm{\scriptsize 144b}$,
M.H.~Klein$^\textrm{\scriptsize 35}$,
M.~Klein$^\textrm{\scriptsize 74}$,
U.~Klein$^\textrm{\scriptsize 74}$,
K.~Kleinknecht$^\textrm{\scriptsize 83}$,
P.~Klimek$^\textrm{\scriptsize 146a,146b}$,
A.~Klimentov$^\textrm{\scriptsize 25}$,
R.~Klingenberg$^\textrm{\scriptsize 43}$,
J.A.~Klinger$^\textrm{\scriptsize 139}$,
T.~Klioutchnikova$^\textrm{\scriptsize 30}$,
E.-E.~Kluge$^\textrm{\scriptsize 58a}$,
P.~Kluit$^\textrm{\scriptsize 107}$,
S.~Kluth$^\textrm{\scriptsize 101}$,
J.~Knapik$^\textrm{\scriptsize 39}$,
E.~Kneringer$^\textrm{\scriptsize 62}$,
E.B.F.G.~Knoops$^\textrm{\scriptsize 85}$,
A.~Knue$^\textrm{\scriptsize 53}$,
A.~Kobayashi$^\textrm{\scriptsize 155}$,
D.~Kobayashi$^\textrm{\scriptsize 157}$,
T.~Kobayashi$^\textrm{\scriptsize 155}$,
M.~Kobel$^\textrm{\scriptsize 44}$,
M.~Kocian$^\textrm{\scriptsize 143}$,
P.~Kodys$^\textrm{\scriptsize 129}$,
T.~Koffas$^\textrm{\scriptsize 29}$,
E.~Koffeman$^\textrm{\scriptsize 107}$,
L.A.~Kogan$^\textrm{\scriptsize 120}$,
S.~Kohlmann$^\textrm{\scriptsize 175}$,
Z.~Kohout$^\textrm{\scriptsize 128}$,
T.~Kohriki$^\textrm{\scriptsize 66}$,
T.~Koi$^\textrm{\scriptsize 143}$,
H.~Kolanoski$^\textrm{\scriptsize 16}$,
M.~Kolb$^\textrm{\scriptsize 58b}$,
I.~Koletsou$^\textrm{\scriptsize 5}$,
A.A.~Komar$^\textrm{\scriptsize 96}$$^{,*}$,
Y.~Komori$^\textrm{\scriptsize 155}$,
T.~Kondo$^\textrm{\scriptsize 66}$,
N.~Kondrashova$^\textrm{\scriptsize 42}$,
K.~K\"oneke$^\textrm{\scriptsize 48}$,
A.C.~K\"onig$^\textrm{\scriptsize 106}$,
T.~Kono$^\textrm{\scriptsize 66}$$^{,x}$,
R.~Konoplich$^\textrm{\scriptsize 110}$$^{,y}$,
N.~Konstantinidis$^\textrm{\scriptsize 78}$,
R.~Kopeliansky$^\textrm{\scriptsize 152}$,
S.~Koperny$^\textrm{\scriptsize 38a}$,
L.~K\"opke$^\textrm{\scriptsize 83}$,
A.K.~Kopp$^\textrm{\scriptsize 48}$,
K.~Korcyl$^\textrm{\scriptsize 39}$,
K.~Kordas$^\textrm{\scriptsize 154}$,
A.~Korn$^\textrm{\scriptsize 78}$,
A.A.~Korol$^\textrm{\scriptsize 109}$$^{,c}$,
I.~Korolkov$^\textrm{\scriptsize 12}$,
E.V.~Korolkova$^\textrm{\scriptsize 139}$,
O.~Kortner$^\textrm{\scriptsize 101}$,
S.~Kortner$^\textrm{\scriptsize 101}$,
T.~Kosek$^\textrm{\scriptsize 129}$,
V.V.~Kostyukhin$^\textrm{\scriptsize 21}$,
V.M.~Kotov$^\textrm{\scriptsize 65}$,
A.~Kotwal$^\textrm{\scriptsize 45}$,
A.~Kourkoumeli-Charalampidi$^\textrm{\scriptsize 154}$,
C.~Kourkoumelis$^\textrm{\scriptsize 9}$,
V.~Kouskoura$^\textrm{\scriptsize 25}$,
A.~Koutsman$^\textrm{\scriptsize 159a}$,
R.~Kowalewski$^\textrm{\scriptsize 169}$,
T.Z.~Kowalski$^\textrm{\scriptsize 38a}$,
W.~Kozanecki$^\textrm{\scriptsize 136}$,
A.S.~Kozhin$^\textrm{\scriptsize 130}$,
V.A.~Kramarenko$^\textrm{\scriptsize 99}$,
G.~Kramberger$^\textrm{\scriptsize 75}$,
D.~Krasnopevtsev$^\textrm{\scriptsize 98}$,
M.W.~Krasny$^\textrm{\scriptsize 80}$,
A.~Krasznahorkay$^\textrm{\scriptsize 30}$,
J.K.~Kraus$^\textrm{\scriptsize 21}$,
A.~Kravchenko$^\textrm{\scriptsize 25}$,
M.~Kretz$^\textrm{\scriptsize 58c}$,
J.~Kretzschmar$^\textrm{\scriptsize 74}$,
K.~Kreutzfeldt$^\textrm{\scriptsize 52}$,
P.~Krieger$^\textrm{\scriptsize 158}$,
K.~Krizka$^\textrm{\scriptsize 31}$,
K.~Kroeninger$^\textrm{\scriptsize 43}$,
H.~Kroha$^\textrm{\scriptsize 101}$,
J.~Kroll$^\textrm{\scriptsize 122}$,
J.~Kroseberg$^\textrm{\scriptsize 21}$,
J.~Krstic$^\textrm{\scriptsize 13}$,
U.~Kruchonak$^\textrm{\scriptsize 65}$,
H.~Kr\"uger$^\textrm{\scriptsize 21}$,
N.~Krumnack$^\textrm{\scriptsize 64}$,
A.~Kruse$^\textrm{\scriptsize 173}$,
M.C.~Kruse$^\textrm{\scriptsize 45}$,
M.~Kruskal$^\textrm{\scriptsize 22}$,
T.~Kubota$^\textrm{\scriptsize 88}$,
H.~Kucuk$^\textrm{\scriptsize 78}$,
S.~Kuday$^\textrm{\scriptsize 4b}$,
S.~Kuehn$^\textrm{\scriptsize 48}$,
A.~Kugel$^\textrm{\scriptsize 58c}$,
F.~Kuger$^\textrm{\scriptsize 174}$,
A.~Kuhl$^\textrm{\scriptsize 137}$,
T.~Kuhl$^\textrm{\scriptsize 42}$,
V.~Kukhtin$^\textrm{\scriptsize 65}$,
R.~Kukla$^\textrm{\scriptsize 136}$,
Y.~Kulchitsky$^\textrm{\scriptsize 92}$,
S.~Kuleshov$^\textrm{\scriptsize 32b}$,
M.~Kuna$^\textrm{\scriptsize 132a,132b}$,
T.~Kunigo$^\textrm{\scriptsize 68}$,
A.~Kupco$^\textrm{\scriptsize 127}$,
H.~Kurashige$^\textrm{\scriptsize 67}$,
Y.A.~Kurochkin$^\textrm{\scriptsize 92}$,
V.~Kus$^\textrm{\scriptsize 127}$,
E.S.~Kuwertz$^\textrm{\scriptsize 169}$,
M.~Kuze$^\textrm{\scriptsize 157}$,
J.~Kvita$^\textrm{\scriptsize 115}$,
T.~Kwan$^\textrm{\scriptsize 169}$,
D.~Kyriazopoulos$^\textrm{\scriptsize 139}$,
A.~La~Rosa$^\textrm{\scriptsize 137}$,
J.L.~La~Rosa~Navarro$^\textrm{\scriptsize 24d}$,
L.~La~Rotonda$^\textrm{\scriptsize 37a,37b}$,
C.~Lacasta$^\textrm{\scriptsize 167}$,
F.~Lacava$^\textrm{\scriptsize 132a,132b}$,
J.~Lacey$^\textrm{\scriptsize 29}$,
H.~Lacker$^\textrm{\scriptsize 16}$,
D.~Lacour$^\textrm{\scriptsize 80}$,
V.R.~Lacuesta$^\textrm{\scriptsize 167}$,
E.~Ladygin$^\textrm{\scriptsize 65}$,
R.~Lafaye$^\textrm{\scriptsize 5}$,
B.~Laforge$^\textrm{\scriptsize 80}$,
T.~Lagouri$^\textrm{\scriptsize 176}$,
S.~Lai$^\textrm{\scriptsize 54}$,
L.~Lambourne$^\textrm{\scriptsize 78}$,
S.~Lammers$^\textrm{\scriptsize 61}$,
C.L.~Lampen$^\textrm{\scriptsize 7}$,
W.~Lampl$^\textrm{\scriptsize 7}$,
E.~Lan\c{c}on$^\textrm{\scriptsize 136}$,
U.~Landgraf$^\textrm{\scriptsize 48}$,
M.P.J.~Landon$^\textrm{\scriptsize 76}$,
V.S.~Lang$^\textrm{\scriptsize 58a}$,
J.C.~Lange$^\textrm{\scriptsize 12}$,
A.J.~Lankford$^\textrm{\scriptsize 163}$,
F.~Lanni$^\textrm{\scriptsize 25}$,
K.~Lantzsch$^\textrm{\scriptsize 21}$,
A.~Lanza$^\textrm{\scriptsize 121a}$,
S.~Laplace$^\textrm{\scriptsize 80}$,
C.~Lapoire$^\textrm{\scriptsize 30}$,
J.F.~Laporte$^\textrm{\scriptsize 136}$,
T.~Lari$^\textrm{\scriptsize 91a}$,
F.~Lasagni~Manghi$^\textrm{\scriptsize 20a,20b}$,
M.~Lassnig$^\textrm{\scriptsize 30}$,
P.~Laurelli$^\textrm{\scriptsize 47}$,
W.~Lavrijsen$^\textrm{\scriptsize 15}$,
A.T.~Law$^\textrm{\scriptsize 137}$,
P.~Laycock$^\textrm{\scriptsize 74}$,
T.~Lazovich$^\textrm{\scriptsize 57}$,
O.~Le~Dortz$^\textrm{\scriptsize 80}$,
E.~Le~Guirriec$^\textrm{\scriptsize 85}$,
E.~Le~Menedeu$^\textrm{\scriptsize 12}$,
M.~LeBlanc$^\textrm{\scriptsize 169}$,
T.~LeCompte$^\textrm{\scriptsize 6}$,
F.~Ledroit-Guillon$^\textrm{\scriptsize 55}$,
C.A.~Lee$^\textrm{\scriptsize 145a}$,
S.C.~Lee$^\textrm{\scriptsize 151}$,
L.~Lee$^\textrm{\scriptsize 1}$,
G.~Lefebvre$^\textrm{\scriptsize 80}$,
M.~Lefebvre$^\textrm{\scriptsize 169}$,
F.~Legger$^\textrm{\scriptsize 100}$,
C.~Leggett$^\textrm{\scriptsize 15}$,
A.~Lehan$^\textrm{\scriptsize 74}$,
G.~Lehmann~Miotto$^\textrm{\scriptsize 30}$,
X.~Lei$^\textrm{\scriptsize 7}$,
W.A.~Leight$^\textrm{\scriptsize 29}$,
A.~Leisos$^\textrm{\scriptsize 154}$$^{,z}$,
A.G.~Leister$^\textrm{\scriptsize 176}$,
M.A.L.~Leite$^\textrm{\scriptsize 24d}$,
R.~Leitner$^\textrm{\scriptsize 129}$,
D.~Lellouch$^\textrm{\scriptsize 172}$,
B.~Lemmer$^\textrm{\scriptsize 54}$,
K.J.C.~Leney$^\textrm{\scriptsize 78}$,
T.~Lenz$^\textrm{\scriptsize 21}$,
B.~Lenzi$^\textrm{\scriptsize 30}$,
R.~Leone$^\textrm{\scriptsize 7}$,
S.~Leone$^\textrm{\scriptsize 124a,124b}$,
C.~Leonidopoulos$^\textrm{\scriptsize 46}$,
S.~Leontsinis$^\textrm{\scriptsize 10}$,
C.~Leroy$^\textrm{\scriptsize 95}$,
C.G.~Lester$^\textrm{\scriptsize 28}$,
M.~Levchenko$^\textrm{\scriptsize 123}$,
J.~Lev\^eque$^\textrm{\scriptsize 5}$,
D.~Levin$^\textrm{\scriptsize 89}$,
L.J.~Levinson$^\textrm{\scriptsize 172}$,
M.~Levy$^\textrm{\scriptsize 18}$,
A.~Lewis$^\textrm{\scriptsize 120}$,
A.M.~Leyko$^\textrm{\scriptsize 21}$,
M.~Leyton$^\textrm{\scriptsize 41}$,
B.~Li$^\textrm{\scriptsize 33b}$$^{,aa}$,
H.~Li$^\textrm{\scriptsize 148}$,
H.L.~Li$^\textrm{\scriptsize 31}$,
L.~Li$^\textrm{\scriptsize 45}$,
L.~Li$^\textrm{\scriptsize 33e}$,
S.~Li$^\textrm{\scriptsize 45}$,
X.~Li$^\textrm{\scriptsize 84}$,
Y.~Li$^\textrm{\scriptsize 33c}$$^{,ab}$,
Z.~Liang$^\textrm{\scriptsize 137}$,
H.~Liao$^\textrm{\scriptsize 34}$,
B.~Liberti$^\textrm{\scriptsize 133a}$,
A.~Liblong$^\textrm{\scriptsize 158}$,
P.~Lichard$^\textrm{\scriptsize 30}$,
K.~Lie$^\textrm{\scriptsize 165}$,
J.~Liebal$^\textrm{\scriptsize 21}$,
W.~Liebig$^\textrm{\scriptsize 14}$,
C.~Limbach$^\textrm{\scriptsize 21}$,
A.~Limosani$^\textrm{\scriptsize 150}$,
S.C.~Lin$^\textrm{\scriptsize 151}$$^{,ac}$,
T.H.~Lin$^\textrm{\scriptsize 83}$,
B.E.~Lindquist$^\textrm{\scriptsize 148}$,
J.T.~Linnemann$^\textrm{\scriptsize 90}$,
E.~Lipeles$^\textrm{\scriptsize 122}$,
A.~Lipniacka$^\textrm{\scriptsize 14}$,
M.~Lisovyi$^\textrm{\scriptsize 58b}$,
T.M.~Liss$^\textrm{\scriptsize 165}$,
D.~Lissauer$^\textrm{\scriptsize 25}$,
A.~Lister$^\textrm{\scriptsize 168}$,
A.M.~Litke$^\textrm{\scriptsize 137}$,
B.~Liu$^\textrm{\scriptsize 151}$$^{,ad}$,
D.~Liu$^\textrm{\scriptsize 151}$,
H.~Liu$^\textrm{\scriptsize 89}$,
J.~Liu$^\textrm{\scriptsize 85}$,
J.B.~Liu$^\textrm{\scriptsize 33b}$,
K.~Liu$^\textrm{\scriptsize 85}$,
L.~Liu$^\textrm{\scriptsize 165}$,
M.~Liu$^\textrm{\scriptsize 45}$,
M.~Liu$^\textrm{\scriptsize 33b}$,
Y.~Liu$^\textrm{\scriptsize 33b}$,
M.~Livan$^\textrm{\scriptsize 121a,121b}$,
A.~Lleres$^\textrm{\scriptsize 55}$,
J.~Llorente~Merino$^\textrm{\scriptsize 82}$,
S.L.~Lloyd$^\textrm{\scriptsize 76}$,
F.~Lo~Sterzo$^\textrm{\scriptsize 151}$,
E.~Lobodzinska$^\textrm{\scriptsize 42}$,
P.~Loch$^\textrm{\scriptsize 7}$,
W.S.~Lockman$^\textrm{\scriptsize 137}$,
F.K.~Loebinger$^\textrm{\scriptsize 84}$,
A.E.~Loevschall-Jensen$^\textrm{\scriptsize 36}$,
K.M.~Loew$^\textrm{\scriptsize 23}$,
A.~Loginov$^\textrm{\scriptsize 176}$,
T.~Lohse$^\textrm{\scriptsize 16}$,
K.~Lohwasser$^\textrm{\scriptsize 42}$,
M.~Lokajicek$^\textrm{\scriptsize 127}$,
B.A.~Long$^\textrm{\scriptsize 22}$,
J.D.~Long$^\textrm{\scriptsize 165}$,
R.E.~Long$^\textrm{\scriptsize 72}$,
K.A.~Looper$^\textrm{\scriptsize 111}$,
L.~Lopes$^\textrm{\scriptsize 126a}$,
D.~Lopez~Mateos$^\textrm{\scriptsize 57}$,
B.~Lopez~Paredes$^\textrm{\scriptsize 139}$,
I.~Lopez~Paz$^\textrm{\scriptsize 12}$,
J.~Lorenz$^\textrm{\scriptsize 100}$,
N.~Lorenzo~Martinez$^\textrm{\scriptsize 61}$,
M.~Losada$^\textrm{\scriptsize 162}$,
P.J.~L{\"o}sel$^\textrm{\scriptsize 100}$,
X.~Lou$^\textrm{\scriptsize 33a}$,
A.~Lounis$^\textrm{\scriptsize 117}$,
J.~Love$^\textrm{\scriptsize 6}$,
P.A.~Love$^\textrm{\scriptsize 72}$,
H.~Lu$^\textrm{\scriptsize 60a}$,
N.~Lu$^\textrm{\scriptsize 89}$,
H.J.~Lubatti$^\textrm{\scriptsize 138}$,
C.~Luci$^\textrm{\scriptsize 132a,132b}$,
A.~Lucotte$^\textrm{\scriptsize 55}$,
C.~Luedtke$^\textrm{\scriptsize 48}$,
F.~Luehring$^\textrm{\scriptsize 61}$,
W.~Lukas$^\textrm{\scriptsize 62}$,
L.~Luminari$^\textrm{\scriptsize 132a}$,
O.~Lundberg$^\textrm{\scriptsize 146a,146b}$,
B.~Lund-Jensen$^\textrm{\scriptsize 147}$,
D.~Lynn$^\textrm{\scriptsize 25}$,
R.~Lysak$^\textrm{\scriptsize 127}$,
E.~Lytken$^\textrm{\scriptsize 81}$,
H.~Ma$^\textrm{\scriptsize 25}$,
L.L.~Ma$^\textrm{\scriptsize 33d}$,
G.~Maccarrone$^\textrm{\scriptsize 47}$,
A.~Macchiolo$^\textrm{\scriptsize 101}$,
C.M.~Macdonald$^\textrm{\scriptsize 139}$,
B.~Ma\v{c}ek$^\textrm{\scriptsize 75}$,
J.~Machado~Miguens$^\textrm{\scriptsize 122,126b}$,
D.~Macina$^\textrm{\scriptsize 30}$,
D.~Madaffari$^\textrm{\scriptsize 85}$,
R.~Madar$^\textrm{\scriptsize 34}$,
H.J.~Maddocks$^\textrm{\scriptsize 72}$,
W.F.~Mader$^\textrm{\scriptsize 44}$,
A.~Madsen$^\textrm{\scriptsize 42}$,
J.~Maeda$^\textrm{\scriptsize 67}$,
S.~Maeland$^\textrm{\scriptsize 14}$,
T.~Maeno$^\textrm{\scriptsize 25}$,
A.~Maevskiy$^\textrm{\scriptsize 99}$,
E.~Magradze$^\textrm{\scriptsize 54}$,
K.~Mahboubi$^\textrm{\scriptsize 48}$,
J.~Mahlstedt$^\textrm{\scriptsize 107}$,
C.~Maiani$^\textrm{\scriptsize 136}$,
C.~Maidantchik$^\textrm{\scriptsize 24a}$,
A.A.~Maier$^\textrm{\scriptsize 101}$,
T.~Maier$^\textrm{\scriptsize 100}$,
A.~Maio$^\textrm{\scriptsize 126a,126b,126d}$,
S.~Majewski$^\textrm{\scriptsize 116}$,
Y.~Makida$^\textrm{\scriptsize 66}$,
N.~Makovec$^\textrm{\scriptsize 117}$,
B.~Malaescu$^\textrm{\scriptsize 80}$,
Pa.~Malecki$^\textrm{\scriptsize 39}$,
V.P.~Maleev$^\textrm{\scriptsize 123}$,
F.~Malek$^\textrm{\scriptsize 55}$,
U.~Mallik$^\textrm{\scriptsize 63}$,
D.~Malon$^\textrm{\scriptsize 6}$,
C.~Malone$^\textrm{\scriptsize 143}$,
S.~Maltezos$^\textrm{\scriptsize 10}$,
V.M.~Malyshev$^\textrm{\scriptsize 109}$,
S.~Malyukov$^\textrm{\scriptsize 30}$,
J.~Mamuzic$^\textrm{\scriptsize 42}$,
G.~Mancini$^\textrm{\scriptsize 47}$,
B.~Mandelli$^\textrm{\scriptsize 30}$,
L.~Mandelli$^\textrm{\scriptsize 91a}$,
I.~Mandi\'{c}$^\textrm{\scriptsize 75}$,
J.~Maneira$^\textrm{\scriptsize 126a,126b}$,
L.~Manhaes~de~Andrade~Filho$^\textrm{\scriptsize 24b}$,
J.~Manjarres~Ramos$^\textrm{\scriptsize 159b}$,
A.~Mann$^\textrm{\scriptsize 100}$,
A.~Manousakis-Katsikakis$^\textrm{\scriptsize 9}$,
B.~Mansoulie$^\textrm{\scriptsize 136}$,
R.~Mantifel$^\textrm{\scriptsize 87}$,
M.~Mantoani$^\textrm{\scriptsize 54}$,
S.~Manzoni$^\textrm{\scriptsize 91a,91b}$,
L.~Mapelli$^\textrm{\scriptsize 30}$,
L.~March$^\textrm{\scriptsize 145c}$,
G.~Marchiori$^\textrm{\scriptsize 80}$,
M.~Marcisovsky$^\textrm{\scriptsize 127}$,
M.~Marjanovic$^\textrm{\scriptsize 13}$,
D.E.~Marley$^\textrm{\scriptsize 89}$,
F.~Marroquim$^\textrm{\scriptsize 24a}$,
S.P.~Marsden$^\textrm{\scriptsize 84}$,
Z.~Marshall$^\textrm{\scriptsize 15}$,
L.F.~Marti$^\textrm{\scriptsize 17}$,
S.~Marti-Garcia$^\textrm{\scriptsize 167}$,
B.~Martin$^\textrm{\scriptsize 90}$,
T.A.~Martin$^\textrm{\scriptsize 170}$,
V.J.~Martin$^\textrm{\scriptsize 46}$,
B.~Martin~dit~Latour$^\textrm{\scriptsize 14}$,
M.~Martinez$^\textrm{\scriptsize 12}$$^{,q}$,
S.~Martin-Haugh$^\textrm{\scriptsize 131}$,
V.S.~Martoiu$^\textrm{\scriptsize 26b}$,
A.C.~Martyniuk$^\textrm{\scriptsize 78}$,
M.~Marx$^\textrm{\scriptsize 138}$,
F.~Marzano$^\textrm{\scriptsize 132a}$,
A.~Marzin$^\textrm{\scriptsize 30}$,
L.~Masetti$^\textrm{\scriptsize 83}$,
T.~Mashimo$^\textrm{\scriptsize 155}$,
R.~Mashinistov$^\textrm{\scriptsize 96}$,
J.~Masik$^\textrm{\scriptsize 84}$,
A.L.~Maslennikov$^\textrm{\scriptsize 109}$$^{,c}$,
I.~Massa$^\textrm{\scriptsize 20a,20b}$,
L.~Massa$^\textrm{\scriptsize 20a,20b}$,
P.~Mastrandrea$^\textrm{\scriptsize 5}$,
A.~Mastroberardino$^\textrm{\scriptsize 37a,37b}$,
T.~Masubuchi$^\textrm{\scriptsize 155}$,
P.~M\"attig$^\textrm{\scriptsize 175}$,
J.~Mattmann$^\textrm{\scriptsize 83}$,
J.~Maurer$^\textrm{\scriptsize 26b}$,
S.J.~Maxfield$^\textrm{\scriptsize 74}$,
D.A.~Maximov$^\textrm{\scriptsize 109}$$^{,c}$,
R.~Mazini$^\textrm{\scriptsize 151}$,
S.M.~Mazza$^\textrm{\scriptsize 91a,91b}$,
G.~Mc~Goldrick$^\textrm{\scriptsize 158}$,
S.P.~Mc~Kee$^\textrm{\scriptsize 89}$,
A.~McCarn$^\textrm{\scriptsize 89}$,
R.L.~McCarthy$^\textrm{\scriptsize 148}$,
T.G.~McCarthy$^\textrm{\scriptsize 29}$,
K.W.~McFarlane$^\textrm{\scriptsize 56}$$^{,*}$,
J.A.~Mcfayden$^\textrm{\scriptsize 78}$,
G.~Mchedlidze$^\textrm{\scriptsize 54}$,
S.J.~McMahon$^\textrm{\scriptsize 131}$,
R.A.~McPherson$^\textrm{\scriptsize 169}$$^{,l}$,
M.~Medinnis$^\textrm{\scriptsize 42}$,
S.~Meehan$^\textrm{\scriptsize 138}$,
S.~Mehlhase$^\textrm{\scriptsize 100}$,
A.~Mehta$^\textrm{\scriptsize 74}$,
K.~Meier$^\textrm{\scriptsize 58a}$,
C.~Meineck$^\textrm{\scriptsize 100}$,
B.~Meirose$^\textrm{\scriptsize 41}$,
B.R.~Mellado~Garcia$^\textrm{\scriptsize 145c}$,
F.~Meloni$^\textrm{\scriptsize 17}$,
A.~Mengarelli$^\textrm{\scriptsize 20a,20b}$,
S.~Menke$^\textrm{\scriptsize 101}$,
E.~Meoni$^\textrm{\scriptsize 161}$,
K.M.~Mercurio$^\textrm{\scriptsize 57}$,
S.~Mergelmeyer$^\textrm{\scriptsize 16}$,
P.~Mermod$^\textrm{\scriptsize 49}$,
L.~Merola$^\textrm{\scriptsize 104a,104b}$,
C.~Meroni$^\textrm{\scriptsize 91a}$,
F.S.~Merritt$^\textrm{\scriptsize 31}$,
A.~Messina$^\textrm{\scriptsize 132a,132b}$,
J.~Metcalfe$^\textrm{\scriptsize 6}$,
A.S.~Mete$^\textrm{\scriptsize 163}$,
C.~Meyer$^\textrm{\scriptsize 83}$,
C.~Meyer$^\textrm{\scriptsize 122}$,
J-P.~Meyer$^\textrm{\scriptsize 136}$,
J.~Meyer$^\textrm{\scriptsize 107}$,
H.~Meyer~Zu~Theenhausen$^\textrm{\scriptsize 58a}$,
R.P.~Middleton$^\textrm{\scriptsize 131}$,
S.~Miglioranzi$^\textrm{\scriptsize 164a,164c}$,
L.~Mijovi\'{c}$^\textrm{\scriptsize 21}$,
G.~Mikenberg$^\textrm{\scriptsize 172}$,
M.~Mikestikova$^\textrm{\scriptsize 127}$,
M.~Miku\v{z}$^\textrm{\scriptsize 75}$,
M.~Milesi$^\textrm{\scriptsize 88}$,
A.~Milic$^\textrm{\scriptsize 30}$,
D.W.~Miller$^\textrm{\scriptsize 31}$,
C.~Mills$^\textrm{\scriptsize 46}$,
A.~Milov$^\textrm{\scriptsize 172}$,
D.A.~Milstead$^\textrm{\scriptsize 146a,146b}$,
A.A.~Minaenko$^\textrm{\scriptsize 130}$,
Y.~Minami$^\textrm{\scriptsize 155}$,
I.A.~Minashvili$^\textrm{\scriptsize 65}$,
A.I.~Mincer$^\textrm{\scriptsize 110}$,
B.~Mindur$^\textrm{\scriptsize 38a}$,
M.~Mineev$^\textrm{\scriptsize 65}$,
Y.~Ming$^\textrm{\scriptsize 173}$,
L.M.~Mir$^\textrm{\scriptsize 12}$,
K.P.~Mistry$^\textrm{\scriptsize 122}$,
T.~Mitani$^\textrm{\scriptsize 171}$,
J.~Mitrevski$^\textrm{\scriptsize 100}$,
V.A.~Mitsou$^\textrm{\scriptsize 167}$,
A.~Miucci$^\textrm{\scriptsize 49}$,
P.S.~Miyagawa$^\textrm{\scriptsize 139}$,
J.U.~Mj\"ornmark$^\textrm{\scriptsize 81}$,
T.~Moa$^\textrm{\scriptsize 146a,146b}$,
K.~Mochizuki$^\textrm{\scriptsize 85}$,
S.~Mohapatra$^\textrm{\scriptsize 35}$,
W.~Mohr$^\textrm{\scriptsize 48}$,
S.~Molander$^\textrm{\scriptsize 146a,146b}$,
R.~Moles-Valls$^\textrm{\scriptsize 21}$,
R.~Monden$^\textrm{\scriptsize 68}$,
M.C.~Mondragon$^\textrm{\scriptsize 90}$,
K.~M\"onig$^\textrm{\scriptsize 42}$,
C.~Monini$^\textrm{\scriptsize 55}$,
J.~Monk$^\textrm{\scriptsize 36}$,
E.~Monnier$^\textrm{\scriptsize 85}$,
A.~Montalbano$^\textrm{\scriptsize 148}$,
J.~Montejo~Berlingen$^\textrm{\scriptsize 30}$,
F.~Monticelli$^\textrm{\scriptsize 71}$,
S.~Monzani$^\textrm{\scriptsize 132a,132b}$,
R.W.~Moore$^\textrm{\scriptsize 3}$,
N.~Morange$^\textrm{\scriptsize 117}$,
D.~Moreno$^\textrm{\scriptsize 162}$,
M.~Moreno~Ll\'acer$^\textrm{\scriptsize 54}$,
P.~Morettini$^\textrm{\scriptsize 50a}$,
D.~Mori$^\textrm{\scriptsize 142}$,
T.~Mori$^\textrm{\scriptsize 155}$,
M.~Morii$^\textrm{\scriptsize 57}$,
M.~Morinaga$^\textrm{\scriptsize 155}$,
V.~Morisbak$^\textrm{\scriptsize 119}$,
S.~Moritz$^\textrm{\scriptsize 83}$,
A.K.~Morley$^\textrm{\scriptsize 150}$,
G.~Mornacchi$^\textrm{\scriptsize 30}$,
J.D.~Morris$^\textrm{\scriptsize 76}$,
S.S.~Mortensen$^\textrm{\scriptsize 36}$,
A.~Morton$^\textrm{\scriptsize 53}$,
L.~Morvaj$^\textrm{\scriptsize 148}$,
M.~Mosidze$^\textrm{\scriptsize 51b}$,
J.~Moss$^\textrm{\scriptsize 143}$,
K.~Motohashi$^\textrm{\scriptsize 157}$,
R.~Mount$^\textrm{\scriptsize 143}$,
E.~Mountricha$^\textrm{\scriptsize 25}$,
S.V.~Mouraviev$^\textrm{\scriptsize 96}$$^{,*}$,
E.J.W.~Moyse$^\textrm{\scriptsize 86}$,
S.~Muanza$^\textrm{\scriptsize 85}$,
R.D.~Mudd$^\textrm{\scriptsize 18}$,
F.~Mueller$^\textrm{\scriptsize 101}$,
J.~Mueller$^\textrm{\scriptsize 125}$,
R.S.P.~Mueller$^\textrm{\scriptsize 100}$,
T.~Mueller$^\textrm{\scriptsize 28}$,
D.~Muenstermann$^\textrm{\scriptsize 72}$,
P.~Mullen$^\textrm{\scriptsize 53}$,
G.A.~Mullier$^\textrm{\scriptsize 17}$,
F.J.~Munoz~Sanchez$^\textrm{\scriptsize 84}$,
J.A.~Murillo~Quijada$^\textrm{\scriptsize 18}$,
W.J.~Murray$^\textrm{\scriptsize 170,131}$,
H.~Musheghyan$^\textrm{\scriptsize 54}$,
A.G.~Myagkov$^\textrm{\scriptsize 130}$$^{,ae}$,
M.~Myska$^\textrm{\scriptsize 128}$,
B.P.~Nachman$^\textrm{\scriptsize 143}$,
O.~Nackenhorst$^\textrm{\scriptsize 49}$,
J.~Nadal$^\textrm{\scriptsize 54}$,
K.~Nagai$^\textrm{\scriptsize 120}$,
R.~Nagai$^\textrm{\scriptsize 157}$,
Y.~Nagai$^\textrm{\scriptsize 85}$,
K.~Nagano$^\textrm{\scriptsize 66}$,
Y.~Nagasaka$^\textrm{\scriptsize 59}$,
K.~Nagata$^\textrm{\scriptsize 160}$,
M.~Nagel$^\textrm{\scriptsize 101}$,
E.~Nagy$^\textrm{\scriptsize 85}$,
A.M.~Nairz$^\textrm{\scriptsize 30}$,
Y.~Nakahama$^\textrm{\scriptsize 30}$,
K.~Nakamura$^\textrm{\scriptsize 66}$,
T.~Nakamura$^\textrm{\scriptsize 155}$,
I.~Nakano$^\textrm{\scriptsize 112}$,
H.~Namasivayam$^\textrm{\scriptsize 41}$,
R.F.~Naranjo~Garcia$^\textrm{\scriptsize 42}$,
R.~Narayan$^\textrm{\scriptsize 31}$,
D.I.~Narrias~Villar$^\textrm{\scriptsize 58a}$,
T.~Naumann$^\textrm{\scriptsize 42}$,
G.~Navarro$^\textrm{\scriptsize 162}$,
R.~Nayyar$^\textrm{\scriptsize 7}$,
H.A.~Neal$^\textrm{\scriptsize 89}$,
P.Yu.~Nechaeva$^\textrm{\scriptsize 96}$,
T.J.~Neep$^\textrm{\scriptsize 84}$,
P.D.~Nef$^\textrm{\scriptsize 143}$,
A.~Negri$^\textrm{\scriptsize 121a,121b}$,
M.~Negrini$^\textrm{\scriptsize 20a}$,
S.~Nektarijevic$^\textrm{\scriptsize 106}$,
C.~Nellist$^\textrm{\scriptsize 117}$,
A.~Nelson$^\textrm{\scriptsize 163}$,
S.~Nemecek$^\textrm{\scriptsize 127}$,
P.~Nemethy$^\textrm{\scriptsize 110}$,
A.A.~Nepomuceno$^\textrm{\scriptsize 24a}$,
M.~Nessi$^\textrm{\scriptsize 30}$$^{,af}$,
M.S.~Neubauer$^\textrm{\scriptsize 165}$,
M.~Neumann$^\textrm{\scriptsize 175}$,
R.M.~Neves$^\textrm{\scriptsize 110}$,
P.~Nevski$^\textrm{\scriptsize 25}$,
P.R.~Newman$^\textrm{\scriptsize 18}$,
D.H.~Nguyen$^\textrm{\scriptsize 6}$,
R.B.~Nickerson$^\textrm{\scriptsize 120}$,
R.~Nicolaidou$^\textrm{\scriptsize 136}$,
B.~Nicquevert$^\textrm{\scriptsize 30}$,
J.~Nielsen$^\textrm{\scriptsize 137}$,
N.~Nikiforou$^\textrm{\scriptsize 35}$,
A.~Nikiforov$^\textrm{\scriptsize 16}$,
V.~Nikolaenko$^\textrm{\scriptsize 130}$$^{,ae}$,
I.~Nikolic-Audit$^\textrm{\scriptsize 80}$,
K.~Nikolopoulos$^\textrm{\scriptsize 18}$,
J.K.~Nilsen$^\textrm{\scriptsize 119}$,
P.~Nilsson$^\textrm{\scriptsize 25}$,
Y.~Ninomiya$^\textrm{\scriptsize 155}$,
A.~Nisati$^\textrm{\scriptsize 132a}$,
R.~Nisius$^\textrm{\scriptsize 101}$,
T.~Nobe$^\textrm{\scriptsize 155}$,
L.~Nodulman$^\textrm{\scriptsize 6}$,
M.~Nomachi$^\textrm{\scriptsize 118}$,
I.~Nomidis$^\textrm{\scriptsize 29}$,
T.~Nooney$^\textrm{\scriptsize 76}$,
S.~Norberg$^\textrm{\scriptsize 113}$,
M.~Nordberg$^\textrm{\scriptsize 30}$,
O.~Novgorodova$^\textrm{\scriptsize 44}$,
S.~Nowak$^\textrm{\scriptsize 101}$,
M.~Nozaki$^\textrm{\scriptsize 66}$,
L.~Nozka$^\textrm{\scriptsize 115}$,
K.~Ntekas$^\textrm{\scriptsize 10}$,
E.~Nurse$^\textrm{\scriptsize 78}$,
F.~Nuti$^\textrm{\scriptsize 88}$,
F.~O'grady$^\textrm{\scriptsize 7}$,
D.C.~O'Neil$^\textrm{\scriptsize 142}$,
V.~O'Shea$^\textrm{\scriptsize 53}$,
F.G.~Oakham$^\textrm{\scriptsize 29}$$^{,d}$,
H.~Oberlack$^\textrm{\scriptsize 101}$,
T.~Obermann$^\textrm{\scriptsize 21}$,
J.~Ocariz$^\textrm{\scriptsize 80}$,
A.~Ochi$^\textrm{\scriptsize 67}$,
I.~Ochoa$^\textrm{\scriptsize 35}$,
J.P.~Ochoa-Ricoux$^\textrm{\scriptsize 32a}$,
S.~Oda$^\textrm{\scriptsize 70}$,
S.~Odaka$^\textrm{\scriptsize 66}$,
H.~Ogren$^\textrm{\scriptsize 61}$,
A.~Oh$^\textrm{\scriptsize 84}$,
S.H.~Oh$^\textrm{\scriptsize 45}$,
C.C.~Ohm$^\textrm{\scriptsize 15}$,
H.~Ohman$^\textrm{\scriptsize 166}$,
H.~Oide$^\textrm{\scriptsize 30}$,
W.~Okamura$^\textrm{\scriptsize 118}$,
H.~Okawa$^\textrm{\scriptsize 160}$,
Y.~Okumura$^\textrm{\scriptsize 31}$,
T.~Okuyama$^\textrm{\scriptsize 66}$,
A.~Olariu$^\textrm{\scriptsize 26b}$,
S.A.~Olivares~Pino$^\textrm{\scriptsize 46}$,
D.~Oliveira~Damazio$^\textrm{\scriptsize 25}$,
A.~Olszewski$^\textrm{\scriptsize 39}$,
J.~Olszowska$^\textrm{\scriptsize 39}$,
A.~Onofre$^\textrm{\scriptsize 126a,126e}$,
K.~Onogi$^\textrm{\scriptsize 103}$,
P.U.E.~Onyisi$^\textrm{\scriptsize 31}$$^{,t}$,
C.J.~Oram$^\textrm{\scriptsize 159a}$,
M.J.~Oreglia$^\textrm{\scriptsize 31}$,
Y.~Oren$^\textrm{\scriptsize 153}$,
D.~Orestano$^\textrm{\scriptsize 134a,134b}$,
N.~Orlando$^\textrm{\scriptsize 154}$,
C.~Oropeza~Barrera$^\textrm{\scriptsize 53}$,
R.S.~Orr$^\textrm{\scriptsize 158}$,
B.~Osculati$^\textrm{\scriptsize 50a,50b}$,
R.~Ospanov$^\textrm{\scriptsize 84}$,
G.~Otero~y~Garzon$^\textrm{\scriptsize 27}$,
H.~Otono$^\textrm{\scriptsize 70}$,
M.~Ouchrif$^\textrm{\scriptsize 135d}$,
F.~Ould-Saada$^\textrm{\scriptsize 119}$,
A.~Ouraou$^\textrm{\scriptsize 136}$,
K.P.~Oussoren$^\textrm{\scriptsize 107}$,
Q.~Ouyang$^\textrm{\scriptsize 33a}$,
A.~Ovcharova$^\textrm{\scriptsize 15}$,
M.~Owen$^\textrm{\scriptsize 53}$,
R.E.~Owen$^\textrm{\scriptsize 18}$,
V.E.~Ozcan$^\textrm{\scriptsize 19a}$,
N.~Ozturk$^\textrm{\scriptsize 8}$,
K.~Pachal$^\textrm{\scriptsize 142}$,
A.~Pacheco~Pages$^\textrm{\scriptsize 12}$,
C.~Padilla~Aranda$^\textrm{\scriptsize 12}$,
M.~Pag\'{a}\v{c}ov\'{a}$^\textrm{\scriptsize 48}$,
S.~Pagan~Griso$^\textrm{\scriptsize 15}$,
E.~Paganis$^\textrm{\scriptsize 139}$,
F.~Paige$^\textrm{\scriptsize 25}$,
P.~Pais$^\textrm{\scriptsize 86}$,
K.~Pajchel$^\textrm{\scriptsize 119}$,
G.~Palacino$^\textrm{\scriptsize 159b}$,
S.~Palestini$^\textrm{\scriptsize 30}$,
M.~Palka$^\textrm{\scriptsize 38b}$,
D.~Pallin$^\textrm{\scriptsize 34}$,
A.~Palma$^\textrm{\scriptsize 126a,126b}$,
Y.B.~Pan$^\textrm{\scriptsize 173}$,
E.St.~Panagiotopoulou$^\textrm{\scriptsize 10}$,
C.E.~Pandini$^\textrm{\scriptsize 80}$,
J.G.~Panduro~Vazquez$^\textrm{\scriptsize 77}$,
P.~Pani$^\textrm{\scriptsize 146a,146b}$,
S.~Panitkin$^\textrm{\scriptsize 25}$,
D.~Pantea$^\textrm{\scriptsize 26b}$,
L.~Paolozzi$^\textrm{\scriptsize 49}$,
Th.D.~Papadopoulou$^\textrm{\scriptsize 10}$,
K.~Papageorgiou$^\textrm{\scriptsize 154}$,
A.~Paramonov$^\textrm{\scriptsize 6}$,
D.~Paredes~Hernandez$^\textrm{\scriptsize 176}$,
M.A.~Parker$^\textrm{\scriptsize 28}$,
K.A.~Parker$^\textrm{\scriptsize 139}$,
F.~Parodi$^\textrm{\scriptsize 50a,50b}$,
J.A.~Parsons$^\textrm{\scriptsize 35}$,
U.~Parzefall$^\textrm{\scriptsize 48}$,
V.~Pascuzzi$^\textrm{\scriptsize 158}$,
E.~Pasqualucci$^\textrm{\scriptsize 132a}$,
S.~Passaggio$^\textrm{\scriptsize 50a}$,
F.~Pastore$^\textrm{\scriptsize 134a,134b}$$^{,*}$,
Fr.~Pastore$^\textrm{\scriptsize 77}$,
G.~P\'asztor$^\textrm{\scriptsize 29}$,
S.~Pataraia$^\textrm{\scriptsize 175}$,
N.D.~Patel$^\textrm{\scriptsize 150}$,
J.R.~Pater$^\textrm{\scriptsize 84}$,
T.~Pauly$^\textrm{\scriptsize 30}$,
J.~Pearce$^\textrm{\scriptsize 169}$,
B.~Pearson$^\textrm{\scriptsize 113}$,
L.E.~Pedersen$^\textrm{\scriptsize 36}$,
M.~Pedersen$^\textrm{\scriptsize 119}$,
S.~Pedraza~Lopez$^\textrm{\scriptsize 167}$,
R.~Pedro$^\textrm{\scriptsize 126a,126b}$,
S.V.~Peleganchuk$^\textrm{\scriptsize 109}$$^{,c}$,
D.~Pelikan$^\textrm{\scriptsize 166}$,
O.~Penc$^\textrm{\scriptsize 127}$,
C.~Peng$^\textrm{\scriptsize 33a}$,
H.~Peng$^\textrm{\scriptsize 33b}$,
B.~Penning$^\textrm{\scriptsize 31}$,
J.~Penwell$^\textrm{\scriptsize 61}$,
D.V.~Perepelitsa$^\textrm{\scriptsize 25}$,
E.~Perez~Codina$^\textrm{\scriptsize 159a}$,
M.T.~P\'erez~Garc\'ia-Esta\~n$^\textrm{\scriptsize 167}$,
L.~Perini$^\textrm{\scriptsize 91a,91b}$,
H.~Pernegger$^\textrm{\scriptsize 30}$,
S.~Perrella$^\textrm{\scriptsize 104a,104b}$,
R.~Peschke$^\textrm{\scriptsize 42}$,
V.D.~Peshekhonov$^\textrm{\scriptsize 65}$,
K.~Peters$^\textrm{\scriptsize 30}$,
R.F.Y.~Peters$^\textrm{\scriptsize 84}$,
B.A.~Petersen$^\textrm{\scriptsize 30}$,
T.C.~Petersen$^\textrm{\scriptsize 36}$,
E.~Petit$^\textrm{\scriptsize 42}$,
A.~Petridis$^\textrm{\scriptsize 1}$,
C.~Petridou$^\textrm{\scriptsize 154}$,
P.~Petroff$^\textrm{\scriptsize 117}$,
E.~Petrolo$^\textrm{\scriptsize 132a}$,
F.~Petrucci$^\textrm{\scriptsize 134a,134b}$,
N.E.~Pettersson$^\textrm{\scriptsize 157}$,
A.~Peyaud$^\textrm{\scriptsize 136}$,
R.~Pezoa$^\textrm{\scriptsize 32b}$,
P.W.~Phillips$^\textrm{\scriptsize 131}$,
G.~Piacquadio$^\textrm{\scriptsize 143}$,
E.~Pianori$^\textrm{\scriptsize 170}$,
A.~Picazio$^\textrm{\scriptsize 86}$,
E.~Piccaro$^\textrm{\scriptsize 76}$,
M.~Piccinini$^\textrm{\scriptsize 20a,20b}$,
M.A.~Pickering$^\textrm{\scriptsize 120}$,
R.~Piegaia$^\textrm{\scriptsize 27}$,
D.T.~Pignotti$^\textrm{\scriptsize 111}$,
J.E.~Pilcher$^\textrm{\scriptsize 31}$,
A.D.~Pilkington$^\textrm{\scriptsize 84}$,
A.W.J.~Pin$^\textrm{\scriptsize 84}$,
J.~Pina$^\textrm{\scriptsize 126a,126b,126d}$,
M.~Pinamonti$^\textrm{\scriptsize 164a,164c}$$^{,ag}$,
J.L.~Pinfold$^\textrm{\scriptsize 3}$,
A.~Pingel$^\textrm{\scriptsize 36}$,
S.~Pires$^\textrm{\scriptsize 80}$,
H.~Pirumov$^\textrm{\scriptsize 42}$,
M.~Pitt$^\textrm{\scriptsize 172}$,
L.~Plazak$^\textrm{\scriptsize 144a}$,
M.-A.~Pleier$^\textrm{\scriptsize 25}$,
V.~Pleskot$^\textrm{\scriptsize 83}$,
E.~Plotnikova$^\textrm{\scriptsize 65}$,
P.~Plucinski$^\textrm{\scriptsize 146a,146b}$,
D.~Pluth$^\textrm{\scriptsize 64}$,
R.~Poettgen$^\textrm{\scriptsize 146a,146b}$,
L.~Poggioli$^\textrm{\scriptsize 117}$,
D.~Pohl$^\textrm{\scriptsize 21}$,
G.~Polesello$^\textrm{\scriptsize 121a}$,
A.~Poley$^\textrm{\scriptsize 42}$,
A.~Policicchio$^\textrm{\scriptsize 37a,37b}$,
R.~Polifka$^\textrm{\scriptsize 158}$,
A.~Polini$^\textrm{\scriptsize 20a}$,
C.S.~Pollard$^\textrm{\scriptsize 53}$,
V.~Polychronakos$^\textrm{\scriptsize 25}$,
K.~Pomm\`es$^\textrm{\scriptsize 30}$,
L.~Pontecorvo$^\textrm{\scriptsize 132a}$,
B.G.~Pope$^\textrm{\scriptsize 90}$,
G.A.~Popeneciu$^\textrm{\scriptsize 26c}$,
D.S.~Popovic$^\textrm{\scriptsize 13}$,
A.~Poppleton$^\textrm{\scriptsize 30}$,
S.~Pospisil$^\textrm{\scriptsize 128}$,
K.~Potamianos$^\textrm{\scriptsize 15}$,
I.N.~Potrap$^\textrm{\scriptsize 65}$,
C.J.~Potter$^\textrm{\scriptsize 28}$,
C.T.~Potter$^\textrm{\scriptsize 116}$,
G.~Poulard$^\textrm{\scriptsize 30}$,
J.~Poveda$^\textrm{\scriptsize 30}$,
V.~Pozdnyakov$^\textrm{\scriptsize 65}$,
M.E.~Pozo~Astigarraga$^\textrm{\scriptsize 30}$,
P.~Pralavorio$^\textrm{\scriptsize 85}$,
A.~Pranko$^\textrm{\scriptsize 15}$,
S.~Prasad$^\textrm{\scriptsize 30}$,
S.~Prell$^\textrm{\scriptsize 64}$,
D.~Price$^\textrm{\scriptsize 84}$,
L.E.~Price$^\textrm{\scriptsize 6}$,
M.~Primavera$^\textrm{\scriptsize 73a}$,
S.~Prince$^\textrm{\scriptsize 87}$,
M.~Proissl$^\textrm{\scriptsize 46}$,
K.~Prokofiev$^\textrm{\scriptsize 60c}$,
F.~Prokoshin$^\textrm{\scriptsize 32b}$,
E.~Protopapadaki$^\textrm{\scriptsize 136}$,
S.~Protopopescu$^\textrm{\scriptsize 25}$,
J.~Proudfoot$^\textrm{\scriptsize 6}$,
M.~Przybycien$^\textrm{\scriptsize 38a}$,
D.~Puddu$^\textrm{\scriptsize 134a,134b}$,
E.~Pueschel$^\textrm{\scriptsize 86}$,
D.~Puldon$^\textrm{\scriptsize 148}$,
M.~Purohit$^\textrm{\scriptsize 25}$$^{,ah}$,
P.~Puzo$^\textrm{\scriptsize 117}$,
J.~Qian$^\textrm{\scriptsize 89}$,
G.~Qin$^\textrm{\scriptsize 53}$,
Y.~Qin$^\textrm{\scriptsize 84}$,
A.~Quadt$^\textrm{\scriptsize 54}$,
D.R.~Quarrie$^\textrm{\scriptsize 15}$,
W.B.~Quayle$^\textrm{\scriptsize 164a,164b}$,
M.~Queitsch-Maitland$^\textrm{\scriptsize 84}$,
D.~Quilty$^\textrm{\scriptsize 53}$,
S.~Raddum$^\textrm{\scriptsize 119}$,
V.~Radeka$^\textrm{\scriptsize 25}$,
V.~Radescu$^\textrm{\scriptsize 42}$,
S.K.~Radhakrishnan$^\textrm{\scriptsize 148}$,
P.~Radloff$^\textrm{\scriptsize 116}$,
P.~Rados$^\textrm{\scriptsize 88}$,
F.~Ragusa$^\textrm{\scriptsize 91a,91b}$,
G.~Rahal$^\textrm{\scriptsize 178}$,
S.~Rajagopalan$^\textrm{\scriptsize 25}$,
M.~Rammensee$^\textrm{\scriptsize 30}$,
C.~Rangel-Smith$^\textrm{\scriptsize 166}$,
F.~Rauscher$^\textrm{\scriptsize 100}$,
S.~Rave$^\textrm{\scriptsize 83}$,
T.~Ravenscroft$^\textrm{\scriptsize 53}$,
M.~Raymond$^\textrm{\scriptsize 30}$,
A.L.~Read$^\textrm{\scriptsize 119}$,
N.P.~Readioff$^\textrm{\scriptsize 74}$,
D.M.~Rebuzzi$^\textrm{\scriptsize 121a,121b}$,
A.~Redelbach$^\textrm{\scriptsize 174}$,
G.~Redlinger$^\textrm{\scriptsize 25}$,
R.~Reece$^\textrm{\scriptsize 137}$,
K.~Reeves$^\textrm{\scriptsize 41}$,
L.~Rehnisch$^\textrm{\scriptsize 16}$,
J.~Reichert$^\textrm{\scriptsize 122}$,
H.~Reisin$^\textrm{\scriptsize 27}$,
C.~Rembser$^\textrm{\scriptsize 30}$,
H.~Ren$^\textrm{\scriptsize 33a}$,
M.~Rescigno$^\textrm{\scriptsize 132a}$,
S.~Resconi$^\textrm{\scriptsize 91a}$,
O.L.~Rezanova$^\textrm{\scriptsize 109}$$^{,c}$,
P.~Reznicek$^\textrm{\scriptsize 129}$,
R.~Rezvani$^\textrm{\scriptsize 95}$,
R.~Richter$^\textrm{\scriptsize 101}$,
S.~Richter$^\textrm{\scriptsize 78}$,
E.~Richter-Was$^\textrm{\scriptsize 38b}$,
O.~Ricken$^\textrm{\scriptsize 21}$,
M.~Ridel$^\textrm{\scriptsize 80}$,
P.~Rieck$^\textrm{\scriptsize 16}$,
C.J.~Riegel$^\textrm{\scriptsize 175}$,
J.~Rieger$^\textrm{\scriptsize 54}$,
O.~Rifki$^\textrm{\scriptsize 113}$,
M.~Rijssenbeek$^\textrm{\scriptsize 148}$,
A.~Rimoldi$^\textrm{\scriptsize 121a,121b}$,
L.~Rinaldi$^\textrm{\scriptsize 20a}$,
B.~Risti\'{c}$^\textrm{\scriptsize 49}$,
E.~Ritsch$^\textrm{\scriptsize 30}$,
I.~Riu$^\textrm{\scriptsize 12}$,
F.~Rizatdinova$^\textrm{\scriptsize 114}$,
E.~Rizvi$^\textrm{\scriptsize 76}$,
S.H.~Robertson$^\textrm{\scriptsize 87}$$^{,l}$,
A.~Robichaud-Veronneau$^\textrm{\scriptsize 87}$,
D.~Robinson$^\textrm{\scriptsize 28}$,
J.E.M.~Robinson$^\textrm{\scriptsize 42}$,
A.~Robson$^\textrm{\scriptsize 53}$,
C.~Roda$^\textrm{\scriptsize 124a,124b}$,
A.~Rodriguez~Perez$^\textrm{\scriptsize 12}$,
S.~Roe$^\textrm{\scriptsize 30}$,
C.S.~Rogan$^\textrm{\scriptsize 57}$,
O.~R{\o}hne$^\textrm{\scriptsize 119}$,
A.~Romaniouk$^\textrm{\scriptsize 98}$,
M.~Romano$^\textrm{\scriptsize 20a,20b}$,
S.M.~Romano~Saez$^\textrm{\scriptsize 34}$,
E.~Romero~Adam$^\textrm{\scriptsize 167}$,
N.~Rompotis$^\textrm{\scriptsize 138}$,
M.~Ronzani$^\textrm{\scriptsize 48}$,
L.~Roos$^\textrm{\scriptsize 80}$,
E.~Ros$^\textrm{\scriptsize 167}$,
S.~Rosati$^\textrm{\scriptsize 132a}$,
K.~Rosbach$^\textrm{\scriptsize 48}$,
P.~Rose$^\textrm{\scriptsize 137}$,
O.~Rosenthal$^\textrm{\scriptsize 141}$,
V.~Rossetti$^\textrm{\scriptsize 146a,146b}$,
E.~Rossi$^\textrm{\scriptsize 104a,104b}$,
L.P.~Rossi$^\textrm{\scriptsize 50a}$,
J.H.N.~Rosten$^\textrm{\scriptsize 28}$,
R.~Rosten$^\textrm{\scriptsize 138}$,
M.~Rotaru$^\textrm{\scriptsize 26b}$,
I.~Roth$^\textrm{\scriptsize 172}$,
J.~Rothberg$^\textrm{\scriptsize 138}$,
D.~Rousseau$^\textrm{\scriptsize 117}$,
C.R.~Royon$^\textrm{\scriptsize 136}$,
A.~Rozanov$^\textrm{\scriptsize 85}$,
Y.~Rozen$^\textrm{\scriptsize 152}$,
X.~Ruan$^\textrm{\scriptsize 145c}$,
F.~Rubbo$^\textrm{\scriptsize 143}$,
I.~Rubinskiy$^\textrm{\scriptsize 42}$,
V.I.~Rud$^\textrm{\scriptsize 99}$,
C.~Rudolph$^\textrm{\scriptsize 44}$,
M.S.~Rudolph$^\textrm{\scriptsize 158}$,
F.~R\"uhr$^\textrm{\scriptsize 48}$,
A.~Ruiz-Martinez$^\textrm{\scriptsize 30}$,
Z.~Rurikova$^\textrm{\scriptsize 48}$,
N.A.~Rusakovich$^\textrm{\scriptsize 65}$,
A.~Ruschke$^\textrm{\scriptsize 100}$,
H.L.~Russell$^\textrm{\scriptsize 138}$,
J.P.~Rutherfoord$^\textrm{\scriptsize 7}$,
N.~Ruthmann$^\textrm{\scriptsize 30}$,
Y.F.~Ryabov$^\textrm{\scriptsize 123}$,
M.~Rybar$^\textrm{\scriptsize 165}$,
G.~Rybkin$^\textrm{\scriptsize 117}$,
N.C.~Ryder$^\textrm{\scriptsize 120}$,
A.~Ryzhov$^\textrm{\scriptsize 130}$,
A.F.~Saavedra$^\textrm{\scriptsize 150}$,
G.~Sabato$^\textrm{\scriptsize 107}$,
S.~Sacerdoti$^\textrm{\scriptsize 27}$,
H.F-W.~Sadrozinski$^\textrm{\scriptsize 137}$,
R.~Sadykov$^\textrm{\scriptsize 65}$,
F.~Safai~Tehrani$^\textrm{\scriptsize 132a}$,
P.~Saha$^\textrm{\scriptsize 108}$,
M.~Sahinsoy$^\textrm{\scriptsize 58a}$,
M.~Saimpert$^\textrm{\scriptsize 136}$,
T.~Saito$^\textrm{\scriptsize 155}$,
H.~Sakamoto$^\textrm{\scriptsize 155}$,
Y.~Sakurai$^\textrm{\scriptsize 171}$,
G.~Salamanna$^\textrm{\scriptsize 134a,134b}$,
A.~Salamon$^\textrm{\scriptsize 133a}$,
J.E.~Salazar~Loyola$^\textrm{\scriptsize 32b}$,
M.~Saleem$^\textrm{\scriptsize 113}$,
D.~Salek$^\textrm{\scriptsize 107}$,
P.H.~Sales~De~Bruin$^\textrm{\scriptsize 138}$,
D.~Salihagic$^\textrm{\scriptsize 101}$,
A.~Salnikov$^\textrm{\scriptsize 143}$,
J.~Salt$^\textrm{\scriptsize 167}$,
D.~Salvatore$^\textrm{\scriptsize 37a,37b}$,
F.~Salvatore$^\textrm{\scriptsize 149}$,
A.~Salvucci$^\textrm{\scriptsize 60a}$,
A.~Salzburger$^\textrm{\scriptsize 30}$,
D.~Sammel$^\textrm{\scriptsize 48}$,
D.~Sampsonidis$^\textrm{\scriptsize 154}$,
A.~Sanchez$^\textrm{\scriptsize 104a,104b}$,
J.~S\'anchez$^\textrm{\scriptsize 167}$,
V.~Sanchez~Martinez$^\textrm{\scriptsize 167}$,
H.~Sandaker$^\textrm{\scriptsize 119}$,
R.L.~Sandbach$^\textrm{\scriptsize 76}$,
H.G.~Sander$^\textrm{\scriptsize 83}$,
M.P.~Sanders$^\textrm{\scriptsize 100}$,
M.~Sandhoff$^\textrm{\scriptsize 175}$,
C.~Sandoval$^\textrm{\scriptsize 162}$,
R.~Sandstroem$^\textrm{\scriptsize 101}$,
D.P.C.~Sankey$^\textrm{\scriptsize 131}$,
M.~Sannino$^\textrm{\scriptsize 50a,50b}$,
A.~Sansoni$^\textrm{\scriptsize 47}$,
C.~Santoni$^\textrm{\scriptsize 34}$,
R.~Santonico$^\textrm{\scriptsize 133a,133b}$,
H.~Santos$^\textrm{\scriptsize 126a}$,
I.~Santoyo~Castillo$^\textrm{\scriptsize 149}$,
K.~Sapp$^\textrm{\scriptsize 125}$,
A.~Sapronov$^\textrm{\scriptsize 65}$,
J.G.~Saraiva$^\textrm{\scriptsize 126a,126d}$,
B.~Sarrazin$^\textrm{\scriptsize 21}$,
O.~Sasaki$^\textrm{\scriptsize 66}$,
Y.~Sasaki$^\textrm{\scriptsize 155}$,
K.~Sato$^\textrm{\scriptsize 160}$,
G.~Sauvage$^\textrm{\scriptsize 5}$$^{,*}$,
E.~Sauvan$^\textrm{\scriptsize 5}$,
G.~Savage$^\textrm{\scriptsize 77}$,
P.~Savard$^\textrm{\scriptsize 158}$$^{,d}$,
C.~Sawyer$^\textrm{\scriptsize 131}$,
L.~Sawyer$^\textrm{\scriptsize 79}$$^{,p}$,
J.~Saxon$^\textrm{\scriptsize 31}$,
C.~Sbarra$^\textrm{\scriptsize 20a}$,
A.~Sbrizzi$^\textrm{\scriptsize 20a,20b}$,
T.~Scanlon$^\textrm{\scriptsize 78}$,
D.A.~Scannicchio$^\textrm{\scriptsize 163}$,
M.~Scarcella$^\textrm{\scriptsize 150}$,
V.~Scarfone$^\textrm{\scriptsize 37a,37b}$,
J.~Schaarschmidt$^\textrm{\scriptsize 172}$,
P.~Schacht$^\textrm{\scriptsize 101}$,
D.~Schaefer$^\textrm{\scriptsize 30}$,
R.~Schaefer$^\textrm{\scriptsize 42}$,
J.~Schaeffer$^\textrm{\scriptsize 83}$,
S.~Schaepe$^\textrm{\scriptsize 21}$,
S.~Schaetzel$^\textrm{\scriptsize 58b}$,
U.~Sch\"afer$^\textrm{\scriptsize 83}$,
A.C.~Schaffer$^\textrm{\scriptsize 117}$,
D.~Schaile$^\textrm{\scriptsize 100}$,
R.D.~Schamberger$^\textrm{\scriptsize 148}$,
V.~Scharf$^\textrm{\scriptsize 58a}$,
V.A.~Schegelsky$^\textrm{\scriptsize 123}$,
D.~Scheirich$^\textrm{\scriptsize 129}$,
M.~Schernau$^\textrm{\scriptsize 163}$,
C.~Schiavi$^\textrm{\scriptsize 50a,50b}$,
C.~Schillo$^\textrm{\scriptsize 48}$,
M.~Schioppa$^\textrm{\scriptsize 37a,37b}$,
S.~Schlenker$^\textrm{\scriptsize 30}$,
K.~Schmieden$^\textrm{\scriptsize 30}$,
C.~Schmitt$^\textrm{\scriptsize 83}$,
S.~Schmitt$^\textrm{\scriptsize 58b}$,
S.~Schmitt$^\textrm{\scriptsize 42}$,
S.~Schmitz$^\textrm{\scriptsize 83}$,
B.~Schneider$^\textrm{\scriptsize 159a}$,
Y.J.~Schnellbach$^\textrm{\scriptsize 74}$,
U.~Schnoor$^\textrm{\scriptsize 48}$,
L.~Schoeffel$^\textrm{\scriptsize 136}$,
A.~Schoening$^\textrm{\scriptsize 58b}$,
B.D.~Schoenrock$^\textrm{\scriptsize 90}$,
E.~Schopf$^\textrm{\scriptsize 21}$,
A.L.S.~Schorlemmer$^\textrm{\scriptsize 54}$,
M.~Schott$^\textrm{\scriptsize 83}$,
D.~Schouten$^\textrm{\scriptsize 159a}$,
J.~Schovancova$^\textrm{\scriptsize 8}$,
S.~Schramm$^\textrm{\scriptsize 49}$,
M.~Schreyer$^\textrm{\scriptsize 174}$,
N.~Schuh$^\textrm{\scriptsize 83}$,
M.J.~Schultens$^\textrm{\scriptsize 21}$,
H.-C.~Schultz-Coulon$^\textrm{\scriptsize 58a}$,
H.~Schulz$^\textrm{\scriptsize 16}$,
M.~Schumacher$^\textrm{\scriptsize 48}$,
B.A.~Schumm$^\textrm{\scriptsize 137}$,
Ph.~Schune$^\textrm{\scriptsize 136}$,
C.~Schwanenberger$^\textrm{\scriptsize 84}$,
A.~Schwartzman$^\textrm{\scriptsize 143}$,
T.A.~Schwarz$^\textrm{\scriptsize 89}$,
Ph.~Schwegler$^\textrm{\scriptsize 101}$,
H.~Schweiger$^\textrm{\scriptsize 84}$,
Ph.~Schwemling$^\textrm{\scriptsize 136}$,
R.~Schwienhorst$^\textrm{\scriptsize 90}$,
J.~Schwindling$^\textrm{\scriptsize 136}$,
T.~Schwindt$^\textrm{\scriptsize 21}$,
E.~Scifo$^\textrm{\scriptsize 117}$,
G.~Sciolla$^\textrm{\scriptsize 23}$,
F.~Scuri$^\textrm{\scriptsize 124a,124b}$,
F.~Scutti$^\textrm{\scriptsize 88}$,
J.~Searcy$^\textrm{\scriptsize 89}$,
P.~Seema$^\textrm{\scriptsize 21}$,
S.C.~Seidel$^\textrm{\scriptsize 105}$,
A.~Seiden$^\textrm{\scriptsize 137}$,
F.~Seifert$^\textrm{\scriptsize 128}$,
J.M.~Seixas$^\textrm{\scriptsize 24a}$,
G.~Sekhniaidze$^\textrm{\scriptsize 104a}$,
K.~Sekhon$^\textrm{\scriptsize 89}$,
S.J.~Sekula$^\textrm{\scriptsize 40}$,
D.M.~Seliverstov$^\textrm{\scriptsize 123}$$^{,*}$,
N.~Semprini-Cesari$^\textrm{\scriptsize 20a,20b}$,
C.~Serfon$^\textrm{\scriptsize 30}$,
L.~Serin$^\textrm{\scriptsize 117}$,
L.~Serkin$^\textrm{\scriptsize 164a,164b}$,
M.~Sessa$^\textrm{\scriptsize 134a,134b}$,
R.~Seuster$^\textrm{\scriptsize 159a}$,
H.~Severini$^\textrm{\scriptsize 113}$,
T.~Sfiligoj$^\textrm{\scriptsize 75}$,
F.~Sforza$^\textrm{\scriptsize 30}$,
A.~Sfyrla$^\textrm{\scriptsize 49}$,
E.~Shabalina$^\textrm{\scriptsize 54}$,
L.Y.~Shan$^\textrm{\scriptsize 33a}$,
R.~Shang$^\textrm{\scriptsize 165}$,
J.T.~Shank$^\textrm{\scriptsize 22}$,
M.~Shapiro$^\textrm{\scriptsize 15}$,
P.B.~Shatalov$^\textrm{\scriptsize 97}$,
K.~Shaw$^\textrm{\scriptsize 164a,164b}$,
S.M.~Shaw$^\textrm{\scriptsize 84}$,
A.~Shcherbakova$^\textrm{\scriptsize 146a,146b}$,
C.Y.~Shehu$^\textrm{\scriptsize 149}$,
P.~Sherwood$^\textrm{\scriptsize 78}$,
L.~Shi$^\textrm{\scriptsize 151}$$^{,ai}$,
S.~Shimizu$^\textrm{\scriptsize 67}$,
C.O.~Shimmin$^\textrm{\scriptsize 163}$,
M.~Shimojima$^\textrm{\scriptsize 102}$,
M.~Shiyakova$^\textrm{\scriptsize 65}$,
A.~Shmeleva$^\textrm{\scriptsize 96}$,
D.~Shoaleh~Saadi$^\textrm{\scriptsize 95}$,
M.J.~Shochet$^\textrm{\scriptsize 31}$,
S.~Shojaii$^\textrm{\scriptsize 91a,91b}$,
S.~Shrestha$^\textrm{\scriptsize 111}$,
E.~Shulga$^\textrm{\scriptsize 98}$,
M.A.~Shupe$^\textrm{\scriptsize 7}$,
P.~Sicho$^\textrm{\scriptsize 127}$,
P.E.~Sidebo$^\textrm{\scriptsize 147}$,
O.~Sidiropoulou$^\textrm{\scriptsize 174}$,
D.~Sidorov$^\textrm{\scriptsize 114}$,
A.~Sidoti$^\textrm{\scriptsize 20a,20b}$,
F.~Siegert$^\textrm{\scriptsize 44}$,
Dj.~Sijacki$^\textrm{\scriptsize 13}$,
J.~Silva$^\textrm{\scriptsize 126a,126d}$,
S.B.~Silverstein$^\textrm{\scriptsize 146a}$,
V.~Simak$^\textrm{\scriptsize 128}$,
O.~Simard$^\textrm{\scriptsize 5}$,
Lj.~Simic$^\textrm{\scriptsize 13}$,
S.~Simion$^\textrm{\scriptsize 117}$,
E.~Simioni$^\textrm{\scriptsize 83}$,
B.~Simmons$^\textrm{\scriptsize 78}$,
D.~Simon$^\textrm{\scriptsize 34}$,
M.~Simon$^\textrm{\scriptsize 83}$,
P.~Sinervo$^\textrm{\scriptsize 158}$,
N.B.~Sinev$^\textrm{\scriptsize 116}$,
M.~Sioli$^\textrm{\scriptsize 20a,20b}$,
G.~Siragusa$^\textrm{\scriptsize 174}$,
S.Yu.~Sivoklokov$^\textrm{\scriptsize 99}$,
J.~Sj\"{o}lin$^\textrm{\scriptsize 146a,146b}$,
T.B.~Sjursen$^\textrm{\scriptsize 14}$,
M.B.~Skinner$^\textrm{\scriptsize 72}$,
H.P.~Skottowe$^\textrm{\scriptsize 57}$,
P.~Skubic$^\textrm{\scriptsize 113}$,
M.~Slater$^\textrm{\scriptsize 18}$,
T.~Slavicek$^\textrm{\scriptsize 128}$,
M.~Slawinska$^\textrm{\scriptsize 107}$,
K.~Sliwa$^\textrm{\scriptsize 161}$,
V.~Smakhtin$^\textrm{\scriptsize 172}$,
B.H.~Smart$^\textrm{\scriptsize 46}$,
L.~Smestad$^\textrm{\scriptsize 14}$,
S.Yu.~Smirnov$^\textrm{\scriptsize 98}$,
Y.~Smirnov$^\textrm{\scriptsize 98}$,
L.N.~Smirnova$^\textrm{\scriptsize 99}$$^{,aj}$,
O.~Smirnova$^\textrm{\scriptsize 81}$,
M.N.K.~Smith$^\textrm{\scriptsize 35}$,
R.W.~Smith$^\textrm{\scriptsize 35}$,
M.~Smizanska$^\textrm{\scriptsize 72}$,
K.~Smolek$^\textrm{\scriptsize 128}$,
A.A.~Snesarev$^\textrm{\scriptsize 96}$,
G.~Snidero$^\textrm{\scriptsize 76}$,
S.~Snyder$^\textrm{\scriptsize 25}$,
R.~Sobie$^\textrm{\scriptsize 169}$$^{,l}$,
F.~Socher$^\textrm{\scriptsize 44}$,
A.~Soffer$^\textrm{\scriptsize 153}$,
D.A.~Soh$^\textrm{\scriptsize 151}$$^{,ai}$,
G.~Sokhrannyi$^\textrm{\scriptsize 75}$,
C.A.~Solans$^\textrm{\scriptsize 30}$,
M.~Solar$^\textrm{\scriptsize 128}$,
J.~Solc$^\textrm{\scriptsize 128}$,
E.Yu.~Soldatov$^\textrm{\scriptsize 98}$,
U.~Soldevila$^\textrm{\scriptsize 167}$,
A.A.~Solodkov$^\textrm{\scriptsize 130}$,
A.~Soloshenko$^\textrm{\scriptsize 65}$,
O.V.~Solovyanov$^\textrm{\scriptsize 130}$,
V.~Solovyev$^\textrm{\scriptsize 123}$,
P.~Sommer$^\textrm{\scriptsize 48}$,
H.Y.~Song$^\textrm{\scriptsize 33b}$$^{,aa}$,
N.~Soni$^\textrm{\scriptsize 1}$,
A.~Sood$^\textrm{\scriptsize 15}$,
A.~Sopczak$^\textrm{\scriptsize 128}$,
B.~Sopko$^\textrm{\scriptsize 128}$,
V.~Sopko$^\textrm{\scriptsize 128}$,
V.~Sorin$^\textrm{\scriptsize 12}$,
D.~Sosa$^\textrm{\scriptsize 58b}$,
C.L.~Sotiropoulou$^\textrm{\scriptsize 124a,124b}$,
R.~Soualah$^\textrm{\scriptsize 164a,164c}$,
A.M.~Soukharev$^\textrm{\scriptsize 109}$$^{,c}$,
D.~South$^\textrm{\scriptsize 42}$,
B.C.~Sowden$^\textrm{\scriptsize 77}$,
S.~Spagnolo$^\textrm{\scriptsize 73a,73b}$,
M.~Spalla$^\textrm{\scriptsize 124a,124b}$,
M.~Spangenberg$^\textrm{\scriptsize 170}$,
F.~Span\`o$^\textrm{\scriptsize 77}$,
W.R.~Spearman$^\textrm{\scriptsize 57}$,
D.~Sperlich$^\textrm{\scriptsize 16}$,
F.~Spettel$^\textrm{\scriptsize 101}$,
R.~Spighi$^\textrm{\scriptsize 20a}$,
G.~Spigo$^\textrm{\scriptsize 30}$,
L.A.~Spiller$^\textrm{\scriptsize 88}$,
M.~Spousta$^\textrm{\scriptsize 129}$,
R.D.~St.~Denis$^\textrm{\scriptsize 53}$$^{,*}$,
A.~Stabile$^\textrm{\scriptsize 91a}$,
S.~Staerz$^\textrm{\scriptsize 30}$,
J.~Stahlman$^\textrm{\scriptsize 122}$,
R.~Stamen$^\textrm{\scriptsize 58a}$,
S.~Stamm$^\textrm{\scriptsize 16}$,
E.~Stanecka$^\textrm{\scriptsize 39}$,
R.W.~Stanek$^\textrm{\scriptsize 6}$,
C.~Stanescu$^\textrm{\scriptsize 134a}$,
M.~Stanescu-Bellu$^\textrm{\scriptsize 42}$,
M.M.~Stanitzki$^\textrm{\scriptsize 42}$,
S.~Stapnes$^\textrm{\scriptsize 119}$,
E.A.~Starchenko$^\textrm{\scriptsize 130}$,
G.H.~Stark$^\textrm{\scriptsize 31}$,
J.~Stark$^\textrm{\scriptsize 55}$,
P.~Staroba$^\textrm{\scriptsize 127}$,
P.~Starovoitov$^\textrm{\scriptsize 58a}$,
R.~Staszewski$^\textrm{\scriptsize 39}$,
P.~Steinberg$^\textrm{\scriptsize 25}$,
B.~Stelzer$^\textrm{\scriptsize 142}$,
H.J.~Stelzer$^\textrm{\scriptsize 30}$,
O.~Stelzer-Chilton$^\textrm{\scriptsize 159a}$,
H.~Stenzel$^\textrm{\scriptsize 52}$,
G.A.~Stewart$^\textrm{\scriptsize 53}$,
J.A.~Stillings$^\textrm{\scriptsize 21}$,
M.C.~Stockton$^\textrm{\scriptsize 87}$,
M.~Stoebe$^\textrm{\scriptsize 87}$,
G.~Stoicea$^\textrm{\scriptsize 26b}$,
P.~Stolte$^\textrm{\scriptsize 54}$,
S.~Stonjek$^\textrm{\scriptsize 101}$,
A.R.~Stradling$^\textrm{\scriptsize 8}$,
A.~Straessner$^\textrm{\scriptsize 44}$,
M.E.~Stramaglia$^\textrm{\scriptsize 17}$,
J.~Strandberg$^\textrm{\scriptsize 147}$,
S.~Strandberg$^\textrm{\scriptsize 146a,146b}$,
A.~Strandlie$^\textrm{\scriptsize 119}$,
M.~Strauss$^\textrm{\scriptsize 113}$,
P.~Strizenec$^\textrm{\scriptsize 144b}$,
R.~Str\"ohmer$^\textrm{\scriptsize 174}$,
D.M.~Strom$^\textrm{\scriptsize 116}$,
R.~Stroynowski$^\textrm{\scriptsize 40}$,
A.~Strubig$^\textrm{\scriptsize 106}$,
S.A.~Stucci$^\textrm{\scriptsize 17}$,
B.~Stugu$^\textrm{\scriptsize 14}$,
N.A.~Styles$^\textrm{\scriptsize 42}$,
D.~Su$^\textrm{\scriptsize 143}$,
J.~Su$^\textrm{\scriptsize 125}$,
R.~Subramaniam$^\textrm{\scriptsize 79}$,
S.~Suchek$^\textrm{\scriptsize 58a}$,
Y.~Sugaya$^\textrm{\scriptsize 118}$,
M.~Suk$^\textrm{\scriptsize 128}$,
V.V.~Sulin$^\textrm{\scriptsize 96}$,
S.~Sultansoy$^\textrm{\scriptsize 4c}$,
T.~Sumida$^\textrm{\scriptsize 68}$,
S.~Sun$^\textrm{\scriptsize 57}$,
X.~Sun$^\textrm{\scriptsize 33a}$,
J.E.~Sundermann$^\textrm{\scriptsize 48}$,
K.~Suruliz$^\textrm{\scriptsize 149}$,
G.~Susinno$^\textrm{\scriptsize 37a,37b}$,
M.R.~Sutton$^\textrm{\scriptsize 149}$,
S.~Suzuki$^\textrm{\scriptsize 66}$,
M.~Svatos$^\textrm{\scriptsize 127}$,
M.~Swiatlowski$^\textrm{\scriptsize 31}$,
I.~Sykora$^\textrm{\scriptsize 144a}$,
T.~Sykora$^\textrm{\scriptsize 129}$,
D.~Ta$^\textrm{\scriptsize 48}$,
C.~Taccini$^\textrm{\scriptsize 134a,134b}$,
K.~Tackmann$^\textrm{\scriptsize 42}$,
J.~Taenzer$^\textrm{\scriptsize 158}$,
A.~Taffard$^\textrm{\scriptsize 163}$,
R.~Tafirout$^\textrm{\scriptsize 159a}$,
N.~Taiblum$^\textrm{\scriptsize 153}$,
H.~Takai$^\textrm{\scriptsize 25}$,
R.~Takashima$^\textrm{\scriptsize 69}$,
H.~Takeda$^\textrm{\scriptsize 67}$,
T.~Takeshita$^\textrm{\scriptsize 140}$,
Y.~Takubo$^\textrm{\scriptsize 66}$,
M.~Talby$^\textrm{\scriptsize 85}$,
A.A.~Talyshev$^\textrm{\scriptsize 109}$$^{,c}$,
J.Y.C.~Tam$^\textrm{\scriptsize 174}$,
K.G.~Tan$^\textrm{\scriptsize 88}$,
J.~Tanaka$^\textrm{\scriptsize 155}$,
R.~Tanaka$^\textrm{\scriptsize 117}$,
S.~Tanaka$^\textrm{\scriptsize 66}$,
B.B.~Tannenwald$^\textrm{\scriptsize 111}$,
S.~Tapia~Araya$^\textrm{\scriptsize 32b}$,
S.~Tapprogge$^\textrm{\scriptsize 83}$,
S.~Tarem$^\textrm{\scriptsize 152}$,
F.~Tarrade$^\textrm{\scriptsize 29}$,
G.F.~Tartarelli$^\textrm{\scriptsize 91a}$,
P.~Tas$^\textrm{\scriptsize 129}$,
M.~Tasevsky$^\textrm{\scriptsize 127}$,
T.~Tashiro$^\textrm{\scriptsize 68}$,
E.~Tassi$^\textrm{\scriptsize 37a,37b}$,
A.~Tavares~Delgado$^\textrm{\scriptsize 126a,126b}$,
Y.~Tayalati$^\textrm{\scriptsize 135d}$,
A.C.~Taylor$^\textrm{\scriptsize 105}$,
F.E.~Taylor$^\textrm{\scriptsize 94}$,
G.N.~Taylor$^\textrm{\scriptsize 88}$,
P.T.E.~Taylor$^\textrm{\scriptsize 88}$,
W.~Taylor$^\textrm{\scriptsize 159b}$,
F.A.~Teischinger$^\textrm{\scriptsize 30}$,
P.~Teixeira-Dias$^\textrm{\scriptsize 77}$,
K.K.~Temming$^\textrm{\scriptsize 48}$,
D.~Temple$^\textrm{\scriptsize 142}$,
H.~Ten~Kate$^\textrm{\scriptsize 30}$,
P.K.~Teng$^\textrm{\scriptsize 151}$,
J.J.~Teoh$^\textrm{\scriptsize 118}$,
F.~Tepel$^\textrm{\scriptsize 175}$,
S.~Terada$^\textrm{\scriptsize 66}$,
K.~Terashi$^\textrm{\scriptsize 155}$,
J.~Terron$^\textrm{\scriptsize 82}$,
S.~Terzo$^\textrm{\scriptsize 101}$,
M.~Testa$^\textrm{\scriptsize 47}$,
R.J.~Teuscher$^\textrm{\scriptsize 158}$$^{,l}$,
T.~Theveneaux-Pelzer$^\textrm{\scriptsize 85}$,
J.P.~Thomas$^\textrm{\scriptsize 18}$,
J.~Thomas-Wilsker$^\textrm{\scriptsize 77}$,
E.N.~Thompson$^\textrm{\scriptsize 35}$,
P.D.~Thompson$^\textrm{\scriptsize 18}$,
R.J.~Thompson$^\textrm{\scriptsize 84}$,
A.S.~Thompson$^\textrm{\scriptsize 53}$,
L.A.~Thomsen$^\textrm{\scriptsize 176}$,
E.~Thomson$^\textrm{\scriptsize 122}$,
M.~Thomson$^\textrm{\scriptsize 28}$,
M.J.~Tibbetts$^\textrm{\scriptsize 15}$,
R.E.~Ticse~Torres$^\textrm{\scriptsize 85}$,
V.O.~Tikhomirov$^\textrm{\scriptsize 96}$$^{,ak}$,
Yu.A.~Tikhonov$^\textrm{\scriptsize 109}$$^{,c}$,
S.~Timoshenko$^\textrm{\scriptsize 98}$,
E.~Tiouchichine$^\textrm{\scriptsize 85}$,
P.~Tipton$^\textrm{\scriptsize 176}$,
S.~Tisserant$^\textrm{\scriptsize 85}$,
K.~Todome$^\textrm{\scriptsize 157}$,
T.~Todorov$^\textrm{\scriptsize 5}$$^{,*}$,
S.~Todorova-Nova$^\textrm{\scriptsize 129}$,
J.~Tojo$^\textrm{\scriptsize 70}$,
S.~Tok\'ar$^\textrm{\scriptsize 144a}$,
K.~Tokushuku$^\textrm{\scriptsize 66}$,
K.~Tollefson$^\textrm{\scriptsize 90}$,
E.~Tolley$^\textrm{\scriptsize 57}$,
L.~Tomlinson$^\textrm{\scriptsize 84}$,
M.~Tomoto$^\textrm{\scriptsize 103}$,
L.~Tompkins$^\textrm{\scriptsize 143}$$^{,al}$,
K.~Toms$^\textrm{\scriptsize 105}$,
B.~Tong$^\textrm{\scriptsize 57}$,
E.~Torrence$^\textrm{\scriptsize 116}$,
H.~Torres$^\textrm{\scriptsize 142}$,
E.~Torr\'o~Pastor$^\textrm{\scriptsize 138}$,
J.~Toth$^\textrm{\scriptsize 85}$$^{,am}$,
F.~Touchard$^\textrm{\scriptsize 85}$,
D.R.~Tovey$^\textrm{\scriptsize 139}$,
T.~Trefzger$^\textrm{\scriptsize 174}$,
L.~Tremblet$^\textrm{\scriptsize 30}$,
A.~Tricoli$^\textrm{\scriptsize 30}$,
I.M.~Trigger$^\textrm{\scriptsize 159a}$,
S.~Trincaz-Duvoid$^\textrm{\scriptsize 80}$,
M.F.~Tripiana$^\textrm{\scriptsize 12}$,
W.~Trischuk$^\textrm{\scriptsize 158}$,
B.~Trocm\'e$^\textrm{\scriptsize 55}$,
C.~Troncon$^\textrm{\scriptsize 91a}$,
M.~Trottier-McDonald$^\textrm{\scriptsize 15}$,
M.~Trovatelli$^\textrm{\scriptsize 169}$,
L.~Truong$^\textrm{\scriptsize 164a,164c}$,
M.~Trzebinski$^\textrm{\scriptsize 39}$,
A.~Trzupek$^\textrm{\scriptsize 39}$,
C.~Tsarouchas$^\textrm{\scriptsize 30}$,
J.C-L.~Tseng$^\textrm{\scriptsize 120}$,
P.V.~Tsiareshka$^\textrm{\scriptsize 92}$,
D.~Tsionou$^\textrm{\scriptsize 154}$,
G.~Tsipolitis$^\textrm{\scriptsize 10}$,
N.~Tsirintanis$^\textrm{\scriptsize 9}$,
S.~Tsiskaridze$^\textrm{\scriptsize 12}$,
V.~Tsiskaridze$^\textrm{\scriptsize 48}$,
E.G.~Tskhadadze$^\textrm{\scriptsize 51a}$,
K.M.~Tsui$^\textrm{\scriptsize 60a}$,
I.I.~Tsukerman$^\textrm{\scriptsize 97}$,
V.~Tsulaia$^\textrm{\scriptsize 15}$,
S.~Tsuno$^\textrm{\scriptsize 66}$,
D.~Tsybychev$^\textrm{\scriptsize 148}$,
A.~Tudorache$^\textrm{\scriptsize 26b}$,
V.~Tudorache$^\textrm{\scriptsize 26b}$,
A.N.~Tuna$^\textrm{\scriptsize 57}$,
S.A.~Tupputi$^\textrm{\scriptsize 20a,20b}$,
S.~Turchikhin$^\textrm{\scriptsize 99}$$^{,aj}$,
D.~Turecek$^\textrm{\scriptsize 128}$,
D.~Turgeman$^\textrm{\scriptsize 172}$,
R.~Turra$^\textrm{\scriptsize 91a,91b}$,
A.J.~Turvey$^\textrm{\scriptsize 40}$,
P.M.~Tuts$^\textrm{\scriptsize 35}$,
A.~Tykhonov$^\textrm{\scriptsize 49}$,
M.~Tylmad$^\textrm{\scriptsize 146a,146b}$,
M.~Tyndel$^\textrm{\scriptsize 131}$,
I.~Ueda$^\textrm{\scriptsize 155}$,
R.~Ueno$^\textrm{\scriptsize 29}$,
M.~Ughetto$^\textrm{\scriptsize 146a,146b}$,
F.~Ukegawa$^\textrm{\scriptsize 160}$,
G.~Unal$^\textrm{\scriptsize 30}$,
A.~Undrus$^\textrm{\scriptsize 25}$,
G.~Unel$^\textrm{\scriptsize 163}$,
F.C.~Ungaro$^\textrm{\scriptsize 88}$,
Y.~Unno$^\textrm{\scriptsize 66}$,
C.~Unverdorben$^\textrm{\scriptsize 100}$,
J.~Urban$^\textrm{\scriptsize 144b}$,
P.~Urquijo$^\textrm{\scriptsize 88}$,
P.~Urrejola$^\textrm{\scriptsize 83}$,
G.~Usai$^\textrm{\scriptsize 8}$,
A.~Usanova$^\textrm{\scriptsize 62}$,
L.~Vacavant$^\textrm{\scriptsize 85}$,
V.~Vacek$^\textrm{\scriptsize 128}$,
B.~Vachon$^\textrm{\scriptsize 87}$,
C.~Valderanis$^\textrm{\scriptsize 83}$,
N.~Valencic$^\textrm{\scriptsize 107}$,
S.~Valentinetti$^\textrm{\scriptsize 20a,20b}$,
A.~Valero$^\textrm{\scriptsize 167}$,
L.~Valery$^\textrm{\scriptsize 12}$,
S.~Valkar$^\textrm{\scriptsize 129}$,
S.~Vallecorsa$^\textrm{\scriptsize 49}$,
J.A.~Valls~Ferrer$^\textrm{\scriptsize 167}$,
W.~Van~Den~Wollenberg$^\textrm{\scriptsize 107}$,
P.C.~Van~Der~Deijl$^\textrm{\scriptsize 107}$,
R.~van~der~Geer$^\textrm{\scriptsize 107}$,
H.~van~der~Graaf$^\textrm{\scriptsize 107}$,
N.~van~Eldik$^\textrm{\scriptsize 152}$,
P.~van~Gemmeren$^\textrm{\scriptsize 6}$,
J.~Van~Nieuwkoop$^\textrm{\scriptsize 142}$,
I.~van~Vulpen$^\textrm{\scriptsize 107}$,
M.C.~van~Woerden$^\textrm{\scriptsize 30}$,
M.~Vanadia$^\textrm{\scriptsize 132a,132b}$,
W.~Vandelli$^\textrm{\scriptsize 30}$,
R.~Vanguri$^\textrm{\scriptsize 122}$,
A.~Vaniachine$^\textrm{\scriptsize 6}$,
F.~Vannucci$^\textrm{\scriptsize 80}$,
G.~Vardanyan$^\textrm{\scriptsize 177}$,
R.~Vari$^\textrm{\scriptsize 132a}$,
E.W.~Varnes$^\textrm{\scriptsize 7}$,
T.~Varol$^\textrm{\scriptsize 40}$,
D.~Varouchas$^\textrm{\scriptsize 80}$,
A.~Vartapetian$^\textrm{\scriptsize 8}$,
K.E.~Varvell$^\textrm{\scriptsize 150}$,
F.~Vazeille$^\textrm{\scriptsize 34}$,
T.~Vazquez~Schroeder$^\textrm{\scriptsize 87}$,
J.~Veatch$^\textrm{\scriptsize 7}$,
L.M.~Veloce$^\textrm{\scriptsize 158}$,
F.~Veloso$^\textrm{\scriptsize 126a,126c}$,
T.~Velz$^\textrm{\scriptsize 21}$,
S.~Veneziano$^\textrm{\scriptsize 132a}$,
A.~Ventura$^\textrm{\scriptsize 73a,73b}$,
D.~Ventura$^\textrm{\scriptsize 86}$,
M.~Venturi$^\textrm{\scriptsize 169}$,
N.~Venturi$^\textrm{\scriptsize 158}$,
A.~Venturini$^\textrm{\scriptsize 23}$,
V.~Vercesi$^\textrm{\scriptsize 121a}$,
M.~Verducci$^\textrm{\scriptsize 132a,132b}$,
W.~Verkerke$^\textrm{\scriptsize 107}$,
J.C.~Vermeulen$^\textrm{\scriptsize 107}$,
A.~Vest$^\textrm{\scriptsize 44}$$^{,an}$,
M.C.~Vetterli$^\textrm{\scriptsize 142}$$^{,d}$,
O.~Viazlo$^\textrm{\scriptsize 81}$,
I.~Vichou$^\textrm{\scriptsize 165}$,
T.~Vickey$^\textrm{\scriptsize 139}$,
O.E.~Vickey~Boeriu$^\textrm{\scriptsize 139}$,
G.H.A.~Viehhauser$^\textrm{\scriptsize 120}$,
S.~Viel$^\textrm{\scriptsize 15}$,
R.~Vigne$^\textrm{\scriptsize 62}$,
M.~Villa$^\textrm{\scriptsize 20a,20b}$,
M.~Villaplana~Perez$^\textrm{\scriptsize 91a,91b}$,
E.~Vilucchi$^\textrm{\scriptsize 47}$,
M.G.~Vincter$^\textrm{\scriptsize 29}$,
V.B.~Vinogradov$^\textrm{\scriptsize 65}$,
I.~Vivarelli$^\textrm{\scriptsize 149}$,
S.~Vlachos$^\textrm{\scriptsize 10}$,
D.~Vladoiu$^\textrm{\scriptsize 100}$,
M.~Vlasak$^\textrm{\scriptsize 128}$,
M.~Vogel$^\textrm{\scriptsize 32a}$,
P.~Vokac$^\textrm{\scriptsize 128}$,
G.~Volpi$^\textrm{\scriptsize 124a,124b}$,
M.~Volpi$^\textrm{\scriptsize 88}$,
H.~von~der~Schmitt$^\textrm{\scriptsize 101}$,
H.~von~Radziewski$^\textrm{\scriptsize 48}$,
E.~von~Toerne$^\textrm{\scriptsize 21}$,
V.~Vorobel$^\textrm{\scriptsize 129}$,
K.~Vorobev$^\textrm{\scriptsize 98}$,
M.~Vos$^\textrm{\scriptsize 167}$,
R.~Voss$^\textrm{\scriptsize 30}$,
J.H.~Vossebeld$^\textrm{\scriptsize 74}$,
N.~Vranjes$^\textrm{\scriptsize 13}$,
M.~Vranjes~Milosavljevic$^\textrm{\scriptsize 13}$,
V.~Vrba$^\textrm{\scriptsize 127}$,
M.~Vreeswijk$^\textrm{\scriptsize 107}$,
R.~Vuillermet$^\textrm{\scriptsize 30}$,
I.~Vukotic$^\textrm{\scriptsize 31}$,
Z.~Vykydal$^\textrm{\scriptsize 128}$,
P.~Wagner$^\textrm{\scriptsize 21}$,
W.~Wagner$^\textrm{\scriptsize 175}$,
H.~Wahlberg$^\textrm{\scriptsize 71}$,
S.~Wahrmund$^\textrm{\scriptsize 44}$,
J.~Wakabayashi$^\textrm{\scriptsize 103}$,
J.~Walder$^\textrm{\scriptsize 72}$,
R.~Walker$^\textrm{\scriptsize 100}$,
W.~Walkowiak$^\textrm{\scriptsize 141}$,
V.~Wallangen$^\textrm{\scriptsize 146a,146b}$,
C.~Wang$^\textrm{\scriptsize 151}$,
F.~Wang$^\textrm{\scriptsize 173}$,
H.~Wang$^\textrm{\scriptsize 15}$,
H.~Wang$^\textrm{\scriptsize 40}$,
J.~Wang$^\textrm{\scriptsize 42}$,
J.~Wang$^\textrm{\scriptsize 150}$,
K.~Wang$^\textrm{\scriptsize 87}$,
R.~Wang$^\textrm{\scriptsize 6}$,
S.M.~Wang$^\textrm{\scriptsize 151}$,
T.~Wang$^\textrm{\scriptsize 21}$,
T.~Wang$^\textrm{\scriptsize 35}$,
X.~Wang$^\textrm{\scriptsize 176}$,
C.~Wanotayaroj$^\textrm{\scriptsize 116}$,
A.~Warburton$^\textrm{\scriptsize 87}$,
C.P.~Ward$^\textrm{\scriptsize 28}$,
D.R.~Wardrope$^\textrm{\scriptsize 78}$,
A.~Washbrook$^\textrm{\scriptsize 46}$,
P.M.~Watkins$^\textrm{\scriptsize 18}$,
A.T.~Watson$^\textrm{\scriptsize 18}$,
I.J.~Watson$^\textrm{\scriptsize 150}$,
M.F.~Watson$^\textrm{\scriptsize 18}$,
G.~Watts$^\textrm{\scriptsize 138}$,
S.~Watts$^\textrm{\scriptsize 84}$,
B.M.~Waugh$^\textrm{\scriptsize 78}$,
S.~Webb$^\textrm{\scriptsize 84}$,
M.S.~Weber$^\textrm{\scriptsize 17}$,
S.W.~Weber$^\textrm{\scriptsize 174}$,
J.S.~Webster$^\textrm{\scriptsize 6}$,
A.R.~Weidberg$^\textrm{\scriptsize 120}$,
B.~Weinert$^\textrm{\scriptsize 61}$,
J.~Weingarten$^\textrm{\scriptsize 54}$,
C.~Weiser$^\textrm{\scriptsize 48}$,
H.~Weits$^\textrm{\scriptsize 107}$,
P.S.~Wells$^\textrm{\scriptsize 30}$,
T.~Wenaus$^\textrm{\scriptsize 25}$,
T.~Wengler$^\textrm{\scriptsize 30}$,
S.~Wenig$^\textrm{\scriptsize 30}$,
N.~Wermes$^\textrm{\scriptsize 21}$,
M.~Werner$^\textrm{\scriptsize 48}$,
P.~Werner$^\textrm{\scriptsize 30}$,
M.~Wessels$^\textrm{\scriptsize 58a}$,
J.~Wetter$^\textrm{\scriptsize 161}$,
K.~Whalen$^\textrm{\scriptsize 116}$,
A.M.~Wharton$^\textrm{\scriptsize 72}$,
A.~White$^\textrm{\scriptsize 8}$,
M.J.~White$^\textrm{\scriptsize 1}$,
R.~White$^\textrm{\scriptsize 32b}$,
S.~White$^\textrm{\scriptsize 124a,124b}$,
D.~Whiteson$^\textrm{\scriptsize 163}$,
F.J.~Wickens$^\textrm{\scriptsize 131}$,
W.~Wiedenmann$^\textrm{\scriptsize 173}$,
M.~Wielers$^\textrm{\scriptsize 131}$,
P.~Wienemann$^\textrm{\scriptsize 21}$,
C.~Wiglesworth$^\textrm{\scriptsize 36}$,
L.A.M.~Wiik-Fuchs$^\textrm{\scriptsize 21}$,
A.~Wildauer$^\textrm{\scriptsize 101}$,
H.G.~Wilkens$^\textrm{\scriptsize 30}$,
H.H.~Williams$^\textrm{\scriptsize 122}$,
S.~Williams$^\textrm{\scriptsize 107}$,
C.~Willis$^\textrm{\scriptsize 90}$,
S.~Willocq$^\textrm{\scriptsize 86}$,
J.A.~Wilson$^\textrm{\scriptsize 18}$,
I.~Wingerter-Seez$^\textrm{\scriptsize 5}$,
F.~Winklmeier$^\textrm{\scriptsize 116}$,
B.T.~Winter$^\textrm{\scriptsize 21}$,
M.~Wittgen$^\textrm{\scriptsize 143}$,
J.~Wittkowski$^\textrm{\scriptsize 100}$,
S.J.~Wollstadt$^\textrm{\scriptsize 83}$,
M.W.~Wolter$^\textrm{\scriptsize 39}$,
H.~Wolters$^\textrm{\scriptsize 126a,126c}$,
B.K.~Wosiek$^\textrm{\scriptsize 39}$,
J.~Wotschack$^\textrm{\scriptsize 30}$,
M.J.~Woudstra$^\textrm{\scriptsize 84}$,
K.W.~Wozniak$^\textrm{\scriptsize 39}$,
M.~Wu$^\textrm{\scriptsize 55}$,
M.~Wu$^\textrm{\scriptsize 31}$,
S.L.~Wu$^\textrm{\scriptsize 173}$,
X.~Wu$^\textrm{\scriptsize 49}$,
Y.~Wu$^\textrm{\scriptsize 89}$,
T.R.~Wyatt$^\textrm{\scriptsize 84}$,
B.M.~Wynne$^\textrm{\scriptsize 46}$,
S.~Xella$^\textrm{\scriptsize 36}$,
D.~Xu$^\textrm{\scriptsize 33a}$,
L.~Xu$^\textrm{\scriptsize 25}$,
B.~Yabsley$^\textrm{\scriptsize 150}$,
S.~Yacoob$^\textrm{\scriptsize 145a}$,
R.~Yakabe$^\textrm{\scriptsize 67}$,
M.~Yamada$^\textrm{\scriptsize 66}$,
D.~Yamaguchi$^\textrm{\scriptsize 157}$,
Y.~Yamaguchi$^\textrm{\scriptsize 118}$,
A.~Yamamoto$^\textrm{\scriptsize 66}$,
S.~Yamamoto$^\textrm{\scriptsize 155}$,
T.~Yamanaka$^\textrm{\scriptsize 155}$,
K.~Yamauchi$^\textrm{\scriptsize 103}$,
Y.~Yamazaki$^\textrm{\scriptsize 67}$,
Z.~Yan$^\textrm{\scriptsize 22}$,
H.~Yang$^\textrm{\scriptsize 33e}$,
H.~Yang$^\textrm{\scriptsize 173}$,
Y.~Yang$^\textrm{\scriptsize 151}$,
Z.~Yang$^\textrm{\scriptsize 14}$,
W-M.~Yao$^\textrm{\scriptsize 15}$,
Y.C.~Yap$^\textrm{\scriptsize 80}$,
Y.~Yasu$^\textrm{\scriptsize 66}$,
E.~Yatsenko$^\textrm{\scriptsize 5}$,
K.H.~Yau~Wong$^\textrm{\scriptsize 21}$,
J.~Ye$^\textrm{\scriptsize 40}$,
S.~Ye$^\textrm{\scriptsize 25}$,
I.~Yeletskikh$^\textrm{\scriptsize 65}$,
A.L.~Yen$^\textrm{\scriptsize 57}$,
E.~Yildirim$^\textrm{\scriptsize 42}$,
K.~Yorita$^\textrm{\scriptsize 171}$,
R.~Yoshida$^\textrm{\scriptsize 6}$,
K.~Yoshihara$^\textrm{\scriptsize 122}$,
C.~Young$^\textrm{\scriptsize 143}$,
C.J.S.~Young$^\textrm{\scriptsize 30}$,
S.~Youssef$^\textrm{\scriptsize 22}$,
D.R.~Yu$^\textrm{\scriptsize 15}$,
J.~Yu$^\textrm{\scriptsize 8}$,
J.M.~Yu$^\textrm{\scriptsize 89}$,
J.~Yu$^\textrm{\scriptsize 64}$,
L.~Yuan$^\textrm{\scriptsize 67}$,
S.P.Y.~Yuen$^\textrm{\scriptsize 21}$,
A.~Yurkewicz$^\textrm{\scriptsize 108}$,
I.~Yusuff$^\textrm{\scriptsize 28}$$^{,ao}$,
B.~Zabinski$^\textrm{\scriptsize 39}$,
R.~Zaidan$^\textrm{\scriptsize 33d}$,
A.M.~Zaitsev$^\textrm{\scriptsize 130}$$^{,ae}$,
J.~Zalieckas$^\textrm{\scriptsize 14}$,
A.~Zaman$^\textrm{\scriptsize 148}$,
S.~Zambito$^\textrm{\scriptsize 57}$,
L.~Zanello$^\textrm{\scriptsize 132a,132b}$,
D.~Zanzi$^\textrm{\scriptsize 88}$,
C.~Zeitnitz$^\textrm{\scriptsize 175}$,
M.~Zeman$^\textrm{\scriptsize 128}$,
A.~Zemla$^\textrm{\scriptsize 38a}$,
J.C.~Zeng$^\textrm{\scriptsize 165}$,
Q.~Zeng$^\textrm{\scriptsize 143}$,
K.~Zengel$^\textrm{\scriptsize 23}$,
O.~Zenin$^\textrm{\scriptsize 130}$,
T.~\v{Z}eni\v{s}$^\textrm{\scriptsize 144a}$,
D.~Zerwas$^\textrm{\scriptsize 117}$,
D.~Zhang$^\textrm{\scriptsize 89}$,
F.~Zhang$^\textrm{\scriptsize 173}$,
G.~Zhang$^\textrm{\scriptsize 33b}$$^{,aa}$,
H.~Zhang$^\textrm{\scriptsize 33c}$,
J.~Zhang$^\textrm{\scriptsize 6}$,
L.~Zhang$^\textrm{\scriptsize 48}$,
R.~Zhang$^\textrm{\scriptsize 33b}$$^{,j}$,
X.~Zhang$^\textrm{\scriptsize 33d}$,
Z.~Zhang$^\textrm{\scriptsize 117}$,
X.~Zhao$^\textrm{\scriptsize 40}$,
Y.~Zhao$^\textrm{\scriptsize 33d,117}$,
Z.~Zhao$^\textrm{\scriptsize 33b}$,
A.~Zhemchugov$^\textrm{\scriptsize 65}$,
J.~Zhong$^\textrm{\scriptsize 120}$,
B.~Zhou$^\textrm{\scriptsize 89}$,
C.~Zhou$^\textrm{\scriptsize 45}$,
L.~Zhou$^\textrm{\scriptsize 35}$,
L.~Zhou$^\textrm{\scriptsize 40}$,
M.~Zhou$^\textrm{\scriptsize 148}$,
N.~Zhou$^\textrm{\scriptsize 33f}$,
C.G.~Zhu$^\textrm{\scriptsize 33d}$,
H.~Zhu$^\textrm{\scriptsize 33a}$,
J.~Zhu$^\textrm{\scriptsize 89}$,
Y.~Zhu$^\textrm{\scriptsize 33b}$,
X.~Zhuang$^\textrm{\scriptsize 33a}$,
K.~Zhukov$^\textrm{\scriptsize 96}$,
A.~Zibell$^\textrm{\scriptsize 174}$,
D.~Zieminska$^\textrm{\scriptsize 61}$,
N.I.~Zimine$^\textrm{\scriptsize 65}$,
C.~Zimmermann$^\textrm{\scriptsize 83}$,
S.~Zimmermann$^\textrm{\scriptsize 48}$,
Z.~Zinonos$^\textrm{\scriptsize 54}$,
M.~Zinser$^\textrm{\scriptsize 83}$,
M.~Ziolkowski$^\textrm{\scriptsize 141}$,
L.~\v{Z}ivkovi\'{c}$^\textrm{\scriptsize 13}$,
G.~Zobernig$^\textrm{\scriptsize 173}$,
A.~Zoccoli$^\textrm{\scriptsize 20a,20b}$,
M.~zur~Nedden$^\textrm{\scriptsize 16}$,
G.~Zurzolo$^\textrm{\scriptsize 104a,104b}$,
L.~Zwalinski$^\textrm{\scriptsize 30}$.
\bigskip
\\
$^{1}$ Department of Physics, University of Adelaide, Adelaide, Australia\\
$^{2}$ Physics Department, SUNY Albany, Albany NY, United States of America\\
$^{3}$ Department of Physics, University of Alberta, Edmonton AB, Canada\\
$^{4}$ $^{(a)}$ Department of Physics, Ankara University, Ankara; $^{(b)}$ Istanbul Aydin University, Istanbul; $^{(c)}$ Division of Physics, TOBB University of Economics and Technology, Ankara, Turkey\\
$^{5}$ LAPP, CNRS/IN2P3 and Universit{\'e} Savoie Mont Blanc, Annecy-le-Vieux, France\\
$^{6}$ High Energy Physics Division, Argonne National Laboratory, Argonne IL, United States of America\\
$^{7}$ Department of Physics, University of Arizona, Tucson AZ, United States of America\\
$^{8}$ Department of Physics, The University of Texas at Arlington, Arlington TX, United States of America\\
$^{9}$ Physics Department, University of Athens, Athens, Greece\\
$^{10}$ Physics Department, National Technical University of Athens, Zografou, Greece\\
$^{11}$ Institute of Physics, Azerbaijan Academy of Sciences, Baku, Azerbaijan\\
$^{12}$ Institut de F{\'\i}sica d'Altes Energies (IFAE), The Barcelona Institute of Science and Technology, Barcelona, Spain, Spain\\
$^{13}$ Institute of Physics, University of Belgrade, Belgrade, Serbia\\
$^{14}$ Department for Physics and Technology, University of Bergen, Bergen, Norway\\
$^{15}$ Physics Division, Lawrence Berkeley National Laboratory and University of California, Berkeley CA, United States of America\\
$^{16}$ Department of Physics, Humboldt University, Berlin, Germany\\
$^{17}$ Albert Einstein Center for Fundamental Physics and Laboratory for High Energy Physics, University of Bern, Bern, Switzerland\\
$^{18}$ School of Physics and Astronomy, University of Birmingham, Birmingham, United Kingdom\\
$^{19}$ $^{(a)}$ Department of Physics, Bogazici University, Istanbul; $^{(b)}$ Department of Physics Engineering, Gaziantep University, Gaziantep; $^{(c)}$ Department of Physics, Dogus University, Istanbul, Turkey\\
$^{20}$ $^{(a)}$ INFN Sezione di Bologna; $^{(b)}$ Dipartimento di Fisica e Astronomia, Universit{\`a} di Bologna, Bologna, Italy\\
$^{21}$ Physikalisches Institut, University of Bonn, Bonn, Germany\\
$^{22}$ Department of Physics, Boston University, Boston MA, United States of America\\
$^{23}$ Department of Physics, Brandeis University, Waltham MA, United States of America\\
$^{24}$ $^{(a)}$ Universidade Federal do Rio De Janeiro COPPE/EE/IF, Rio de Janeiro; $^{(b)}$ Electrical Circuits Department, Federal University of Juiz de Fora (UFJF), Juiz de Fora; $^{(c)}$ Federal University of Sao Joao del Rei (UFSJ), Sao Joao del Rei; $^{(d)}$ Instituto de Fisica, Universidade de Sao Paulo, Sao Paulo, Brazil\\
$^{25}$ Physics Department, Brookhaven National Laboratory, Upton NY, United States of America\\
$^{26}$ $^{(a)}$ Transilvania University of Brasov, Brasov, Romania; $^{(b)}$ National Institute of Physics and Nuclear Engineering, Bucharest; $^{(c)}$ National Institute for Research and Development of Isotopic and Molecular Technologies, Physics Department, Cluj Napoca; $^{(d)}$ University Politehnica Bucharest, Bucharest; $^{(e)}$ West University in Timisoara, Timisoara, Romania\\
$^{27}$ Departamento de F{\'\i}sica, Universidad de Buenos Aires, Buenos Aires, Argentina\\
$^{28}$ Cavendish Laboratory, University of Cambridge, Cambridge, United Kingdom\\
$^{29}$ Department of Physics, Carleton University, Ottawa ON, Canada\\
$^{30}$ CERN, Geneva, Switzerland\\
$^{31}$ Enrico Fermi Institute, University of Chicago, Chicago IL, United States of America\\
$^{32}$ $^{(a)}$ Departamento de F{\'\i}sica, Pontificia Universidad Cat{\'o}lica de Chile, Santiago; $^{(b)}$ Departamento de F{\'\i}sica, Universidad T{\'e}cnica Federico Santa Mar{\'\i}a, Valpara{\'\i}so, Chile\\
$^{33}$ $^{(a)}$ Institute of High Energy Physics, Chinese Academy of Sciences, Beijing; $^{(b)}$ Department of Modern Physics, University of Science and Technology of China, Anhui; $^{(c)}$ Department of Physics, Nanjing University, Jiangsu; $^{(d)}$ School of Physics, Shandong University, Shandong; $^{(e)}$ Department of Physics and Astronomy, Shanghai Key Laboratory for  Particle Physics and Cosmology, Shanghai Jiao Tong University, Shanghai; $^{(f)}$ Physics Department, Tsinghua University, Beijing 100084, China\\
$^{34}$ Laboratoire de Physique Corpusculaire, Clermont Universit{\'e} and Universit{\'e} Blaise Pascal and CNRS/IN2P3, Clermont-Ferrand, France\\
$^{35}$ Nevis Laboratory, Columbia University, Irvington NY, United States of America\\
$^{36}$ Niels Bohr Institute, University of Copenhagen, Kobenhavn, Denmark\\
$^{37}$ $^{(a)}$ INFN Gruppo Collegato di Cosenza, Laboratori Nazionali di Frascati; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} della Calabria, Rende, Italy\\
$^{38}$ $^{(a)}$ AGH University of Science and Technology, Faculty of Physics and Applied Computer Science, Krakow; $^{(b)}$ Marian Smoluchowski Institute of Physics, Jagiellonian University, Krakow, Poland\\
$^{39}$ Institute of Nuclear Physics Polish Academy of Sciences, Krakow, Poland\\
$^{40}$ Physics Department, Southern Methodist University, Dallas TX, United States of America\\
$^{41}$ Physics Department, University of Texas at Dallas, Richardson TX, United States of America\\
$^{42}$ DESY, Hamburg and Zeuthen, Germany\\
$^{43}$ Institut f{\"u}r Experimentelle Physik IV, Technische Universit{\"a}t Dortmund, Dortmund, Germany\\
$^{44}$ Institut f{\"u}r Kern-{~}und Teilchenphysik, Technische Universit{\"a}t Dresden, Dresden, Germany\\
$^{45}$ Department of Physics, Duke University, Durham NC, United States of America\\
$^{46}$ SUPA - School of Physics and Astronomy, University of Edinburgh, Edinburgh, United Kingdom\\
$^{47}$ INFN Laboratori Nazionali di Frascati, Frascati, Italy\\
$^{48}$ Fakult{\"a}t f{\"u}r Mathematik und Physik, Albert-Ludwigs-Universit{\"a}t, Freiburg, Germany\\
$^{49}$ Section de Physique, Universit{\'e} de Gen{\`e}ve, Geneva, Switzerland\\
$^{50}$ $^{(a)}$ INFN Sezione di Genova; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Genova, Genova, Italy\\
$^{51}$ $^{(a)}$ E. Andronikashvili Institute of Physics, Iv. Javakhishvili Tbilisi State University, Tbilisi; $^{(b)}$ High Energy Physics Institute, Tbilisi State University, Tbilisi, Georgia\\
$^{52}$ II Physikalisches Institut, Justus-Liebig-Universit{\"a}t Giessen, Giessen, Germany\\
$^{53}$ SUPA - School of Physics and Astronomy, University of Glasgow, Glasgow, United Kingdom\\
$^{54}$ II Physikalisches Institut, Georg-August-Universit{\"a}t, G{\"o}ttingen, Germany\\
$^{55}$ Laboratoire de Physique Subatomique et de Cosmologie, Universit{\'e} Grenoble-Alpes, CNRS/IN2P3, Grenoble, France\\
$^{56}$ Department of Physics, Hampton University, Hampton VA, United States of America\\
$^{57}$ Laboratory for Particle Physics and Cosmology, Harvard University, Cambridge MA, United States of America\\
$^{58}$ $^{(a)}$ Kirchhoff-Institut f{\"u}r Physik, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg; $^{(b)}$ Physikalisches Institut, Ruprecht-Karls-Universit{\"a}t Heidelberg, Heidelberg; $^{(c)}$ ZITI Institut f{\"u}r technische Informatik, Ruprecht-Karls-Universit{\"a}t Heidelberg, Mannheim, Germany\\
$^{59}$ Faculty of Applied Information Science, Hiroshima Institute of Technology, Hiroshima, Japan\\
$^{60}$ $^{(a)}$ Department of Physics, The Chinese University of Hong Kong, Shatin, N.T., Hong Kong; $^{(b)}$ Department of Physics, The University of Hong Kong, Hong Kong; $^{(c)}$ Department of Physics, The Hong Kong University of Science and Technology, Clear Water Bay, Kowloon, Hong Kong, China\\
$^{61}$ Department of Physics, Indiana University, Bloomington IN, United States of America\\
$^{62}$ Institut f{\"u}r Astro-{~}und Teilchenphysik, Leopold-Franzens-Universit{\"a}t, Innsbruck, Austria\\
$^{63}$ University of Iowa, Iowa City IA, United States of America\\
$^{64}$ Department of Physics and Astronomy, Iowa State University, Ames IA, United States of America\\
$^{65}$ Joint Institute for Nuclear Research, JINR Dubna, Dubna, Russia\\
$^{66}$ KEK, High Energy Accelerator Research Organization, Tsukuba, Japan\\
$^{67}$ Graduate School of Science, Kobe University, Kobe, Japan\\
$^{68}$ Faculty of Science, Kyoto University, Kyoto, Japan\\
$^{69}$ Kyoto University of Education, Kyoto, Japan\\
$^{70}$ Department of Physics, Kyushu University, Fukuoka, Japan\\
$^{71}$ Instituto de F{\'\i}sica La Plata, Universidad Nacional de La Plata and CONICET, La Plata, Argentina\\
$^{72}$ Physics Department, Lancaster University, Lancaster, United Kingdom\\
$^{73}$ $^{(a)}$ INFN Sezione di Lecce; $^{(b)}$ Dipartimento di Matematica e Fisica, Universit{\`a} del Salento, Lecce, Italy\\
$^{74}$ Oliver Lodge Laboratory, University of Liverpool, Liverpool, United Kingdom\\
$^{75}$ Department of Physics, Jo{\v{z}}ef Stefan Institute and University of Ljubljana, Ljubljana, Slovenia\\
$^{76}$ School of Physics and Astronomy, Queen Mary University of London, London, United Kingdom\\
$^{77}$ Department of Physics, Royal Holloway University of London, Surrey, United Kingdom\\
$^{78}$ Department of Physics and Astronomy, University College London, London, United Kingdom\\
$^{79}$ Louisiana Tech University, Ruston LA, United States of America\\
$^{80}$ Laboratoire de Physique Nucl{\'e}aire et de Hautes Energies, UPMC and Universit{\'e} Paris-Diderot and CNRS/IN2P3, Paris, France\\
$^{81}$ Fysiska institutionen, Lunds universitet, Lund, Sweden\\
$^{82}$ Departamento de Fisica Teorica C-15, Universidad Autonoma de Madrid, Madrid, Spain\\
$^{83}$ Institut f{\"u}r Physik, Universit{\"a}t Mainz, Mainz, Germany\\
$^{84}$ School of Physics and Astronomy, University of Manchester, Manchester, United Kingdom\\
$^{85}$ CPPM, Aix-Marseille Universit{\'e} and CNRS/IN2P3, Marseille, France\\
$^{86}$ Department of Physics, University of Massachusetts, Amherst MA, United States of America\\
$^{87}$ Department of Physics, McGill University, Montreal QC, Canada\\
$^{88}$ School of Physics, University of Melbourne, Victoria, Australia\\
$^{89}$ Department of Physics, The University of Michigan, Ann Arbor MI, United States of America\\
$^{90}$ Department of Physics and Astronomy, Michigan State University, East Lansing MI, United States of America\\
$^{91}$ $^{(a)}$ INFN Sezione di Milano; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Milano, Milano, Italy\\
$^{92}$ B.I. Stepanov Institute of Physics, National Academy of Sciences of Belarus, Minsk, Republic of Belarus\\
$^{93}$ National Scientific and Educational Centre for Particle and High Energy Physics, Minsk, Republic of Belarus\\
$^{94}$ Department of Physics, Massachusetts Institute of Technology, Cambridge MA, United States of America\\
$^{95}$ Group of Particle Physics, University of Montreal, Montreal QC, Canada\\
$^{96}$ P.N. Lebedev Physical Institute of the Russian Academy of Sciences, Moscow, Russia\\
$^{97}$ Institute for Theoretical and Experimental Physics (ITEP), Moscow, Russia\\
$^{98}$ National Research Nuclear University MEPhI, Moscow, Russia\\
$^{99}$ D.V. Skobeltsyn Institute of Nuclear Physics, M.V. Lomonosov Moscow State University, Moscow, Russia\\
$^{100}$ Fakult{\"a}t f{\"u}r Physik, Ludwig-Maximilians-Universit{\"a}t M{\"u}nchen, M{\"u}nchen, Germany\\
$^{101}$ Max-Planck-Institut f{\"u}r Physik (Werner-Heisenberg-Institut), M{\"u}nchen, Germany\\
$^{102}$ Nagasaki Institute of Applied Science, Nagasaki, Japan\\
$^{103}$ Graduate School of Science and Kobayashi-Maskawa Institute, Nagoya University, Nagoya, Japan\\
$^{104}$ $^{(a)}$ INFN Sezione di Napoli; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Napoli, Napoli, Italy\\
$^{105}$ Department of Physics and Astronomy, University of New Mexico, Albuquerque NM, United States of America\\
$^{106}$ Institute for Mathematics, Astrophysics and Particle Physics, Radboud University Nijmegen/Nikhef, Nijmegen, Netherlands\\
$^{107}$ Nikhef National Institute for Subatomic Physics and University of Amsterdam, Amsterdam, Netherlands\\
$^{108}$ Department of Physics, Northern Illinois University, DeKalb IL, United States of America\\
$^{109}$ Budker Institute of Nuclear Physics, SB RAS, Novosibirsk, Russia\\
$^{110}$ Department of Physics, New York University, New York NY, United States of America\\
$^{111}$ Ohio State University, Columbus OH, United States of America\\
$^{112}$ Faculty of Science, Okayama University, Okayama, Japan\\
$^{113}$ Homer L. Dodge Department of Physics and Astronomy, University of Oklahoma, Norman OK, United States of America\\
$^{114}$ Department of Physics, Oklahoma State University, Stillwater OK, United States of America\\
$^{115}$ Palack{\'y} University, RCPTM, Olomouc, Czech Republic\\
$^{116}$ Center for High Energy Physics, University of Oregon, Eugene OR, United States of America\\
$^{117}$ LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit{\'e} Paris-Saclay, Orsay, France\\
$^{118}$ Graduate School of Science, Osaka University, Osaka, Japan\\
$^{119}$ Department of Physics, University of Oslo, Oslo, Norway\\
$^{120}$ Department of Physics, Oxford University, Oxford, United Kingdom\\
$^{121}$ $^{(a)}$ INFN Sezione di Pavia; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Pavia, Pavia, Italy\\
$^{122}$ Department of Physics, University of Pennsylvania, Philadelphia PA, United States of America\\
$^{123}$ National Research Centre "Kurchatov Institute" B.P.Konstantinov Petersburg Nuclear Physics Institute, St. Petersburg, Russia\\
$^{124}$ $^{(a)}$ INFN Sezione di Pisa; $^{(b)}$ Dipartimento di Fisica E. Fermi, Universit{\`a} di Pisa, Pisa, Italy\\
$^{125}$ Department of Physics and Astronomy, University of Pittsburgh, Pittsburgh PA, United States of America\\
$^{126}$ $^{(a)}$ Laborat{\'o}rio de Instrumenta{\c{c}}{\~a}o e F{\'\i}sica Experimental de Part{\'\i}culas - LIP, Lisboa; $^{(b)}$ Faculdade de Ci{\^e}ncias, Universidade de Lisboa, Lisboa; $^{(c)}$ Department of Physics, University of Coimbra, Coimbra; $^{(d)}$ Centro de F{\'\i}sica Nuclear da Universidade de Lisboa, Lisboa; $^{(e)}$ Departamento de Fisica, Universidade do Minho, Braga; $^{(f)}$ Departamento de Fisica Teorica y del Cosmos and CAFPE, Universidad de Granada, Granada (Spain); $^{(g)}$ Dep Fisica and CEFITEC of Faculdade de Ciencias e Tecnologia, Universidade Nova de Lisboa, Caparica, Portugal\\
$^{127}$ Institute of Physics, Academy of Sciences of the Czech Republic, Praha, Czech Republic\\
$^{128}$ Czech Technical University in Prague, Praha, Czech Republic\\
$^{129}$ Faculty of Mathematics and Physics, Charles University in Prague, Praha, Czech Republic\\
$^{130}$ State Research Center Institute for High Energy Physics (Protvino), NRC KI, Russia\\
$^{131}$ Particle Physics Department, Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{132}$ $^{(a)}$ INFN Sezione di Roma; $^{(b)}$ Dipartimento di Fisica, Sapienza Universit{\`a} di Roma, Roma, Italy\\
$^{133}$ $^{(a)}$ INFN Sezione di Roma Tor Vergata; $^{(b)}$ Dipartimento di Fisica, Universit{\`a} di Roma Tor Vergata, Roma, Italy\\
$^{134}$ $^{(a)}$ INFN Sezione di Roma Tre; $^{(b)}$ Dipartimento di Matematica e Fisica, Universit{\`a} Roma Tre, Roma, Italy\\
$^{135}$ $^{(a)}$ Facult{\'e} des Sciences Ain Chock, R{\'e}seau Universitaire de Physique des Hautes Energies - Universit{\'e} Hassan II, Casablanca; $^{(b)}$ Centre National de l'Energie des Sciences Techniques Nucleaires, Rabat; $^{(c)}$ Facult{\'e} des Sciences Semlalia, Universit{\'e} Cadi Ayyad, LPHEA-Marrakech; $^{(d)}$ Facult{\'e} des Sciences, Universit{\'e} Mohamed Premier and LPTPM, Oujda; $^{(e)}$ Facult{\'e} des sciences, Universit{\'e} Mohammed V, Rabat, Morocco\\
$^{136}$ DSM/IRFU (Institut de Recherches sur les Lois Fondamentales de l'Univers), CEA Saclay (Commissariat {\`a} l'Energie Atomique et aux Energies Alternatives), Gif-sur-Yvette, France\\
$^{137}$ Santa Cruz Institute for Particle Physics, University of California Santa Cruz, Santa Cruz CA, United States of America\\
$^{138}$ Department of Physics, University of Washington, Seattle WA, United States of America\\
$^{139}$ Department of Physics and Astronomy, University of Sheffield, Sheffield, United Kingdom\\
$^{140}$ Department of Physics, Shinshu University, Nagano, Japan\\
$^{141}$ Fachbereich Physik, Universit{\"a}t Siegen, Siegen, Germany\\
$^{142}$ Department of Physics, Simon Fraser University, Burnaby BC, Canada\\
$^{143}$ SLAC National Accelerator Laboratory, Stanford CA, United States of America\\
$^{144}$ $^{(a)}$ Faculty of Mathematics, Physics {\&} Informatics, Comenius University, Bratislava; $^{(b)}$ Department of Subnuclear Physics, Institute of Experimental Physics of the Slovak Academy of Sciences, Kosice, Slovak Republic\\
$^{145}$ $^{(a)}$ Department of Physics, University of Cape Town, Cape Town; $^{(b)}$ Department of Physics, University of Johannesburg, Johannesburg; $^{(c)}$ School of Physics, University of the Witwatersrand, Johannesburg, South Africa\\
$^{146}$ $^{(a)}$ Department of Physics, Stockholm University; $^{(b)}$ The Oskar Klein Centre, Stockholm, Sweden\\
$^{147}$ Physics Department, Royal Institute of Technology, Stockholm, Sweden\\
$^{148}$ Departments of Physics {\&} Astronomy and Chemistry, Stony Brook University, Stony Brook NY, United States of America\\
$^{149}$ Department of Physics and Astronomy, University of Sussex, Brighton, United Kingdom\\
$^{150}$ School of Physics, University of Sydney, Sydney, Australia\\
$^{151}$ Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{152}$ Department of Physics, Technion: Israel Institute of Technology, Haifa, Israel\\
$^{153}$ Raymond and Beverly Sackler School of Physics and Astronomy, Tel Aviv University, Tel Aviv, Israel\\
$^{154}$ Department of Physics, Aristotle University of Thessaloniki, Thessaloniki, Greece\\
$^{155}$ International Center for Elementary Particle Physics and Department of Physics, The University of Tokyo, Tokyo, Japan\\
$^{156}$ Graduate School of Science and Technology, Tokyo Metropolitan University, Tokyo, Japan\\
$^{157}$ Department of Physics, Tokyo Institute of Technology, Tokyo, Japan\\
$^{158}$ Department of Physics, University of Toronto, Toronto ON, Canada\\
$^{159}$ $^{(a)}$ TRIUMF, Vancouver BC; $^{(b)}$ Department of Physics and Astronomy, York University, Toronto ON, Canada\\
$^{160}$ Faculty of Pure and Applied Sciences, and Center for Integrated Research in Fundamental Science and Engineering, University of Tsukuba, Tsukuba, Japan\\
$^{161}$ Department of Physics and Astronomy, Tufts University, Medford MA, United States of America\\
$^{162}$ Centro de Investigaciones, Universidad Antonio Narino, Bogota, Colombia\\
$^{163}$ Department of Physics and Astronomy, University of California Irvine, Irvine CA, United States of America\\
$^{164}$ $^{(a)}$ INFN Gruppo Collegato di Udine, Sezione di Trieste, Udine; $^{(b)}$ ICTP, Trieste; $^{(c)}$ Dipartimento di Chimica, Fisica e Ambiente, Universit{\`a} di Udine, Udine, Italy\\
$^{165}$ Department of Physics, University of Illinois, Urbana IL, United States of America\\
$^{166}$ Department of Physics and Astronomy, University of Uppsala, Uppsala, Sweden\\
$^{167}$ Instituto de F{\'\i}sica Corpuscular (IFIC) and Departamento de F{\'\i}sica At{\'o}mica, Molecular y Nuclear and Departamento de Ingenier{\'\i}a Electr{\'o}nica and Instituto de Microelectr{\'o}nica de Barcelona (IMB-CNM), University of Valencia and CSIC, Valencia, Spain\\
$^{168}$ Department of Physics, University of British Columbia, Vancouver BC, Canada\\
$^{169}$ Department of Physics and Astronomy, University of Victoria, Victoria BC, Canada\\
$^{170}$ Department of Physics, University of Warwick, Coventry, United Kingdom\\
$^{171}$ Waseda University, Tokyo, Japan\\
$^{172}$ Department of Particle Physics, The Weizmann Institute of Science, Rehovot, Israel\\
$^{173}$ Department of Physics, University of Wisconsin, Madison WI, United States of America\\
$^{174}$ Fakult{\"a}t f{\"u}r Physik und Astronomie, Julius-Maximilians-Universit{\"a}t, W{\"u}rzburg, Germany\\
$^{175}$ Fakult\"[a]t f{\"u}r Mathematik und Naturwissenschaften, Fachgruppe Physik, Bergische Universit{\"a}t Wuppertal, Wuppertal, Germany\\
$^{176}$ Department of Physics, Yale University, New Haven CT, United States of America\\
$^{177}$ Yerevan Physics Institute, Yerevan, Armenia\\
$^{178}$ Centre de Calcul de l'Institut National de Physique Nucl{\'e}aire et de Physique des Particules (IN2P3), Villeurbanne, France\\
$^{a}$ Also at Department of Physics, King's College London, London, United Kingdom\\
$^{b}$ Also at Institute of Physics, Azerbaijan Academy of Sciences, Baku, Azerbaijan\\
$^{c}$ Also at Novosibirsk State University, Novosibirsk, Russia\\
$^{d}$ Also at TRIUMF, Vancouver BC, Canada\\
$^{e}$ Also at Department of Physics {\&} Astronomy, University of Louisville, Louisville, KY, United States of America\\
$^{f}$ Also at Department of Physics, California State University, Fresno CA, United States of America\\
$^{g}$ Also at Department of Physics, University of Fribourg, Fribourg, Switzerland\\
$^{h}$ Also at Departamento de Fisica e Astronomia, Faculdade de Ciencias, Universidade do Porto, Portugal\\
$^{i}$ Also at Tomsk State University, Tomsk, Russia\\
$^{j}$ Also at CPPM, Aix-Marseille Universit{\'e} and CNRS/IN2P3, Marseille, France\\
$^{k}$ Also at Universita di Napoli Parthenope, Napoli, Italy\\
$^{l}$ Also at Institute of Particle Physics (IPP), Canada\\
$^{m}$ Also at Particle Physics Department, Rutherford Appleton Laboratory, Didcot, United Kingdom\\
$^{n}$ Also at Department of Physics, St. Petersburg State Polytechnical University, St. Petersburg, Russia\\
$^{o}$ Also at Department of Physics, The University of Michigan, Ann Arbor MI, United States of America\\
$^{p}$ Also at Louisiana Tech University, Ruston LA, United States of America\\
$^{q}$ Also at Institucio Catalana de Recerca i Estudis Avancats, ICREA, Barcelona, Spain\\
$^{r}$ Also at Graduate School of Science, Osaka University, Osaka, Japan\\
$^{s}$ Also at Department of Physics, National Tsing Hua University, Taiwan\\
$^{t}$ Also at Department of Physics, The University of Texas at Austin, Austin TX, United States of America\\
$^{u}$ Also at Institute of Theoretical Physics, Ilia State University, Tbilisi, Georgia\\
$^{v}$ Also at CERN, Geneva, Switzerland\\
$^{w}$ Also at Georgian Technical University (GTU),Tbilisi, Georgia\\
$^{x}$ Also at Ochadai Academic Production, Ochanomizu University, Tokyo, Japan\\
$^{y}$ Also at Manhattan College, New York NY, United States of America\\
$^{z}$ Also at Hellenic Open University, Patras, Greece\\
$^{aa}$ Also at Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{ab}$ Also at LAL, Univ. Paris-Sud, CNRS/IN2P3, Universit{\'e} Paris-Saclay, Orsay, France\\
$^{ac}$ Also at Academia Sinica Grid Computing, Institute of Physics, Academia Sinica, Taipei, Taiwan\\
$^{ad}$ Also at School of Physics, Shandong University, Shandong, China\\
$^{ae}$ Also at Moscow Institute of Physics and Technology State University, Dolgoprudny, Russia\\
$^{af}$ Also at Section de Physique, Universit{\'e} de Gen{\`e}ve, Geneva, Switzerland\\
$^{ag}$ Also at International School for Advanced Studies (SISSA), Trieste, Italy\\
$^{ah}$ Also at Department of Physics and Astronomy, University of South Carolina, Columbia SC, United States of America\\
$^{ai}$ Also at School of Physics and Engineering, Sun Yat-sen University, Guangzhou, China\\
$^{aj}$ Also at Faculty of Physics, M.V.Lomonosov Moscow State University, Moscow, Russia\\
$^{ak}$ Also at National Research Nuclear University MEPhI, Moscow, Russia\\
$^{al}$ Also at Department of Physics, Stanford University, Stanford CA, United States of America\\
$^{am}$ Also at Institute for Particle and Nuclear Physics, Wigner Research Centre for Physics, Budapest, Hungary\\
$^{an}$ Also at Flensburg University of Applied Sciences, Flensburg, Germany\\
$^{ao}$ Also at University of Malaya, Department of Physics, Kuala Lumpur, Malaysia\\
$^{*}$ Deceased
\end{flushleft}

%\end{document}
% Created with xml2latex.py

